Robots Need Some Education: On the complexity of learning in evolutionary robotics

Evolutionary Robotics and Robot Learning are two fields in robotics that aim to automatically optimize robot designs. The key difference between them lies in what is being optimized and the time scale involved. Evolutionary Robotics is a field that applies evolutionary computation techniques to evolve the morphologies or controllers, or both. Robot Learning, on the other hand, involves any learning technique aimed at optimizing a robot's controller in a given morphology. In terms of time scales, evolution occurs across multiple generations, whereas learning takes place within the `lifespan' of an individual robot. Integrating Robot Learning with Evolutionary Robotics requires the careful design of suitable learning algorithms in the context of evolutionary robotics. The effects of introducing learning into the evolutionary process are not well-understood and can thus be tricky. This thesis investigates these intricacies and presents several learning algorithms developed for an Evolutionary Robotics context.

==> 1/figures/models/models.tex <==
% \begin{minipage}[c]{0.99\textwidth}       
%         \centering
%         \includegraphics[width=\textwidth]{figures/models/legend_tu_short.eps}
% \end{minipage}

\begin{minipage}[c]{0.99\textwidth} %## ROW 1
\tiny
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[BabyA \footnotesize{$(16)$}]{\includegraphics[width=\textwidth]{figures/models/babyA.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[BabyB \footnotesize{$(22)$}]{\includegraphics[width=\textwidth]{figures/models/babyB.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Blokky \footnotesize{$(6)$}]{\includegraphics[width=\textwidth]{figures/models/blokky.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Garrix \footnotesize{$(21)$}]{\includegraphics[width=\textwidth]{figures/models/garrix.png}}
        \end{minipage}
\end{minipage}

\begin{minipage}[c]{0.99\textwidth}  %## ROW 2
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Gecko \footnotesize{$(13)$}]{\includegraphics[width=\textwidth]{figures/models/gecko.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Insect \footnotesize{$(20)$}]{\includegraphics[width=\textwidth]{figures/models/insect.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Linkin \footnotesize{$(21)$}]{\includegraphics[width=\textwidth]{figures/models/linkin.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Longleg \footnotesize{$(24)$}]{\includegraphics[width=\textwidth]{figures/models/longleg.png}}
        \end{minipage}
        \hfill
\end{minipage}

\begin{minipage}[c]{0.99\textwidth}  %## ROW 3
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Penguin \footnotesize{$(21)$}]{\includegraphics[width=\textwidth]{figures/models/penguin.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Pentapod \footnotesize{$(22)$}]{\includegraphics[width=\textwidth]{figures/models/pentapod.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Queen \footnotesize{$(19)$}]{\includegraphics[width=\textwidth]{figures/models/queen.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Salamander \footnotesize{$(25)$}]{\includegraphics[width=\textwidth]{figures/models/salamander.png}}
        \end{minipage}
\end{minipage}

\begin{minipage}[c]{0.99\textwidth}  %## ROW 4
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Snake \footnotesize{$(15)$}]{\includegraphics[width=\textwidth]{figures/models/snake.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Spider \footnotesize{$(18)$}]{\includegraphics[width=\textwidth]{figures/models/spider.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Squarish \footnotesize{$(12)$}]{\includegraphics[width=\textwidth]{figures/models/squarish.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Stingray \footnotesize{$(18)$}]{\includegraphics[width=\textwidth]{figures/models/stingray.png}}
        \end{minipage}
\end{minipage}

\begin{minipage}[c]{0.99\textwidth}  %## ROW 5
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Tinlicker \footnotesize{$(11)$}]{\includegraphics[width=\textwidth]{figures/models/tinlicker.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Turtle \footnotesize{$(28)$}]{\includegraphics[width=\textwidth]{figures/models/turtle.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[WW \footnotesize{$(17)$}]{\includegraphics[width=\textwidth]{figures/models/ww.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Zappa \footnotesize{$(22)$}]{\includegraphics[width=\textwidth]{figures/models/zappa.png}}
        \end{minipage}
\end{minipage} 
% height=2.75cm

==> 1/figures/result_contour/contour.tex <==
\begin{minipage}{0.99\textwidth}
        \begin{minipage}[t]{0.28\textwidth}
        \centering
        \subfloat[BO]{\includegraphics[width=\textwidth]{figures/result_contour/contour_bo.pdf}}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.28\textwidth}
        \centering
        \subfloat[NIPES]{\includegraphics[width=\textwidth]{figures/result_contour/contour_nipes.pdf}}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.28\textwidth}
        \centering
        \subfloat[RevDE]{\includegraphics[width=\textwidth]{figures/result_contour/contour_revde.pdf}}
    \end{minipage}
    \begin{minipage}[t]{0.075\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/result_contour/contour_grad.pdf}
    \end{minipage}
    \hfill
\end{minipage}






==> 1/figures/result_curve/curve.tex <==
% \begin{minipage}[c]{0.99\textwidth}       
%         \centering
%         \includegraphics[width=\textwidth]{figures/result_curve/legend_tu_short.eps}
% \end{minipage}
\begin{minipage}[c]{0.99\textwidth} %## ROW 1
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[BabyA]{\includegraphics[width=\textwidth]{figures/result_curve/babya.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[BabyB]{\includegraphics[width=\textwidth]{figures/result_curve/babyb.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[Blokky]{\includegraphics[width=\textwidth]{figures/result_curve/blokky.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[Garrix]{\includegraphics[width=\textwidth]{figures/result_curve/garrix.pdf}}
        \end{minipage}
\end{minipage}

\begin{minipage}[c]{0.99\textwidth}  %## ROW 2
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[Gecko]{\includegraphics[width=\textwidth]{figures/result_curve/gecko.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[Insect]{\includegraphics[width=\textwidth]{figures/result_curve/insect.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[Linkin]{\includegraphics[width=\textwidth]{figures/result_curve/linkin.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[Longleg]{\includegraphics[width=\textwidth]{figures/result_curve/longleg.pdf}}
        \end{minipage}
        \hfill
\end{minipage}

\begin{minipage}[c]{0.99\textwidth}  %## ROW 3
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[Penguin]{\includegraphics[width=\textwidth]{figures/result_curve/penguin.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[Pentapod]{\includegraphics[width=\textwidth]{figures/result_curve/pentapod.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[Queen]{\includegraphics[width=\textwidth]{figures/result_curve/queen.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[Salamander]{\includegraphics[width=\textwidth]{figures/result_curve/salamander.pdf}}
        \end{minipage}
\end{minipage}

\begin{minipage}[c]{0.99\textwidth}  %## ROW 4
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[Snake]{\includegraphics[width=\textwidth]{figures/result_curve/snake.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[Spider]{\includegraphics[width=\textwidth]{figures/result_curve/spider.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[Squarish]{\includegraphics[width=\textwidth]{figures/result_curve/squarish.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[Stingray]{\includegraphics[width=\textwidth]{figures/result_curve/stingray.pdf}}
        \end{minipage}
\end{minipage}

\begin{minipage}[c]{0.99\textwidth}  %## ROW 5
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[Tinlicker]{\includegraphics[width=\textwidth]{figures/result_curve/tinlicker.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[Turtle]{\includegraphics[width=\textwidth]{figures/result_curve/turtle.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[WW]{\includegraphics[width=\textwidth]{figures/result_curve/ww.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \subfloat[Zappa]{\includegraphics[width=\textwidth]{figures/result_curve/zappa.pdf}}
        \end{minipage}
\end{minipage} 
% height=2.75cm

==> 1/main.tex <==
% \documentclass[twoside]{article}
% \usepackage{ecj,palatino,epsfig,latexsym}
% \usepackage{booktabs} % For formal tables
% \usepackage{subcaption}
% \usepackage{tikz,xcolor,hyperref}
% \usepackage{amssymb}


% \hypersetup{%
%     pdfborder = {0 0 0}
% }
%     % packages for Flow diagrams
%     \usepackage{tikz}
%     \usetikzlibrary{shapes.geometric, arrows, positioning, automata}
%     \tikzstyle{process} = [rectangle, minimum width=2cm, minimum height=1cm, text centered, draw=black, fill=white!30]
%     \tikzstyle{sum} = \tikzstyle{sum} = [draw, circle, minimum size=.5cm]
%     \tikzstyle{arrow} = [thick,->,>=stealth]
%     \def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;}

% \renewcommand{\baselinestretch}{2}
    
% \usepackage{amsmath}
% \DeclareMathOperator{\taninv}{tan^{-1}}
% \usepackage{bm}
% \usepackage{units}
% \usepackage{float}
% \usepackage{dblfloatfix}
% \usepackage{hyperref}

% \usepackage{algorithm}
% \usepackage{algpseudocode}
% \usepackage{makecell}
%% do not add any other page- or text-size instruction here


% \title{\bf Comparing robot controller optimization methods on evolvable morphologies}  
\begin{document}

% \maketitle

% In this paper we compare Bayesian Optimization, Differential Evolution, and an Evolution Strategy, employed as a gait learning algorithm in modular robots. The motivational scenario is the joint evolution of morphologies and controllers, where `newborn' robots also undergo a learning process to optimize their inherited controllers (without changing their bodies). This context raises the question: How do gait learning algorithms compare when applied to various morphologies that are not known in advance (thus need to be treated without priors)? To answer this question, we use a test suite of twenty different robot morphologies to evaluate our gait learners and compare their efficiency, efficacy, and sensitivity to morphological differences. The results indicate that Bayesian Optimization and Differential Evolution deliver the same solution quality (walking speed for the robot) with fewer evaluations than the Evolution Strategy. Furthermore, the Evolution Strategy is more sensitive for morphological differences (its efficacy varies more between different morphologies) and is more subject to luck (repeated runs on the same morphology show greater variance in the outcomes). 

% %We investigate gait learning algorithms applied in a modular robot system where morphologies and controllers evolve simultaneously. In such systems, `newborn' robots must perform a learning process that optimizes the inherited brain for the inherited body, because stochastic recombination can reshuffle parental genes and cause a body-brain mismatch in the offspring. In this paper we compare three different algorithms for this, Bayesian Optimization, Differential Evolution, and an Evolution Strategy, applied to obtain a good controller on given robot morphologies. Akin to using a number of data sets to compare learning algorithms in Machine Learning, we use a number of robots to compare our learning algorithms. Using our test suite of twenty different morphologies, we compare the efficiency, the efficacy, and the sensitivity to differences in the morphologies. 


% \begin{keywords}
% Evolutionary robotics, morphological evolution, controller optimization

% \end{keywords}

\input{text}
% \small

% \bibliographystyle{apalike}
% \bibliography{bibliography}


\end{document}


==> 1/text.tex <==
\section{Introduction}
Evolutionary Robotics (ER) is concerned with using evolutionary methods to automate the design process of robots \cite{nolfi2000evolutionary, floreano2008evolutionary, bongard2013evolutionary, vargas2014horizons, doncieux2015evolutionary}. In general, robots consist of two major components, a body (morphology, hardware) and a brain (controller, software) and evolution can be employed to optimize both. As of today, however, a majority of ER studies considers the evolution of brains with a fixed body \cite{winfield2015evolvable, prabhu2018survey}. The specific morphologies encountered in the literature vary from simple wheeled robots, like e-pucks or Thymios, to robots with two, four or more legs, but the usual approach is to take one or more of such robots and evolve controllers for some task(s) in a given environment. Obviously, evolving both the morphology and controller simultaneously is a more general approach, but it has not received much attention from the research community so far -- perhaps, because it can be very challenging \cite{lipson2016difficulty}. 

Technically speaking, the work in this paper falls in the dominant category of optimizing the controllers of robots with a fixed body, but the motivational scenario is the joint evolution of morphologies and controllers. A key issue in this scenario is the need to optimize the controller of each `newborn' robot quickly after birth \cite{eiben2013triangle}. As phrased in \cite{eiben2020if}: ``{\em If it evolves it needs to learn}''. The main goal for this paper is to perform an experimental comparison of a number of learning methods that can be used in a generic ER system, where morphologies and controllers evolve together. We call such a system a morpho-evo-robo (M-ER) system in the sequel.


%
%\begin{figure}[h!]
%    \centering
%    \includegraphics[width=0.5\linewidth,keepaspectratio]{figures/TOL.pdf}
%    \caption{\small Triangle of life as proposed by %\cite{eiben2013triangle}. A new robot is designed and build in an evolutionary process (triangle). The new robot will undergo a lifetime learning phase (circular loop) before it is assessed for its final fitness. This can ensure the survival of capable bodies with complex control strategies that require learning.}
%    \label{fig:tol}
%\end{figure}

This context implies two specific challenges regarding the learning methods. 
 The first challenge is that the learning method needs to work on a large variety of morphologies. Unlike most papers on robot learning (where the performance of the learner is assessed on a single robot's performance), we focus on the context of learning as a nested loop inside an evolutionary process. The shapes, sizes, and complexity of the evolving robots can be very different and unpredictable during this process. Consequently, a suitable learning algorithm should work without priors and its performance should not depend much on the robots' layout. 

The second challenge is that the learning algorithm needs to be very sample efficient. Of course, algorithm efficiency is always important, but in our context it is more pressing than usually, because the number of learning trials works as a multiplier of the total optimization effort. For example, if the evolutionary process has a budget of $N$ evaluations, i.e., generating and testing $N$ robots in total (where $N$ is usually the product of the population size and the total number of generations), then allowing 1000 evaluations for learning\footnote{We maintain a broad view and see all generate-and-test search methods as potential learning algorithms if they can work in the `brain space' of the robots at hand.} increases the total number of evaluations to 1000 $\times N$. 

Given this background, the paper has two main contributions. Firstly, we provide an empirical analysis of three different algorithms that have been successfully applied as learners in robots:
\begin{enumerate}
    \item Bayesian Optimization, (BO) from \cite{lan2020learning},
    \item Evolution Strategy, (NIPES) from \cite{le2020sample},
    \item Differential Evolution, (RevDE) from \cite{tomczak2020differential},
\end{enumerate}  

Secondly, we propose and illustrate new assessment methodology. In particular, we present an algorithm to produce a test suite consisting of robots with different morphologies and explicitly consider performance variations over morphologies as a quality indicator of the learning algorithms. Furthermore, we employ morphological descriptors, e.g., size, symmetry, length-width proportion, to span a multidimensional space where we can visualize and analyze the performance of the learners. The learning algorithms\footnote{\url{https://github.com/fudavd/revolve/tree/learning}} as well as the robot test suite\footnote{\url{https://doi.org/10.34894/QMHMUO}} are open source.

The main goal of our work is to help compare different algorithms used as learning methods in an M-ER system without actually running them inside a computationally very expensive M-ER experiment. Further to the usual comparison criteria of efficiency and efficacy, we consider two more metrics: 1) how sensitive is the algorithm's performance w.r.t. the morphology of robots produced during an evolutionary process (i.e. robustness) and 2) how sensitive is the algorithm's performance w.r.t. random effects during its execution (i.e. consistency or luckiness on a given morphology).
%The specific objective of this study is to compare three different algorithms that have been successfully applied as learners in robots:
%\begin{enumerate}
%    \item Bayesian Optimization, (BO) from \cite{lan2021learning},
%    \item Evolution Strategy, (NIPES) from \cite{le2020sample},
%    \item Differential Evolution, (RevDE) from \cite{tomczak2020differential},
%\end{enumerate}  
% \noindent with a tight budget of 300 trials. 
%The comparison will take three measures into account: efficiency, efficacy, and the robustness to different morphologies.



%Our approach to compare these algorithms is influenced by the two challenges discussed above. Regarding the first one, we propose a new methodology. This methodology is motivated by the usual practice in {\it machine learning}, where algorithms are compared on a number of data sets as test cases. In our context of {\it learning machines}, a good test case is not a database, but a specific robot body. Thus, in this study we specify a test suite of $N$ robots and compare the aforementioned algorithms on all of these. Regarding the need for speed, we maintain a low budget in terms of learning trials, 300 task-performance evaluations. This number is a practically motivated trade-off. With one minute per trial the whole learning process is doable in the real world in one working day (accounting for additional overhead), while preliminary experiments indicated that 300 trials can be sufficient to obtain decent task-performance in our application.



% We propose $<$5 hours of simulated time as it would be feasible to conduct a single experiment in the real world in one working day (accounting for additional overhead).

\section{Related Work}
Early M-ER work already showed the challenge for pure body-controller evolution to produce complex robots, without learning, \cite{pollack2000golem, hornby2001body}. Learning, as we propose, helps to reduce the effect of an initial body-brain mismatch which can lead to reduced efficacy \cite{medvet2021biodiversity}, and early convergence by lowering morphological variation in the population \cite{lipson2016difficulty}. 
Similar to learning, several papers have suggested slightly different solutions to mitigate the body-brain mismatch problem.
\cite{cheney2018scalable} implemented a form of novelty protection in which `younger' robot designs were protected from individuals that survived for more generations. Protecting a novel individual will increase its chance to adapt the controller properly for its body. This technique corresponds with implementing a single learning iteration every time a morphology is protected. Such an approach is thus similar to ours except that our robots are always protected for a fixed period. Similarly, \cite{de2020influences} implemented protection in the form of speciation within their version of NEAT \cite{stanley2002evolving}.  More recently \cite{le2022morpho} proposed a library of controller structures for several robot types to reduce the initial mismatch problem.

\cite{nygaard2017overcoming} demonstrated improvements in their M-ER system by introducing two phases during evolution. The first phase consists of both controller and morphology evolution, while during the second phase only the controller evolves in a fixed body. The results showed that, without the second phase, morphology and controller evolution led to sub-optimal controllers which required additional fine-tuning. We extend on this research by investigating different learners and applied on several different morphologies.

As mentioned before, investigating learning methods for evolutionary robotics implies additional constraints in terms of general applicability (shape and size). Similarly to our work, \cite{10.1162/ARTL_a_00223} investigated different online gait learning algorithms (RL-PoWER, \cite{kober2009policy}; simulated annealing, \cite{aarts1989simulated}; and HyperNEAT, \cite{gauci:gecco07}), and analyzed the predictability of the optimized fitness values.

At last, let us clarify the relation between learning as we discuss it here and existing M-ER research on controller evolution. Optimizing robot controllers by evolutionary algorithms on given, fixed robot morphologies (the majority of M-ER research) can be seen as a sub-area within the field of robot controller optimization. In that field, the focus is on the optimization of a specific robot with a possibly high computational budget and M-ER is distinguished by the choice for a specific type of optimizers, Evolutionary Algorithms. For our study, robot evolution is the enveloping context, where an evolutionary process optimizes robot morphologies and controllers simultaneously and we use learning as an addition within the evolutionary loop. As said above, we are very open and see many types of algorithms as potential learners, e.g., Reinforcement Learning, Simulated Annealing, Bayesian Optimization and Evolutionary Algorithms.


%Here, we focus on controller optimization (i.e. additional learning) integrated within an evolutionary process. Lifetime learning requires broad applicability (over different morphologies) with a limited budget (high efficiency). In contrast to regular controller optimization, which often focuses on the optimization of a specific robot with a high computational budget. An additional advantage of `learning' within the evolutionary loop is that we can introduce other types of optimizers. For example reinforcement learning \cite{jelisavcic2017real}, Bayesian Optimization \cite{lan2018directed}, and CPPNs \cite{jelisavcic2019lamarckian}. 

% In a paper by \cite{lan2020time}, BO was compared to a standard EA and an algorithm that implemented EA with BO initialization BEA. The comparison showed that Although BO performed initially better than the standard EA algorithm, the sample-efficiency led to an early convergence and thus lower end-performance compared to the EA. 
% This showed the characteristics of both algorithms, namely fast but sub-optimal in BO and slow but robust EA. The BEA algorithm tried to get the best from both worlds and showed a significant difference between end-performance (vs. BO) and rate of learning (vs. EA).


%%%%%%%%%%%%%%%%%%%%%%%%%%% System description %%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{System description}
An evolutionary robotics system demands the robot designs to be evolvable (both body and brain). Although we only focus on the learning with a fixed body in this paper, keep in mind that we limit ourselves in the following ways: 1) Morphologies are modular to be able to evolve in a full evolutionary setup. This results in a discrete robot design space where small morphological differences require very different optimal control. 2) Controllers are model-agnostic --meaning that they don't assume a certain robot/functionality-- and scalable in the sense that they can provide control for any amount/type of motor on the robot. Such demands for the robot controller will affect the learning algorithm for the controller as well.

The aforementioned properties are desirable in a well-functioning evolutionary robotics system. We can hypothesize possible requirements/advantageous properties for our learning algorithms as well. But, to our knowledge, we are the first to investigate this by direct comparison on a wide variety of robot instances.


\subsection{Robot morphologies}
Our robots consist of modules based on the RoboGen framework \cite{auerbach2014robogen}. We altered the original design to match real-world counterparts and only use the following modules: core component, brick components, and active hinges. The core component function as a container for a micro-controller with battery, and is a large brick with four attachment slots on its lateral faces. The brick component is a smaller cube with attachment points on its lateral sides. The active hinge component is a joint actuated by a servomotor with an attachment point on both ends.  Pictures of the real modules are shown below (\autoref{fig:modules}). We can describe a robot's genotype using a tree structure with the core module as the root node (such a tree is depicted in \autoref{fig:CPG_model_comparing}b).

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.75\linewidth,keepaspectratio]{figures/modules.jpg}
    \caption{\small Real instances of the modules we simulate. From left to right: Core module with micro-controller and battery, active hinge/joint, and brick.}
    \label{fig:modules}
\end{figure}

\subsection{Robot controllers} In this study, the controllers are optimized for gait-learning (i.e. move as far as possible in any direction within a certain time). We used a network of interconnected Central Pattern Generators (CPGs) with internal model control feedback, as it has shown to improve learning \cite{van2020effects}. In short, CPGs are pairs of artificial neurons ($x_i$,$y_i$) that reciprocally inhibit and excite each other to produce oscillatory behavior \cite{ijspeert2008central}. Here, $i$ denotes the specific joint that is associated with a single CPG. The change of a neuron state is calculated by multiplying the current state of the opposite neuron with a weight ($w$), shown in \autoref{fig:CPG_model_comparing}a. The weights $w_{x_iy_i}$ and $w_{y_ix_i}$ represent a connection between each neuron pair. A output neuron $out_i$ is coupled to the $x$-neuron with an strength $w_{x_io_i}$. The output of $out_i$ will serve as the input command to the servomotors in a joint (\textit{i.e.} servo). In our case, we picked a tangent hyperbolic activation function as our output neuron to bound the motor input between [-1,1]. 


\begin{figure}[ht]
\centering
\begin{minipage}[c]{\linewidth}
% \hspace{2em}
        \begin{minipage}[t]{0.45\linewidth}
            \centering
            \subfloat[CPG]{\input{figures/CPG}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.45\linewidth}
            \centering
            \subfloat[CPG network]{\input{figures/CPG_net}}
        \end{minipage}

            % \includegraphics[width=0.6\linewidth, ,keepaspectratio]{Figures/CPG_model.png}
           \vspace{-.5em} \caption{\textbf{a}) A single CPG. \textbf{b}) The CPG network for our Spider, containing 8 CPGs (numbers) with 10 connections (blue lines).}\label{fig:CPG_model_comparing}
\end{minipage}
\end{figure}

To enable more complex output patterns, CPG connections between neighboring joints are allowed, see \autoref{fig:CPG_model_comparing}b. We define neighboring joints at joint $i$ as the set ($\mathcal{N}_i$) of each joint $j$ positioned within a Manhattan distance of 2 modules (i.e. discrete modular distance $\bm{l}_1$=2). The resulting differential equations of the CPG network is shown in \autoref{eq:ODE_CPG_comparing}. Connections between neighboring joints $j$ are denoted as $w_{x_jx_i}$.
        
        \begin{align}\label{eq:ODE_CPG_comparing}
            % \begin{split}
                \Dot{x}_i = w_{y_ix_i}y_i + \sum_{j \in \mathcal{N}_i} x_{j} w_{x_jx_i} &&\Dot{y}_i = w_{x_iy_i}x_i
            % \end{split}
        \end{align}
        
By changing the weights of the CPGs, we can improve our controller for the task of gait-learning. To simplify the search space, the following relations are imposed between the weights: $w_{x_iy_i} = -w_{y_ix_i}$; $ w_{x_jx_i} = -w_{x_ix_j}$; $w_{x_io_i} = 1$. For a given network containing $N_C$ CPGs and $|\mathcal{N}|$ neighboring pairs, the total number of weights to be optimized equate to $N_w=N_C+|\mathcal{N}|$ i.e., a search space $\left(\mathbb{R}^{N_w} \right)$. At the start of each learning trial all neurons' initial states will be set to a predefined value $(x,y)=\left(-\frac{1}{\sqrt{2}},\frac{1}{\sqrt{2}}\right)$. The sampling period of the controller is $\unit[0.125]{s}$.
        
        % \begin{equation}\label{eq:output}
        %     \begin{split}
        %         out_i(x_i) & = \frac{2}{1 + e^{-2 x_iw_{x_io_i}}} - 1
        %     \end{split}
        % \end{equation}
        
\subsection{Learning methods}
At the start of optimization, we initialize the robot's CPG-network with uniform random weights between $[-1, 1]$. Subsequently, gait-learning is done by changing the weights of the respective network. We limit the number of evaluations to 300 trials, which has shown to be sufficient to learn viable controllers using BO \cite{lan2020learning}. Additionally, 300 trials would equate to 5 hours of simulated time which can be conducted within one working day in the real world (accounting for additional overhead).

\textit{Bayesian Optimization} is a state-of-the-art framework that had successful implementations in machine-learning, engineering, and science \cite{jasper2012practical}. In short, the BO algorithm contains two different functionalities. The first functionality is a function approximator that tries to model the fitness as a function of the search space parameters (in our case the weights of the CPG network). In theory, this approximator can be any type of function, but in BO Gaussian Processes ($\mathcal{GP}$) are used for their sample efficiency. The second functionality is an acquisition function that selects the next sample in the search space. The acquisition function chooses between samples that show high potential in fitness by the $\mathcal{GP}$ (exploitation), or that show a high degree of uncertainty by the $\mathcal{GP}$ (exploration). BO is interesting as a well-known benchmark for sample efficient search algorithms, as well as its proven track-record to learn gait quickly on our evolutionary system \cite{lan2020time}. 

With the specific choice on the type of kernel for the $\mathcal{GP}$ and acquisition function, we can tailor the BO algorithm. We choose an upper confidence bound acquisition function and Mat\'ern 5/2 kernel. As initialization, we use Latin Hypercube Sampling that selects 50 evenly distributed pseudo-random samples in search-space. The hyper-parameters of the BO are shown in \autoref{tab:parameters_comparing}. Hyper-parameters were obtained by extensive grid-search in previous work \cite{lan2020learning}.

\textit{Evolutionary Strategies} are evolutionary optimization algorithms in which a mutation operation is done by adding a random vector in search space. The distribution of the random vector (\textit{i.e.} mean, variance and correlation with a multivariate distribution) is often defined using Co-variance Matrix adaptation (CMA-ES, \cite{hansen2016cma}). A basic cycle of the CMA-ES is as follows: (1) draw $\lambda$-samples from a normal distribution over search space; (2) evaluate the fitness over $\lambda$-samples; (3) perform selection over the top $\mu$-samples; (4) With the new population adapt the covariance matrix with $\sigma$-step (that decreases over the generations); (5) draw $\lambda$-samples according to the new distribution defined by the covariance matrix and repeat from (2).

For our ES learner, we implement a special CMA-ES algorithm with Novelty search and restart mechanisms with Increasing Population (NIPES), from \cite{le2020sample}. Here, novelty is based on the difference in CPG-weights between individuals within the current population and an archive of previous generations. Restart mechanisms re-initialize the evolutionary process with a doubled population size, every time a stopping criterion is met. These mechanisms address early convergence, the degeneration of the covariance matrix and the need for more global exploration. Our initial population size ($\lambda_0$) is set at 10 individuals, with $\sigma$ equal to 1. Stagnation threshold is defined as a standard deviation $\leq 0.05$ over the fitness values within a population and the between the last 5 generations. Other hyper-parameters of the NIPES algorithm are shown in \autoref{tab:parameters_comparing}.

\textit{Differential Evolution} is an EA that samples new candidates by perturbing the current population \cite{storn1997differential}. This perturbation is calculated using linear operations over two genotype vectors that are obtained by randomly shuffling the current population. An advantage of this approach is that the optimization does not require any assumption on the distribution of the population (unlike ES), meaning that the DE approach is model agnostic. A potential limitation in DE is that it can suffer from small populations and lose diversity too quickly. This is because the randomness of the perturbation (when creating new samples) is directly linked to the size of the population. Unfortunately, we can not afford a very large population size to prevent this limitation, due to our tight budget of 300 evaluations. 

Reversible DE (RevDE) proposes a solution by applying a special set of linearly reversible transformation to produce a wide spread over search space when selecting new samples \cite{tomczak2020differential}. The algorithm works as follows: (1) initialize a population of size $\lambda$ (2) evaluate the fitness over all $\lambda$-samples; (3) select the top $\mu$-samples to obtain genotype vectors $\mu_1\in\mathbb{R}^{\mu\times N_w}$; (4) randomly row shuffle $\mu_1$ twice to obtain two additional vectors ($\mu_2,\mu_3$), and create new samples with the following linear relations: $\lambda_1=\mu_1+F(\mu_2-\mu_3)$, $\lambda_2=\mu_2+F(\mu_3-\lambda_1)$,  $\lambda_3=\mu_3+F(\lambda_1-\lambda_2)$. Apply uniform crossover with probability $CR$ between each $\lambda_n$ and $\mu_n$, and repeat from (2). The number of evaluations per generation$(\lambda$-samples) is 3 times that of $\mu_1$ which set to 10 (\autoref{tab:parameters_comparing}). Scaling factor $F=0.5$ has shown to result in stable exploration/exploitation behavior in RevDE, with a $CR=0.9$ (from \cite{tomczak2020differential}). 

% \renewcommand{\arraystretch}{0.6} %
\begin{table}[ht!]
    \setlength{\textfloatsep}{0.7\baselineskip plus 0.2\baselineskip minus 0.5\baselineskip}    
    \small
    \caption{\small Hyperparameters of each learning algorithm}
    \label{tab:parameters_comparing}
    \centering
    \renewcommand{\arraystretch}{1}
    \begin{tabular}{l ll}
    \toprule
    \textbf{BO}         & Value & Description \\ \midrule
    Initial sampling    & LHS       & Sampling method\\
    Initial samples     & 50        & Number of samples\\ 
    Learning iterations & 250       & Number of evaluations\\ 
    Kernel type         & Mat\'ern 5/2 & Approximation kernel\\
    Kernel variance     & 1.0       \\ 
    Kernel length       & 0.2       \\ 
    UCB alpha           & 3.0       & Acquisition function weight\\  
    \bottomrule
    \toprule
    \textbf{NIPES}         & Value     & Description \\ \midrule
    $\lambda$           & 10        & initial population \\
    $\sigma$            & 1.0       & Adaption step size\\ 
    Stagnation threshold & $\leq 0.05$ & STD over fitness \\ 
    Stagnation window size & 5 & Number of generations\\
    Novelty: $\mu$      & 1         & Initial ratio\\
    Novelty: $\mu$-decrement & 0.05 &   \\
    Novelty: k          & 15        & Nearest neighbors \\
    Novelty: threshold  & 0.9       & To add to archive\\
    Novelty: probability & 0.4      & To add to archive\\
    \bottomrule
    \toprule
    \textbf{RevDE}         & Value     & Description \\ \midrule
    $\lambda$           & 30        & Population size \\
    $\mu$               & 10        & Top-samples size  \\
    $F$                 & 0.5       & Scaling factor\\ 
    $CR$                & 0.9       & Crossover probability \\ 
    \bottomrule
    \end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Experiments %%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Experiments}

A link to the git repository can be found here\footnote{\url{https://github.com/fudavd/revolve/tree/learning}}. The straightforward way to compare the three learning algorithms is to plug them into our evolutionary robot system and run a good number of repetitions with different random seeds for each combination. However, this would require an extremely long time to conduct. (With 300 learning trials per newborn robot it would take 300 times longer than the pure evolutionary run.) Therefore, we create a test suite of several robot morphologies and test the learning algorithms on the robots in the test suite only. 

As mentioned before, our learning objective is to find a controller that is able to produce the best gait for a given morphology. For this task of gait-learning, we define the robot's fitness as its average speed in a \unit[60]{seconds} evaluation period, i.e. the displacement distance in centimetres per second (\unit[]{cm/s}). 

\begin{equation}\label{eq:fitness_comparing}
    fitness = \sqrt{\Delta x^2+\Delta y^2}/60
\end{equation}

To make a robust assessment of the performance per data set, we carry out $N_{rep}=30$ repetitions with random initialization over all robots in the test suite.

\begin{figure}[ht!]
\includegraphics[width=\textwidth]{figures/ECJ.pdf}
\captionsetup{width=.95\textwidth}\footnotesize
\caption{\label{fig:method1}\small Flow chart describing our method for assessing learner performance on evolvable robots. Top left: the process starts with an M-ER experiment evolved for high speed (i.e. task performance) and novelty (shown as green dots indicating fitness in morphology space). From this experiment we select individuals from the last generation. The collection of robot pictures shows the initial test suite which is hand-picked. Both the last generation and the initial test suite can be represented in morphological space. Right: the test suite is extended by iteratively adding individuals from the last generation based on maximizing novelty. Bottom: the resulting 20 robots are used to compare different learning algorithms.}
\end{figure}

\subsection{Test suite construction}

To construct the test suite for the learning algorithms, we present here a methodology that is described in \autoref{fig:method1}. The test suite is made of two parts: a set of ``viable'' and diverse robots produced an evolutionary process, and a set of hand-picked manually-designed robots. The resulting test suite is displayed below \autoref{fig:test_suite}.

To generate the robots for the first part, the key process is to run evolutionary robotics experiments driven by standard (performance-based) fitness, together with novelty search. The performance-based fitness drive is to produce ''viable'' robots, that is, robots that have functional utility for the given task and are therefore likely to achieve increased performance after learning. The novelty-based drive is to keep up diversity within the population, in order to produce a more diversified test suite for the learning algorithms. 

The second part of the test suite consists of robots hand-picked by the experimenters. It is to allow the inclusion of pre-existing, potentially user-designed robots in the test suite. This part is entirely optional, and can be replaced with an empty set in case one wants to evaluate learning algorithms purely on evolved morphologies.

\begin{figure}[ht!]
\vspace{-1em}
\input{figures/models/models}
\captionsetup{width=.95\textwidth}\footnotesize
\caption{\label{fig:test_suite}\small Test suite of all 20 robots, with number of weights to be optimized in brackets $(N_w)$. The base set consisted of three hand-designed robots (Spider, Gecko and Snake), and two offspring of the Gecko and the Spider (BabyA and BabyB). The remaining set is selected from a population of evolved robots, using novelty search.}
\end{figure}

In our setup, to generate the first part of the test set, we have run an evolutionary algorithm with a population of $500$ individuals, and evolved for speed and novelty by considering as fitness the product of the speed (i.e. task performance) and the mean distance of \textit{k-nearest neighbors} in the morphological space \cite{miras2018effects}. The evolutionary process run for 100 generations. The population of the final generation was used to generate $15$ out of the $20$ robots in the test suite, by maximizing novelty using a pairwise Euclidean distance in morphology space. Specifically we measured morphological distance in 7-dimensions, \textit{size}, \textit{number of joints}, \textit{proportion}, \textit{branching}, \textit{number of limbs}, \textit{coverage}, and \textit{symmetry} from \cite{miras2018search}. The remaining $5$ robots of the test suite were the hand-designed robots presented in~\cite{van2020effects}: Gecko, Spider, and Snake, and two children of Gecko and Spider: BabyA and BabyB.

% \textcolor{red}{To construct a good test suite, we apply a special method to generate an `interesting' set of morphologically different robots. To this end, we interpret `interesting' as advanced in an evolutionary sense, that is, having a high fitness in the given application context. The essence of our method is to evolve a good set of robots for the given task and to build a test suite by iteratively selecting a subset of the evolved robots trying to maximize the diversity. Additionally, we allow that the users manually include 'interesting' robots as per their (subjective) preference. 
%represents a fair cross-section of robots one could encounter during evolution and should expect to perform well on when learning. \autoref{alg:test_suite} shows the steps we took to obtain a dataset (i.e. 20 robots) that represent the different types of morphologies one can encounter during ER. 
%The resulting set of robots is meant to assess learners for ER by being both learnable (i.e. capable to compare performance differences) and diverse (i.e. a good representation of possible morphologies during an ER experiment). 
%Specifically, our method, illustrated in \autoref{fig:method1}, consists of two parts. In the first part, we evolve a population of robots (in our case 100 individuals) based on their speed and novelty. That is, for this evolutionary process, fitness is not simply defined as in \autoref{eq:fitness_comparing}, but by the product of speed and the mean distance of \textit{k-nearest neighbors} in the morphological space \cite{miras2018effects}. In the second part, we create the test suite. First we hand-pick with five robots: our hand-designed Gecko, Spider, and Snake, and two `children' of Gecko and Spider, BabyA and BabyB. (Obviously, seeding the test suite by a set of hand-picked robots is optional; starting with an empty set is also possible.) Subsequently, we construct a test suite of 20 robots by adding 15 from the last generation of robots evolved in the first part. Adding a robot to the test suite is based on maximizing novelty using a pairwise Euclidean distance in morphology space. Specifically we measured morphological distance in 7-dimensions, \textit{size}, \textit{number of joints}, \textit{proportion}, \textit{branching}, \textit{number of limbs}, \textit{coverage}, and \textit{symmetry} from \cite{miras2018search}. The resulting set of 20 robots is shown in \autoref{fig:test_suite}.}


% \begin{algorithm}[!ht]
% \small
%   \caption{\small Pseudo-code generate test-suite}
%   \label{alg:test_suite}
%   \begin{algorithmic}[1]
%     %   \State Initiate $n$ initial samples: $\bm{X}=\left[ \bm{\vec{w}}_1, \bm{\vec{w}}_2, \dots, \bm{\vec{w}}_n \right] $ \Comment{with $n = 50$ pseudo-random samples by LHS}
%     \State \textit{pop}$_0 \longleftarrow$ Initiate $100$ initial individuals
%     \State \textit{gen} = 0
%     \While {\textit{gen} $\le$ \textit{max gen}}  \Comment{Evolve population of robots}
%         \For {\textit{individual} in \textit{pop}}
%             \State \textit{S} $\longleftarrow$ evaluate speed
%             \State \textit{N} $\longleftarrow$ evaluate novelty \hspace{7em}\Comment{\makecell[tr]{mean-distance \textit{k-nearest neighbors} \\ in morpghology space}}
%             \State \textit{F} $\longleftarrow$ \textit{Fitness}(individual) = \textit{S*N}
%         \EndFor
%         \State \textit{pop$_{gen+1}$} $\longrightarrow$ NextGen(selection, crossover, mutation, \textit{pop}$_{gen}$, \textit{F})
%         \State \textit{gen} += 1
%     \EndWhile
%     \State \textit{test-suite} $\longleftarrow {\displaystyle\max_{\textit{individuals}}} \sum_x \sum_{y\neq x} d(x,y) | x,y \leftarrow individuals \in \textrm{\textit{gen}$_{max gen}$}$
%   \end{algorithmic}
% \end{algorithm}



\subsection{Learner performance measures}
To compare the different learning algorithms, we consider three performance indicators: \textit{efficiency}, \textit{efficacy}, and the \textit{robustness to different morphologies}. The assessments are based on inspecting the learning curves for each morphology and each learning algorithm. Additionally, to evaluate the overall performance we will aggregate the results over the morphologies ($N_{rob}=20$) and perform statistical analysis (one-way ANOVA) to see if there is a significant difference between the learning methods (threshold set at $p\leq0.05$). In extension, additional post-hoc analysis between the learning algorithms is done if we find a significant difference. Violations of the assumption on normality and/or equal variance result in taking a different appropriate statistical measure. The specific definitions of the performance indicators are as follows. 
\textit{Efficacy} (Mean Best Fitness, \textbf{MBF}): We measure efficacy by the quality achieved at the end of the learning process (so end-values of \autoref{eq:fitness_comparing}). Since we consider gait-learning here, the quality of a learner is defined by the speed of the robot's best controller. As this measure can be sensitive to `luck', we get more useful statistics by taking the average over 30 different runs. Thus here, the efficacy of a learning method is defined by the mean best fitness averaged over the 30 independent repetitions. 


\textit{Efficiency} (Average number of Evaluations to Solution, \textbf{AES}): Efficiency indicates how quickly the learner finds its best solution. To this end, we use the Average number of Evaluations to Solution metric as defined in \cite{eiben2003introduction}. More than indicating efficiency, AES can provide insight into the maximum number of evaluations required for our learner. If we overestimate the maximum number of evaluations required, then the AES values tend to be (much) lower compared to the evaluation limit set during the experiment.

\textit{Robustness and Consistency}: The robustness of a learner is defined by the differences in performance over various robot morphologies. We can measure this in two different ways, by the Variance of the learners' efficacy (ROB-MBF) or the variance of the learners' efficiency (ROB-AES) calculated over the test suite (i.e. between all morphologies). 
%As our test suite is composed of novelty, ROB-MBF and ROB-AES will indicate how consistently the learner performs in the morphological space.
Significant differences in variance between the groups can be found by conducting an $F$-test of equality of variances (with $\mathrm{df=(2, 57)}$). 

Adding to the above measures, it is interesting to consider the standard deviation of the MBF and AES values over the 30 repetitions on individual robot morphologies (i.e. within all morphologies). We call this property consistency as it provides information on the sensitivity of an algorithm to `luck'. A learner with a small standard deviation is consistent in its performance, while larger values show that it can get lucky or unlucky easily. Similarly to robustness, we distinguish consistency in quality (CON-MBF) and consistency in efficiency (CON-AES).  
%The meaning of the latter measure is less obvious but can serve as an indication of the precision of each end-fitness value per morphology, while the former indicates the variation in performance over different morphologies.

On top of the statistical comparison, we are also interested in the shape of the fitness landscapes. Implementing novelty search in the selection process of our 20 robots resulted in 20 data points spread out over morphological space \cite{miras2018effects}. We approximate the (learner specific) fitness landscape by interpolating the fitness values between each of these data points. The resulting contour-plot shows a fitness estimate (i.e. height) in morphological descriptor space for each learner type (see \autoref{fig:res_contour}). This method provides us an estimate of the dynamic of each of the optimization algorithm with respect to morphological design. To this end, we use a Gaussian mask to calculate a weighted average over each point in morphological space (see \autoref{eq:Gauss_2}). The interpolation works as follows. For each data point $k$ (20 robots) we place a Gaussian ($\mathcal{P}_k(x,y)$) at the corresponding position $(x_k, y_k)$ in morphological space, where dimensions $x$ and $y$ refer any combination of two morphological traits. Subsequently, a weighted average over all fitnesses is taken at each point $x$ and $y$ to create a full contour plot as shown in \autoref{eq:Weight_comparing}. Here, $F_k$ denotes the MBF value of robot $k$.

\begin{equation}\label{eq:Gauss_2}% \small
    \begin{aligned}
        \mathcal{P}_k(x,y) &= \frac{1}{2 \pi \sigma_p^2}exp\Bigg\{-\frac{(x-x_k)^2}{2\sigma_{p}^2} -\frac{(y-y_k)^2}{2\sigma_p^2}\Bigg\}\\
    \end{aligned}
\end{equation}
\begin{equation}\label{eq:Weight_comparing}% \small
    \begin{aligned}
        \mathcal{F}(x,y) &= \frac{\sum_k \mathcal{P}_k(x,y)F_k}{\sum_k \mathcal{P}_k(x,y)}\hphantom{xxxxxxxxXxxlxlxlxl}\\
    \end{aligned}
\end{equation}

This method creates a smooth landscape with a very local effect of each fitness value. The locality is solely dependent on the shape of the Gaussian mask, parameterized with $\sigma=0.1$. It should be noted that this contour plot, at most, provides an insight into the shape of the fitness landscape and does not produce a valuable fitness estimation. We, therefore, present the height of our fitness landscape with minimum-maximum bounds. Nevertheless, the contour plots help us to identify different attractors in morphology space for each learner.

\subsection{Test procedure} 
The three learning algorithms (BO, NIPES, and RevDE) are compared over the 20 robots in our test suite. To make a reliable assessment, we will conduct $30$ different runs on each robot per learner (so $30\times3\times20=1800$ runs in total). Each run consists of $300$ learning trials (i.e. evaluation) and has no other termination condition. At the start of each learning trial, we place a robot in neutral position (all joint angles $\unit[0]{rad}$) centred on a flat horizontal plane with a gravitational pull of $\unit[9.81]{m/s^2}$. We use Gazebo for the simulation with the ODE physics engine and RK4 integration ($\mathrm{dt}=\unit[0.05]{s}$).
%The fitness is used by BO, ES, and DE to improve the controller in the subsequent trials.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Results %%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Results}
All three algorithms could successfully learn good controllers on all morphologies. \autoref{fig:res_curve_com} exhibits the fitness curves for BO in blue, NIPES in orange, and RevDE in dotted gray, showing the mean best fitness values over 30 runs with their respective 95\% confidence intervals ($\pm1.96\times \mathrm{SE}$, Standard Error). A significant difference between the curves can be identified when there is no overlap between the curves. The final MBF values (at generation 300) are shown in \autoref{tab:mbf-end}a. The table is for increasing $N_w$ and shows no search space size dependency of
the MBF for any learner (\autoref{tab:mbf-end}b). In 8 cases there is no significant difference between BO, NIPES and RevDE, for the BabyA, Gecko, Insect, Linkin, Spider, Stingray, WW, and Zappa. NIPES significantly outperforms the other learners on 6 robots (BabyB, Longleg, Penguin, Pentapod, Snake, and Tinlicker), BO only outperforms on Turtle, while RevDE never beats the other two learners with a significant margin. 

\begin{figure*}[ht!]
% \vspace{-em}
\input{figures/result_curve/curve}
% \vspace{-1em}
\captionsetup{width=.95\textwidth}\footnotesize
\caption{\small Maximum speed over time (the number of evaluations) during gait-learning, averaged over 30 independent repetitions. The blue lines show the Bayesian Optimization, orange lines the evolution strategy (NIPES) , and the dotted gray lines the differential evolution (RevDE). The bands indicate the 95\% confidence intervals ($\pm1.96\times\mathrm{SE}$).}
\label{fig:res_curve_com}
        % \vspace{-1em}
\end{figure*}

\begin{figure}[ht]
    \centering
\begin{minipage}{0.99\textwidth}
        \begin{minipage}[t]{0.65\textwidth}
        \centering
        \subfloat[]{
\footnotesize
    \centering
    \begin{tabular}{l c|ccc}
    \multicolumn{2}{l|}{ID \hphantom{1}$N_w$}    & BO & NIPES & RevDE \\ \hline
c&\hphantom{1}6 & 3.88$\pm0.19$ & 4.19$\pm0.44$ & \textbf{4.31} $\pm0.25$ \\
q&11 & 3.08$\pm0.19$ & \underline{\textbf{5.18}}$\pm0.32$ & 3.83 $\pm0.28$ \\ 
o&12 & 3.09$\pm0.22$ & 2.72$\pm0.19$ & \textbf{3.32} $\pm0.32$ \\
e&13 & 4.18$\pm0.17$ & 4.31$\pm0.64$ & \textbf{4.46} $\pm0.36$ \\ 
m&15 & 4.46$\pm0.21$ & \underline{\textbf{6.07}}$\pm1.15$ & 4.67 $\pm0.27$ \\
a&16 & 4.15$\pm0.18$ & \textbf{4.36}$\pm0.25$ & 4.35 $\pm0.35$ \\
s&17 & 3.86$\pm0.25$ & 3.66$\pm0.19$ & \textbf{3.98} $\pm0.26$ \\
n&18 & 4.67$\pm0.34$ & 4.77$\pm0.76$ & \textbf{4.97} $\pm0.55$ \\
p&18 & 5.77$\pm0.33$ & 5.35$\pm0.32$ & \textbf{5.86} $\pm0.41$ \\
k&19 & \textbf{3.19}$\pm0.28$ & 2.59$\pm0.27$ & 3.00 $\pm0.29$ \\
f&20 & 4.67$\pm0.26$ & \textbf{4.90}$\pm0.70$ & 4.67 $\pm0.27$ \\
g&21 & 5.70$\pm0.28$ & 5.58$\pm0.59$ & \textbf{5.75} $\pm0.48$ \\
d&21 & \textbf{4.11}$\pm0.34$ & 3.33$\pm0.22$ & 3.66 $\pm0.37$ \\ 
i&21 & 3.57$\pm0.16$ & \underline{\textbf{4.31}}$\pm0.42$ & 3.31 $\pm0.15$ \\
t&22 & 3.84$\pm0.19$ & 4.05$\pm0.31$ & \textbf{4.05} $\pm0.35$ \\  
j&22 & 3.40$\pm0.18$ & \underline{\textbf{5.93}}$\pm0.73$ & 3.08 $\pm0.22$ \\
b&22 & 4.36$\pm0.25$ & \underline{\textbf{5.15}}$\pm0.59$ & 3.75 $\pm0.23$ \\
h&24 & 4.13$\pm0.19$ & \underline{\textbf{4.82}}$\pm0.37$ & 3.94 $\pm0.28$ \\
l&25 & \textbf{4.65}$\pm0.23$ & 4.11$\pm0.24$ & 4.39 $\pm0.30$ \\
r&28 & \underline{\textbf{3.42}}$\pm0.27$ & 2.73$\pm0.18$ & 2.98 $\pm0.12$ \\ \hline
\multicolumn{2}{l|}{- \hphantom{1}18.55} & 4.11$\pm0.73$  & \textbf{4.40}$\pm1.0$\hphantom{0} & 4.12$\pm0.77$\\
    \end{tabular}
    }
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.3\textwidth}
        \centering
        \subfloat[]{\includegraphics[width=\textwidth]{figures/N_w.pdf}}
    \end{minipage}
    \hfill
\end{minipage}
\captionsetup{width=.95\textwidth}\footnotesize
    \caption{\small (a) Mean Best Fitness (MBF$\pm1.96\times\mathrm{SE}$) per morphology for each learner ($N_{rep}=30$). Morphologies are identified by the letters used in Figure \ref{fig:test_suite} and sorted in ascending order of the number of weights of their controller, $N_w$. For each morphology, the best result is indicated with \textbf{boldface} while \underline{underline} indicates significantly better performance compared to the other learners. The last row shows the aggregated MBF result for each learner over all morphologies ($N_{rob} = 20$). (b) represents the same data visually per learner. The results show that none of the learners is dependent on the search space size ($N_w$) with respect to MBF.}
    \label{tab:mbf-end}
\end{figure}

Based on our data we can identify the `champions', i.e., the fastest robots in our test suite over all runs and repetitions. Considering the overall top speed the Snake is the best (\unit[17.76]{cm/s} found by NIPES), followed by the Insect (\unit[14.71]{cm/s} found by NIPES), and the Spider (\unit[14.33]{cm/s} found by NIPES). Considering the average best speed (i.e. MBF results), the best robots are the Snake (\unit[6.07]{cm/s} with NIPES), Pentapod (\unit[5.93]{cm/s} with NIPES), and Spider (\unit[5.86]{cm/s} with RevDE). 

%Bases on our data we can identify the `champions', i.e., the fastest robots in our test suite. Considering the top speed the Snake is the fastest (\unit[17.76]{cm/s} found by NIPES), followed by the Insect (\unit[14.71]{cm/s} found by NIPES), and the Spider (\unit[14.33]{cm/s} found by NIPES). Considering MBF results, the best robots are the Snake (\unit[6.07]{cm/s} with NIPES), Pentapod (\unit[5.93]{cm/s} with NIPES), and Spider (\unit[5.86]{cm/s} with RevDE). 


Following up the obtained efficacy results from \autoref{tab:mbf-end}, we can now produce our fitness landscapes (\autoref{fig:res_contour}). We only present a single instance of the possible morphological measure combinations, i.e. showing the fitness landscape as a function of \textit{joints} and \textit{symmetry}. These morphological measures have been used before to produce fitness landscapes \cite{miras2018effects, de2020influences}, and show interesting differences between the learners. As mentioned before, the height in these plots only indicates possible attractors. Here, we can see that overall BO and RevDE seem to have similar attractors in morphological space, meaning that these learners perform well on similar types of morphologies. In comparison, NIPES seems to have a much larger basin of attraction and a deeper region of lower fitnesses. Furthermore, differences between the lowest and the highest point are more pronounced in NIPES compared to BO and RevDE, which correspond to the results from the fitness curves. Lastly, the shape of the fitness landscape in NIPES hints to a possible bias for morphologies with many joints. This could be an unwanted property for the implementation of learning.

\begin{figure}[ht]
\input{figures/result_contour/contour}
\captionsetup{width=.95\textwidth}\footnotesize
\caption{\label{fig:res_contour}\small Fitness landscape based on symmetry and number of joints for each learner BO, NIPES and RevDE. Fitnesses are interpolated using a weighted gaussian mask. Here we see BO and RevDE produce similar landscapes while NIPES find a different maximum (at joints: 0.8, symmetry: 0.45). Also the strong differences between maximum and minimum indicate a stronger biases towards certain morphologies in NIPES, when used during M-ER.}
\end{figure}

We present a numerical summary of the results on the learner performance measures in \autoref{tab:res_DATA}. Assumptions on normality were met for all condition and measure combinations. Regarding \textit{efficacy}, we can see that the overall differences in the mean best fitness are not significant ($p>0.05$). On the measure of \textit{efficiency}, we did find significantly different results between the learners. It should be noted that the assumption of equal variances was violated here (visible in the significant difference of ROB-AES). Therefore, a more conservative Kruskal-Wallis test was performed to measure differences between the mean AES. With post-hoc analysis (using \textit{Mann–Whitney U}-test with Bonferroni correction), NIPES turns out to be slower than the other methods, since its AES values are significantly higher compared to both BO ($p<0.001$) and RevDE ($p<0.01$). In contrast, the AES of the BO and RevDE do not differ significantly from one another. 

\begin{center}
\begin{table}[ht]\small
% \scriptsize
    % \setlength{\textfloatsep}{0.7\baselineskip plus 0.2\baselineskip minus 0.5\baselineskip}    
\captionsetup{width=.95\textwidth}
    \caption{\footnotesize Efficacy (MBF), efficiency (AES), robustness (ROB-MBF and ROB-AES), and consistency (CON-MBF and CON-AES) per learning algorithm over the test suite of $N_{rob}=20$ different morphologies $\pm\mathrm{STD}$. The last column show the $p$-values of each test, $F$-test for ROB, and ANOVA for the other metrics. The * indicates the use of Kruskal–Wallis test. Best values are indicated by \textbf{bold} font (it should be noted that best and second were only significantly different for the CON-AES metric)
    \label{tab:res_DATA}}
    \centering
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{l cccr}
    \toprule
    Measure                     & BO        & NIPES & RevDE &$p$-value  \\ \midrule
    MBF     & 4.11$\pm0.73$  & \textbf{4.40}$\pm1.0$\hphantom{0} & 4.12$\pm0.77$ & 0.48 \\
    AES                         & \textbf{149}$\pm10$\hphantom{0} & 171$\pm21$\hphantom{0} & 151$\pm13$\hphantom{0} & *$\leq$0.001 \\
    ROB-MBF         & \textbf{0.54} & 1.0 & 0.63 & 0.48 \\
    ROB-AES                         & \textbf{96} &456 &173 & $\leq$0.001 \\
    CON-MBF    & \textbf{0.66}$\pm0.16$   & 1.24$\pm0.70$ & 0.86$\pm0.28$ & $\leq$0.001\\
    CON-AES    & 83$\pm9$\hphantom{0} & \textbf{75}$\pm9$\hphantom{0} & 85$\pm6$\hphantom{0} & $\leq$0.001\\
    \bottomrule
    \end{tabular}
\end{table}
\end{center}

Considering \textit{robustness} we can distinguish the (in)sensitivity of the efficiency and the efficacy of the learners with respect to the different morphologies. The ROB-MBF show that the variance between the efficacy of learners does not differ significantly ($p>0.05$). In contrast, the robustness of the efficiency (ROB-AES) did differ significantly between the different learners ($p<0.001$). A closer inspection of this result reveals that ROB-AES in NIPES is significantly higher compared to BO ($p<0.001$) and RevDE ($p<0.05$), while BO and RevDE did not differ significantly. This indicates that the efficiency of NIPES varies a lot between different morphologies.

In contrast to the results on robustness to different morphologies, differences between the consistency in solution quality are significant. This difference in results for ROB-MBF and CON-MBF show that both measures do represent distinct properties of the learners. In particular, for NIPES the CON-MBF results show statistically significant differences ($p<0.001$) indicating that this learner is more subject to `luck' than BO ($p<0.001$) and RevDE ($p<0.001$). On a given robot the maximum speed can greatly vary for NIPES. This is not surprising taking into account that it is a greedy optimizer that can get trapped in local optima. The low budget of 300 trials is apparently not enough to compensate for this effect by restarts. Furthermore, CON-AES shows that NIPES varies significantly compared to BO ($p<0.01$) and RevDE ($p<0.001$). This shows that the variation in end-solution-time between runs within the same morphology is lower. 

These results provide important insights into the overall quality of the learners. The data show differences in terms of sample efficiency: BO and RevDE deliver the same solution quality (walking speed for the robot, MBF) with fewer evaluations than NIPES (based on AES). Additionally, the results provide further insights regarding robustness and consistency: 1) A full-fledged M-ER experiment, evolving both morphology and controller with NIPES as a learner, will perform more inconsistently (i.e. luck-based) than an M-ER run with BO or RevDE as a learner. The inconsistency is amplified by the fact that a learner is applied only once to a 'newborn' robot, without the repetitions runs per morphology as done in this study. 2) Using 30 repetitions per morphology we successfully mitigated the effect of `luckiness' in NIPES and got a good estimate of the true MBF. Without these repetitions we would probably see significant differences in variance as well (ROB-MBF). Furthermore, NIPES is less robust than the other two algorithms, because its efficiency varies more over different robot morphologies. 


\section{Discussion}
The main goal of our work is to present a practicable way of analysing and comparing different algorithms used for learning during an M-ER experiment. Our method enables a comparison without the high costs of running a full M-ER experiment with learning. For example, consider a scenario where individual learning within a population of evolving robots in a new environment could be useful. To make an informed choice of a learning algorithm, we can follow the steps outlined in this work to create a data set and analyze the performance of the available options (see \autoref{fig:method1}). An advantage of our method is that this can be fully adjusted according to specific needs. We could alter the evolved population in the first part, where we change the fitness criteria, morphological traits, novelty measure or even combine different runs/generations. We can hand-pick different robots, or leave the initial set empty. We can apply the same analysis presented here using consistency and robustness, or for example, split our data set for hyper-parameter tuning using k-folds.

Let us quickly summarize the results of our learner comparison. We found that
NIPES outperforms BO and RevDE on 6 morphologies in terms of MBF. Nevertheless, NIPES does not perform significantly better on the whole test (in fact, none of the algorithms did). The potential to be superior on specific morphologies but not overall, indicates a chance for a morphological bias --or morphological dependency-- within NIPES. This is also supported by NIPES' lower robustness, i.e. greater performance differences between morphologies. Additionally, this superiority is unreliable, because NIPES is significantly less consistent or more luck-based (i.e. high variation within morphologies). Given the size of the significant differences it can therefore be questioned whether MBF is the best indicator of learner `performance' within the context of a broader evolutionary experiment. In a single learning only context, it is possible to re-start NIPES until a lucky run is found (provided that NIPES is positively biased for the specific robot at hand).  Unfortunately, within M-ER a morphological bias inside a learner is likely disadvantageous, and multiple learning runs on a robot are very costly.

Both BO and RevDE are comparably more efficient than NIPES. BO outperforms RevDE on one morphology but is also not statistically different in terms of performance with respect to RevDE. Addidionally, their significantly higher robustness scores indicate a more general performance in terms of morphological search space. In terms of wall-clock time, the BO experiments took the longest ~15 minutes compared to NIPES 10 minutes, and RevDE 8 minutes. But we consider this metric irrelevant in terms of the expected application within a 5 hour learning experiment.

Recall that the algorithms used in our experiments are meant to be used in combination with morphological robot evolution as learning methods in newborn robots. One of the contributions of this paper is the methodology to compare such learning algorithms without running the full-blown experiments, meaning evolution with learning. The validity of this methodology is motivated by three ideas. Firstly, we can show differences between learners with several specific robots as test cases. The straightforward approach to compose an adequate test suite would be to select a ``representative'' set of robots. However, it is not clear what ``representative'' should mean in our context. This motivates the second idea: we chose to create a set of robots that is well-spread in the space of possible morphologies and we define that space through several quantifiable morphological traits. In this paper we used seven traits, leading to a 7-dimensional space with a natural distance measure. Lastly, each individual in the test set should have enough potential to learn. Comparison is only informative when learners can differentiate from one another. We achieved this by selecting from a previously evolved population.

It is important to note that changing the design space of the robots changes the applicable morphological traits. For instance, if the design allows wheels, then the number of wheels of a robot is an appropriate trait that defines a new dimension of the morphological space. In general, it is not known what traits are relevant for the working of the learning algorithms. For example, the size of a robot may be important and the proportion of its length and width irrelevant. Thus, our recommendation is to use all possible traits until more research on the long term delivers insights to select more cleverly. 

 Our view on applicable learning algorithms is very permissive: we consider any generate-and-test style search algorithm applicable, if only it can search in the space of possible controller configurations. Obviously, this depends on the given controller architecture and the learnable components therein, but in general, the number of options is large, including, for instance, Bayesian Optimization (that we considered here), Reinforcement Learning and Simulated Annealing (that we did not), and all kinds of evolutionary algorithms (of which we studied two). Let us briefly note that, if the choice of controller learning algorithm is also evolutionary, then great care needs to be taken to avoid confusion with the outer evolutionary method for full robot design (both body and brain). For comprehensiveness of the discussion, we shall not discuss this in detail here. Let us only note that it is useful to distinguish the outer evolutionary loop, where new individuals are new robots with a body and a brain and the inner evolutionary loop (the learning method), where new individuals are new brains for the given robot body.

A given test suite of robots with a number of learning algorithms can be compared by the usual metrics regarding efficiency, efficacy, and robustness. Rooted in our application, there are two very important measures: \emph{efficiency} because infant robots should optimize their controllers quickly after birth; and \emph{robustness}, because evolution (the outer loop) can produce very different robots and the learner should work well on all of them. The current study is the first of its kind into this, which means that we should be careful with generalizations. However, our data suggest that finding robust learners is not too hard and that 300 learning trials --probably even 200-- can be enough to achieve decent performance. Additionally, in recent studies it was found that the learning potential of evolved robots, the so-called learning delta, is growing throughout evolution \cite{miras2020evolving, le2022morpho, luo2022effects}. If this turns out to be a general effect, then the maximum number of learning trials could even be lowered. The obvious caveat is that we only considered one task in a simple environment. More complex tasks and environments may require more steps and may induce more pronounced differences among learning algorithms. 


\section{Concluding remarks}

Let us conclude this paper with elaborating on the greater perspective, beyond the specific technical results. As explained in the beginning, our motivational scenario concerns a system where  morphologies and controllers of (modular) robots evolve simultaneously. In this scenario, newborn robots must learn to adjust their inherited controller to their inherited morphology quickly after birth, cf.~\cite{eiben2013triangle, eiben2020if}. This context implies two specific challenges for a learning algorithm. Firstly, the lack of priors regarding the morphology (because we do not know what robot bodies evolution will produce) and secondly, the need for exceptional sample efficiency (because allowing $N$ learning trials will multiply the total number of evaluations by $N$). Obviously, these challenges are important in general, not only in the context of evolutionary robotics, because an algorithm that works without priors is widely applicable and an algorithm that is sample efficient reduces the time needed for development and optimization. This leads to a generic research question: What good algorithms are there for efficiently optimizing the controller of a (modular) robot whose morphology is not known in advance? This paper delivers a contribution to the field of adaptive robotics by explicitly identifying this combination of challenges and the implied research question. Furthermore, we provide an answer to this question by introducing and employing a new methodology.

The methodological challenge we address is rooted in the computational costs of comparing learning methods by running them in the intended application, a system with evolving robots. For example, allowing 100 learning trials per newborn robot sounds as a modest learning budget, but increasing the number of evaluations by 100 can be a show-stopper. (In a worst case scenario, an evolutionary experiment of two weeks without learning can become an experiment of 200 weeks with learning.) Our contribution to this end is the introduction of a new methodology. The essence of this approach is the usage of a relatively small test suite of robots with a high fitness (produced by evolution) and diversity (achieved by the selection process) as shown in Figure \ref{fig:method1}.   

Our study also illustrated new assessment criteria for comparing algorithms for robot learning: robustness and consistency. These go beyond the usual suspects of efficiency and efficacy, and bear special relevance in the context of combining morphological evolution with learning in infant robots.

The use of morphological descriptors, in particular, plotting and comparing the performance of learners in the multi-dimensional space they span, provides a possibility to intelligently change the learning algorithm during evolution. Specifically, if the evolving population enters a region in the morphological search space where the actually used learner is known to be inferior to another one, then this learner can be dropped and replaced by a better one. For example, learner A could be known to be superior for wheeled robots and learner B for robots with legs. Then the system can switch to using learner B instead of learner A if wheeled robots become extinct during the M-ER process and legged robots dominate the population. In a more sophisticated case, the learner can be individually chosen for each newborn robot, based on its morphology.


In summary, we argue that the development of new robot learning algorithms would benefit from using diverse test suites of many morphologies, instead of extensive learning on one specific robot only.



%In summary, we argue that --in contrast to most work in robot learning-- our approach based on efficient training on many morphologies instead of extensive learning on one provides better insights when assessing new robot learning algorithms.



%In this paper, we investigated learning methods to be applied in newborn robots within evolutionary robot systems, where morphologies and controllers evolve simultaneously. We conducted an empirical comparison of three methods, Bayesian Optimization, an Evolution Strategy NIPES and a Differential Evolution RevDE on a test suite of 20 robots for the task of gait-learning. The results show that BO and RevDE can deliver the same solution quality (walking speed for the robot) with fewer evaluations than NIPES. Furthermore, NIPES is less robust than the other two algorithms, because its performance varies more over different robot morphologies. 

% \section{Acknowledgements}
%   This work is supported by the Technology Innovation Institute, UAE.

==> 2/Loader.tex <==

% \usepackage{booktabs} % For formal tables
% % Language and font encodings
% \usepackage[english]{babel}
% \usepackage[utf8x]{inputenc}
% \usepackage[T1]{fontenc}
% \usepackage{floatrow}
% \usepackage{siunitx}
% \usepackage{adjustbox}
% \usepackage{subcaption}
% \usepackage{blindtext}
% \usepackage{multirow}
% \usepackage{tabularx}
% \usepackage{array}
% \usepackage{graphicx}
% \usepackage{color, colortbl}
% \usepackage{tikz}
% \usepackage{amsmath}
% \DeclareMathOperator{\taninv}{tan^{-1}}
% \usepackage{amssymb}
% \usepackage{bm}
% \usepackage{units}
% % \usetikzlibrary{positioning}
% %% Sets page size and mareality gapins

% %% Useful packages
% \usepackage{amsmath}
% \usepackage{graphicx}
% % \usepackage[colorinlistoftodos]{todonotes}
% \usepackage[bookmarks=false]{hyperref}
% \usepackage{makecell}
% \usepackage{soul}


% % Make Figure Great Again
%     \usepackage{float} % [H]
%     \usepackage{wrapfig} % text wrapping
%     \usepackage{caption} % \caption
%     \usepackage{subcaption} % \subcaption
%     \usepackage{graphicx} % \includegraphics
%     \usepackage[font=small,labelfont=bf]{caption}

%     % packages for Flow diagrams
%     \usepackage{tikz}
%     \usetikzlibrary{shapes.geometric, arrows, positioning, automata}
%     \tikzstyle{process} = [rectangle, minimum width=2cm, minimum height=1cm, text centered, draw=black, fill=white!30]
%     \tikzstyle{sum} = \tikzstyle{sum} = [draw, circle, minimum size=.5cm]
%     \tikzstyle{arrow} = [thick,->,>=stealth]
%     \def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;}


% % Make Tables Great Again
%     \usepackage{pdflscape} % enable landscape mode
%     \usepackage{multirow} % multirow
%     \usepackage{longtable} % multipage
%     \usepackage{array} % fixed width
%     \renewcommand{\arraystretch}{1.5}
%     \usepackage{booktabs} % top/mid/bottomrule
%     \usepackage{makecell} % tableception
%     \usepackage{diagbox} % \diagbox{}{}
%     \usepackage{rotating}
%     % \setlength{\columnsep}{0.6cm}

% % correct bad hyphenation here
% \hyphenation{op-tical net-works semi-conduc-tor}

\begin{document}


% The elephant in the room for evolutionary robotics is the reality gap. In history of the field several studies investigated this phenomenon on fixed robot morphologies and proposed ways to circumvent it. The main objective of this paper is to understand the reality gap in a wider context: a system where both morphologies and controllers are evolved. To this end, we construct a test suite of robots with various morphologies and evolve their controllers for an effective gait. Comparing the simulated and the real-world  performance of evolved controllers sampled in different  generations during the evolutionary process for all robots we gain new insights into the factors that influence the reality gap.

The elephant in the room for evolutionary robotics is the reality gap. In the history of the field, several studies investigated this phenomenon on fixed robot morphologies where only the controllers evolved. This paper addresses the reality gap in a wider context, in a system where both morphologies and controllers evolve. In this context the morphology of the robots becomes a variable with a currently unknown influence. To examine this influence, we construct a test suite of robots with various morphologies and evolve their controllers for an effective gait. Comparing the simulated and the real-world performance of evolved controllers sampled at different generations during the evolutionary process, we gain new insights into the factors that influence the reality gap.

\input{Main.tex}

\input{Appendix.tex}
% that's all folks
\end{document}




==> 2/Main.tex <==
\section{Introduction}
% \normalsize
Evolutionary robotics (ER) is a research area with an attractive proposition: to design robots for a given task and environment one can use an evolutionary algorithm that will `breed' a good design with less user effort than traditional engineering approaches \cite{nolfi2000evolutionary, doncieux2015evolutionary}.
%Importantly, this holds for both the morphologies (bodies) and the controllers (brains) of the robots. 
While, in principle, this is indeed possible, in practice the evolutionary approach is limited by the so-called reality gap, the phenomenon that robots evolved in computer simulations only work well in computer simulations \cite{jakobi1995noise, jakobi1997evolutionary,mouret201720}. The reality gap problem is rooted in the fact that the simulated world can deviate from the real world in crucial aspects because computer models and simulators are based on abstractions and approximations. Additionally, an evolutionary optimizer can and will exploit any feature in the simulated world, including the badly modeled ones. This implies that the performance of a solution evolved in simulation decreases once it is transferred to a real robot. The performance difference --the reality gap-- can be significant and observations and conclusions about system behavior may be mere artefacts of the simulator.    

The ER research community has spent considerable effort in mitigating the reality gap problem. (See the next section for an overview). Typically, these studies concern the design of a good brain (controller) for a fixed robot body (morphology). In this context, evolution applies only to the `brain space' which contains all possible robot controllers for the given robot. Thus, populations consist of robot controllers that undergo selection and reproduction until the fitness (task performance) is sufficient, or the maximum number of generations is reached.
%computational budget is exhausted. 

This paper addresses the reality gap in a wider context, in a system where morphologies and controllers evolve simultaneously. Our aim is to gain new insights into the factors that influence the reality gap in such a system. In particular, we address two research questions. Firstly, how does the reality gap depend on the robot morphologies? 
% For instance, will smaller robots with fewer actuators suffer less than bigger robots with many actuators? 
Secondly, how does the reality gap change during an evolutionary run? %Specifically, we consider the evolution of a good controller on a given body. 
We expect that solutions produced in later generations during the evolutionary process exploit more of the simulator's specific details, which increases the reality gap. Thus, our working hypothesis is that the reality gap increases over the course of an evolutionary run. 
%Regarding the second aspect, the impact of the robot morphologies, we do not have a hypothesis, but hope to detect some relationship between the robot morphologies and the reality gap. 

%In particular, we are interested in the dynamics of the reality gap during an evolutionary run in which both morphology and controller are evolved. Furthermore, 
% \vspace{-1em}
\section{Related work}
% \vspace{-0.5em}
Research into the reality gap has a history of more than 20 years in ER \cite{mouret201720}. Based on different ways to reduce the reality gap, \cite{ligot2020simulation} suggested to split the literature into four distinct categories, as shown in \autoref{tab:reality_class}.

\begin{table}[ht]
% \setlength{\tabcolsep}{20pt}
\centering
\renewcommand{\arraystretch}{1.25}
\input{figures/RG_class}
    \captionof{table}{\label{tab:reality_class}
        Classification of related work about the reality gap. Adapted and extended from \cite{ligot2020simulation}.}
\end{table}
% \vspace{-1em}
Reducing the reality gap during the simulation process (top left \autoref{tab:reality_class}) aims to improve the simulator in such a way that the predicted behavior mimics real behavior more closely. This can be achieved by continuously integrating real data to the simulator \cite{miglino1995evolving}, adding noise on sensor level \cite{jakobi1995noise}, or by learning the model of the robot in its environment online \cite{bongard2004once, zagal2004back}.

Improving the robustness of the results found in simulation (bottom left \autoref{tab:reality_class}) attempts to reduce the impact of the reality gap on the real robot. Here, it is (rightfully) assumed that the reality gap is unavoidable (i.e. errors are inherent in simulators) and can only be reduced so much. Robustness of solutions can be increased by implementing adaptive feedback control \cite{van2020effects}, developing robots within a variety of different environments \cite{boeing2012leveraging}, or randomly perturbing environmental parameters like gravity during development \cite{jakobi1997evolutionary, jakobi1998minimal,tobin2017domain}.

Another approach aims at improving the designing process and not on the simulator itself (for example, search methods, search space adaptations, genotypical expression \textit{etc.}). Here, exploitation is prevented by improving the solutions proposed during evolution. With this intend, improving the robustness of design (bottom right \autoref{tab:reality_class}) is based on the idea that, in the end, all optimizers will suffer from the reality gap if the search space is expressive enough to exploit the flaws in the simulator \cite{rosser2020sim2real}. To counteract this exploitation, we can try to only exploit the general physical dynamics of the simulator and make our designing process more robust by limiting the amount of over-fitting possible \cite{hasselmann2021empirical}. Proposed solutions lie in the automatic tuning of hyper-parameters \cite{floreano1996evolution, urzelai2000evolutionary, floreano2001evolution}, and slowly increasing the representational power of the search space \cite{francesca2014automode}. Additionally, a proper search space design could prevent sources of the reality gap like breaking of the robot \cite{10.3389/frobt.2021.699814}, or split optimization in different task-independent requirements to reduce the overall exploitation in the simulator \cite{10.3389/frobt.2021.684304}. 

At last, this paper positions itself in the category that aims to prevent the exploitation in the simulator (top right \autoref{tab:reality_class}). Work in this category focuses on the dependency of the reality gap to the search space to pre-emptively filter out bad designs based on this relation. This will increases the effective budget (ratio of meaningful evaluations) of the optimizer as we don't consider badly transferable solutions to test (i.e. large reality gap). This approach differs from incorporating the reality gap in the fitness, as it does not directly change the optimizers search behavior but rather dismisses bad designs before considering testing them in the real world. Incorporation of the reality gap in the fitness would not reduce the effective budget but make the search more robust against exploitation (which falls under the previous category). A clear example of this category is a paper by \cite{koos2012transferability} that constrained the designing process with a model that estimated the size of the reality gap. To our knowledge this category has only been covered scarcely in literature. With our work, we hope to contribute to this research with some useful heuristics to help reduce the reality gap in ER.

\section{System description}

We conduct this study in a simple lab environment with a solid floor without obstacles where robots are evolved for the task of efficient locomotion, also known as gait learning.  

\subsection{Robot morphologies}
Our robots consist of modules that are based on the RoboGen framework \cite{auerbach2014robogen}. A modular design space has the advantage of rapid real-world prototyping through pre-fabrication of 3D printed modules and off-the-shelf components, as shown in other frameworks as well \cite{pollack2000golem, veenstra2017evolution, faina2013edhmor}. We altered the original Robogen module designs to prevent breaking, improve servomotors, and allow feedback control in the near future. This new design consist of three components: a core component (\unit[$9\times9\times6$]{cm}, \unit[250]{gr}), brick components (\unit[$6\times6\times6$]{cm}, \unit[30]{gr}), and active hinges (\unit[$12\times6\times6$]{cm}, \unit[69]{gr}). The core component is a container with a micro-controller (Raspberry Pi 3B+\footnote{\url{https://www.raspberrypi.org/products/raspberry-pi-3-model-b-plus/}}), a custom designed bridge to our servomotors (as detailed in \cite{lan2020learning}) and a battery (LiPO, 3.7V \unit[7800]{mAh}). It has four attachment slots on its lateral faces to which other modules can be attached via screws. The brick component is a smaller cube with similar attachment points on its lateral sides as well. The active hinge component is a joint actuated by a servomotor (Tower Pro MG996R, full specs here\footnote{\url{https://www.towerpro.com.tw/product/mg996r/}}) with an attachment point on both ends. We describe a robot's body plan using a tree structure with the core module as the root node.

\subsection{Robot controllers} 
%In this study, we investigate the reality gap for the task of gait-learning. The robots learn this behavior by optimizing the weights in 
The robots in this study are controlled by a network of interconnected Central Pattern Generators (CPGs), where each CPG drives one of the servo motors.  In short, CPGs are pairs of artificial neurons ($x_i$,$y_i$) that reciprocally inhibit and excite each other to produce oscillatory behavior \cite{ijspeert2008central} and make the robot locomote. CPG controllers have shown to learn good gaits efficiently \cite{korkmaz2019locomotion} and were tested on our modular robots before in the real world \cite{lan2020learning}.


Let $i$ denote the specific joint that is associated with a single CPG. The change of a neuron state is calculated by multiplying the current state of the opposite neuron with a weight ($w$), shown in \autoref{fig:CPG_model_RG}a. The weights $w_{x_iy_i}$ and $w_{y_ix_i}$ represent a connection between each neuron pair. An output neuron $out_i$ is coupled to the $x$-neuron with an strength $w_{x_io_i}$. The output of $out_i$ will serve as the input command for the servomotor in the specific joint. In our case, we picked a tangent hyperbolic activation function as our output neuron to bound the motor input between [-1,1] rad. 


\begin{figure}[ht!]
\centering
\begin{minipage}[c]{\linewidth}

        \begin{minipage}[t]{0.45\linewidth}
            \centering
            \subfloat[CPG]{\input{figures/CPG}}
        \end{minipage}
        \quad
        \begin{minipage}[t]{0.35\linewidth}
            \centering
            \subfloat[CPG network]{\input{figures/CPG_net}}
        \end{minipage}
        % \hfill
            % \includegraphics[width=0.6\linewidth, ,keepaspectratio]{Figures/CPG_model.png}
           \caption{\textbf{a}) A single CPG. \textbf{b}) The CPG network for the Spider robot, containing 8 CPGs (numbers) with 10 connections (blue lines between the CPGs). See Figure \ref{fig:models_s}e and Figure \ref{fig:models_r}e for the images of the simulated and the real robot.}\label{fig:CPG_model_RG}
\end{minipage}
\end{figure}

To enable more complex output patterns, CPG connections between neighboring joints are allowed, see \autoref{fig:CPG_model_RG}b. We define neighboring joints at joint $i$ as the set ($\mathcal{N}_i$) of each joint $j$ positioned within a Manhattan distance of 2 modules. The resulting differential equations of the CPG network is shown in \autoref{eq:ODE_CPG_RG}. Connections between neighboring joints $j$ are denoted as $w_{x_jx_i}$.
        \vspace{-.5em}
        \begin{align}\label{eq:ODE_CPG_RG}
            % \begin{split}
                \Dot{x}_i = w_{y_ix_i}y_i + \sum_{j \in \mathcal{N}_i} x_{j} w_{x_jx_i} &&\Dot{y}_i = w_{x_iy_i}x_i
            % \end{split}
        \end{align}
        
By changing the weights of the CPGs, we can improve our controller for the task of gait-learning. To simplify the search space, the following relations are imposed between the weights: $w_{x_iy_i} = -w_{y_ix_i}$; $ w_{x_jx_i} = -w_{x_ix_j}$; $w_{x_io_i} = 1$. At the start of each learning trial all neuron states will be set to a predefined value $(x,y)=\left(-\frac{1}{\sqrt{2}},\frac{1}{\sqrt{2}}\right)$. The sampling period of the controller is $\unit[0.125]{s}$. The same controller is compiled on the micro-controller to transfer the learned behavior to the real world. Motor commands are thus computed on-board after a `start command' is sent from our laptop to the robot.
        
\subsection{Learning method}
We optimize the CPG-network's weights in simulation with an EA called Reversible Differential Evolution (RevDE) \cite{tomczak2020differential}. In general, differential evolution tackles the optimization problem by producing new candidate solutions with the current population and a set of perturbations on their genotype. These perturbations are calculated using two genotype vectors that are obtained by randomly shuffling the current population. The advantage of this approach is the straightforward implementation and the model agnostic nature of the perturbations. Unfortunately, traditional differential evolution can suffer from a small population size by losing diversity rather quickly.

RevDE solves this problem by applying a special set of linearly reversible transformation to maintain a high sample spread \cite{tomczak2020differential}. The algorithm works as follows: (1) initialize a population with $\lambda$-samples (2) evaluate the fitness over all $\lambda$-samples; (3) perform selection over the top samples to obtain the genotype vector $\mu_1$; (4) randomly shuffle $\mu_1$ twice to obtain vectors ($\mu_2,\mu_3$), and create new samples as follows: $\lambda_1=\mu_1+F(\mu_2-\mu_3)$, $\lambda_2=\mu_2+F(\mu_3-\lambda_1)$,  $\lambda_3=\mu_3+F(\lambda_1-\lambda_2)$. Apply uniform crossover with probability $CR$ between each $\lambda_n$ and $\mu_n$, and repeat from (2). The number of evaluations per generation$(\lambda$-samples) is 3 times that of the number of individuals selected (size of each $\mu$) which set to 20 (\autoref{tab:parameters_IMC}). Scaling factor $F=0.5$ has shown to result in stable exploration/exploitation behavior in RevDE, with a $CR=0.9$ (from \cite{tomczak2020differential}). 

\begin{table}[ht!]
    \setlength{\textfloatsep}{0.7\baselineskip plus 0.2\baselineskip minus 0.5\baselineskip}    
    \small
    \captionof{table}{\label{tab:parameters_IMC}Hyperparameters of the RevDE learner.}
    \centering
    \renewcommand{\arraystretch}{1}
    \begin{tabular}{l cl}
    \toprule
    Parameter         & Value     & Description \\ \midrule
    Generations        & 100       &\\
    $\lambda$           & 60        & Population size \\
    $\mu$               & 20        & Top-samples size  \\
    $F$                 & 0.5       & Scaling factor\\ 
    $CR$                & 0.9       & Crossover probability \\ 
    \bottomrule
    \end{tabular}
\end{table}

% \vspace{-1.5em}
\section{Experiments}
\label{sec:exp}
Our aim is to get new insights into the dynamics of the reality gap in evolutionary robot systems where both morphologies and controllers undergo evolution. Unfortunately, morphological evolution in the real world is very time consuming since it requires that every new robot offspring is physically built and tested. A full blown experiment would require constructing and testing thousands of robots in the real world and is therefore currently infeasible. As a pragmatic workaround we decided to use a limited number of robots and study the process of evolving their controllers. Importantly, these robots are selected from the morphology space of an evolutionary robot system, hence they represent different options within the same species.

%We test the overall best performing controller, and the median controller of the 31 runs' best-controller so far at every $10^{th}$ generation. In total we test 11 controllers in 6 different robot morphologies \autoref{fig:models}. 
% \vspace{-.5em}
\subsection{Test suite}
The robots in this test suite were selected from 1000 previously evolved individuals (multiple runs, \cite{miras2018effects}) using novelty search. Novelty search was based on seven morphological traits detailed further in \cite{miras2018search}: \textit{size}, \textit{number of joints}, \textit{proportion}, \textit{branching}, \textit{number of limbs}, \textit{coverage}, and \textit{symmetry}. The resulting test suite is shown in \autoref{fig:models_s}.

The rationale behind the creation of the test suite was as follows: 1) Selecting morphologies from a collection of previous runs ensures that the selected robot morphologies are viable candidates for gait learning. Non-viable morphologies (in terms of learning) are by default unsuitable for investigating the reality gap as a function of evolutionary dynamics. 2) The use of novelty search for the selection procedure provides a proxy for the wide variety of morphologies that are to be expected in a fully (both controller and morphology) evolutionary system. Reducing the chance of a bias for a specific morphology will provide a better insight in its dependency on the search space. Selecting morphologies by hand would have introduced a possible bias towards certain shapes.
 %\autoref{GECCO paper} 
% The reality gap experiments consist of 2 phases: 1) The simulator phase, in which the controllers are optimized per robot for 100 generations of 60 controllers. These experiments are repeated 31 times with an independent random seed for good statistics. For a reliable insight into the dynamics of the reality gap we compare the median performing controller of the 31 runs on the real world counterpart. 2) The real-world phase, in which 11 controllers are evaluated in the real-world counterpart of the robots in the test suite. For these tests we  select the overall best performing controller found by the RevDE optimizer and for every $10^{th}$ generation we choose the controller with the median performance. This why we ran an odd number, specifically 31, repetitions.

Using this test suite we conduct the reality gap experiments in two phases.

\subsection{Simulation experiments}
 The first phase is executed in simulation. For each robot in the test suite we evolve the controller for gait learning for 100 generations of 60 individuals using RevDE. Thus, each run amounts to testing 6000 controllers on the given robot. One such test can be seen as a fitness evaluation from the RevDE perspective and as a learning trial from the robots perspective. Each trial  takes \unit[30]{s} in simulation. At the start of each trial, we place a robot in a neutral position (all joint angles $\unit[0]{rad}$) centred on a flat horizontal plane with a gravitational pull of $\unit[9.81]{m/s^2}$, as shown in \autoref{fig:models_s}. We use Gazebo for the simulation with the ODE physics engine and RK4 integration ($\mathrm{dt}=\unit[0.05]{s}$). Fitness is defined as the average speed during a trial (in \unit[]{cm/s}), calculated by taking the absolute distance traveled in centimetres divided by \unit[30]{s}. The full Github source can be found here\footnote{\url{https://github.com/fudavd/revolve/tree/IEEE-TCDS_2021}}.
 
\begin{figure}[ht!]\centering
\input{figures/models/models}
\caption{\label{fig:models_s}Test suite of six robots as rendered in the simulator.}
\end{figure}
 
These experiments are repeated 31 times for every morphology; thus for each morphology, the controller evolution results are aggregated over 31 independent runs. 

\subsection{Real-world experiments}
The second phase tests the performance of the evolved controllers in the real world. Experimenting with real robots is by far the most challenging part. With our current lab facilities employing automated continuous 3D printing of modules, off-the-shelf components (servos, Raspberry Pies, batteries) and manual assembly, the construction of one robot takes approximately 6 hours of work. The physical instances of our six robots in the test suite are shown in \autoref{fig:models_r}. %With the physical instances ready, the dynamics of the reality gap during controller evolution in simulation is then investigated as follows.

As explained above, on each robot we have executed 31 evolutionary runs in simulation. For each evolutionary run we log and plot the best performing controller in the population per generation. Thus, in the end, each morphology has 31 curves showing the best controller as a function of the generation number. (See Figure \ref{fig:res_curve_rg} for the aggregated curves.)

To measure the reality gap we test one controller every $10^{th}$ generation on the real robot. To this end, we choose to use the controller belonging to the median of the 31 best controllers for that generation. We decided not to use the best controller here, because a single lucky run could dominate all tests, and distort the results. Besides every $10^{th}$ generation, we are also interested in the reality gap for the best controller over all 31 runs. We use this as an indication of maximal over-fitting (assuming that the most exploitation has occurred in the best controller). For the sake of robustness, each real-world controller test is repeated three times (in total 33 real experiments of \unit[30]{s} per robot). Distance traveled was measured using an overhead camera with tracking software to calculate the number of pixels moved (see \autoref{fig:lab}). Fitness (average speed \unit[]{cm/s}) was then computed by calibrating the number of pixels per centimetre using a measuring tape. Here, we define the reality gap as the absolute difference of the simulated fitness (absolute velocity) and the mean fitness over the corresponding 3 repetitions in the real world.


\begin{figure}[ht!]\centering
\input{figures/models/models_r}
\caption{\label{fig:models_r}Test suite of six robots in the real world.}
\end{figure}

\begin{figure}[ht!]\centering
\input{figures/lab}
\caption{\label{fig:lab}Real world experiment setup.}
\vspace{-1em}
\end{figure}

\subsection{Analysis}
In addition to the relation of the reality gap with respect to evolutionary dynamics, we are also interested in several other indicators. The goal of these indicators is to provide a prediction of the size of the reality gap before testing in the real world. This could help to dismiss bad designs and behaviors before they are tested in the real world, which would increase the effective budget. These indicators are, therefore, solely measured in simulation. Here, we split our analysis into robot body indicators (specified by morphological descriptors \cite{miras2018effects}), and robot brains (defined by behavioral measures). For our morphological descriptors we are interested in the following three indicators:

\textit{Symmetry}, is defined as a ratio of modules that match on the opposite side of a line of symmetry, divided by the total number of possible module matches. The line of symmetry is 1 module thick (i.e. it doesn't contribute to the total possible matches) and only along horizontal, or vertical axis. Of these two, only the maximum symmetry is used.

\textit{Limb ratio}, is the number of actual limbs divided by how many limbs a specific morphology could have had, based on its size. Here, we define a limb as a module with a single connection. The limb ratio indicates how many extremities are present in a body relative to its size.

\textit{Block ratio}, indicate the number of passive modules or `dead weight' in a robot. It is calculated by the total number of block components divided by the total number of modules present in the body.

The choice of these three descriptors is based on the amount of spread of our test suite in these dimensions. More specifically, our 6 selected morphologies show the highest standard deviation in these descriptors. The morphological descriptors can help the evolutionary process to filter out morphologies before considering their behavior. This will increases the effective budget (number of evaluations) for the optimizer by only considering viable options. Unfortunately, over-fitting and simulator exploitation can still occur when considering a viable morphology. We try to capture this dynamic in our behavioral measures with the following three indicators:

\textit{Vertical speed}, in simulation we record the centre of mass position and velocity of our robot every \unit[5]{ms} (see \autoref{fig:con_measures}). The vertical speed is defined as the sum of the absolute velocity in the Z-direction (i.e. green arrow in \autoref{fig:con_measures}). 

\textit{Velocity direction}, is the sum of the centre of mass' absolute angle of velocity with respect to the horizontal plane (denoted as $\theta$ in \autoref{fig:con_measures}). 

\textit{Balance}, is defined as the total absolute roll and pitch angle of the robot head component relative to the horizontal plane. This measure is normalized such that a constant horizontal head position corresponds to Balance = 1, while a constant 180 degree rotated head position corresponds to 0.

\begin{figure}[ht!]
\input{figures/Con_measures}
\caption{\label{fig:con_measures}Visual representation of the measures used. Every \unit[5]{ms} in simulation we obtain the center of mass position (grey sphere), and velocity (red arrow). For the behavioral measures we calculate the absolute speed in vertical direction (green arrow), and the absolute angle with the horizontal plane.}
\end{figure}

Our final analysis will be on the reality gap landscape as a function of controller measures. We interpolate the reality gap data in behavioral space using a Gaussian mask to calculate a weighted average (see \autoref{eq:Gauss_RG}). This mask ($\mathcal{P}_k(x,y)$) is placed at each data point $k$ in behavioral space $(x_k, y_k)$, where dimensions $x$ and $y$ refer to the combination of two behavioral measures. Subsequently, a weighted average (based on $\mathcal{P}_k$) of the reality gap is taken at each point in behavioral space (see \autoref{eq:Weight_RG}). Here, $RG_k$ denotes the reality gap value of data-point $k$ for a specific behavior. As all 6 robots are tested with 11 different controllers in the real world (the median every $10^{th}$ gen + the best controller overall), we obtain 66 unique data-points for our behavioral space landscape.

\begin{equation}\label{eq:Gauss_RG}% \small
    \begin{aligned}
        \mathcal{P}_k(x,y) &= \frac{1}{2 \pi \sigma_p^2}exp\Bigg\{-\frac{(x-x_k)^2}{2\sigma_{p}^2} -\frac{(y-y_k)^2}{2\sigma_p^2}\Bigg\}\\
    \end{aligned}
\end{equation}
\begin{equation}\label{eq:Weight_RG}% \small
    \begin{aligned}
        \mathcal{F}(x,y) &= \frac{\sum_k \mathcal{P}_k(x,y)RG_k}{\sum_k \mathcal{P}_k(x,y)}\hphantom{xxxxXxXxxlxlxlxl}\\
    \end{aligned}
\end{equation}

\section{Results}
From the simulation phase, 11 controllers were tested per morphology in the real world: 1 overall best-, and 10 median controllers at every $10^{th}$ generation. Learning curves with their corresponding real fitnesses are presented in \autoref{fig:res_curve_rg}. The red curve presents the median fitness in simulation with its respective standard deviation bounds ($\pm$ STD) in blue. On the side, each star shows the overall best performance. The results from the real experiments are shown as black crosses. Here, we can see that real-world performance follows the learning curves for the first couple of generations in Gecko, Snake, and Spider, but then falls off around the $50^{th}$ generations. Additionally, the Blokky and Stingray morphologies seem to be indifferent to the improvements in the simulator. Lastly, we see that the overall best controllers do not seem to drop more in performance than the median, which suggests that the source for the reality gap does not originate from over-fitting in our experiments.

\begin{figure}[ht!]
\input{figures/Perf_curve}
\caption{\label{fig:res_curve_rg}Performance curves of the real and simulated experiments for all robots. The red curves show the best fitness averaged over 31 independent runs in the simulator; the shaded region denotes 95\% confidence interval. The black crosses exhibit the fitness measured three times on the real robot using the median controller of the given generation.}
\end{figure}

\autoref{tab:RG} shows the average reality gap values for each of the six robots in the test suite, \autoref{fig:res_RG_gen} displays them per generation number.

In \autoref{fig:res_RG_gen} we also plot a trend line to spot a possible relationship between the reality gap as a function of generations. Overall we see a trend of increasing reality gap values as controller evolution progresses. Interesting to note is that we can distinguish different types of relationships with this reality gap increase. 

\begin{figure}[ht!]
\input{figures/RG_vs_gen}
\caption{\label{fig:res_RG_gen}Reality gap as a function of generation.}
\end{figure}

Blokky, Salamander and Stingray seem to have morphologies that are exploiting the simulator from the start on. Here, the increase of the reality gap can be attributed to increasing the controller fitness in simulation, i.e. exploiting the simulator further. Over-fitting is not a concern here as the morphology itself does not seem viable in reality in the first place.

For Gecko, Snake and Spider the reality gap shows a progression that is more as expected. Early on, the reality gap reduces as the optimizer selects less random behaviors and develops well-transferable controllers based on generalizable physics in the simulator. Further in the evolutionary optimization, the chances of finding a controller that is exploiting the simulator increases due to over-fitting. For example, the snake relies on rolling sideways over the ground. A small perturbation to such an unstable gait can result in very different outcomes, resulting in highly fluctuating reality gap values.

The average reality gap values per robot in \autoref{tab:RG} show a remarkable split. The Gecko and the Spider have values around 1, while the other robots sit just under or above 2. Although the limited number of six robots is not enough for a statistically grounded explanation, we can still formulate a hypothesis: robots `walking on all four' suffer less from the reality gap. 

\begin{table}[ht!]
    \small
    \captionof{table}{\label{tab:RG} Average reality gap values per robot}
    \centering
    \renewcommand{\arraystretch}{1}
    \begin{tabular}{l c}
    \toprule
    Robot           & Avg. RG value \\ \midrule
    Blokky          & 1.92 \\ 
    Gecko           & 1.04 \\
    Salamander      & 2.25 \\
    Snake           & 2.27 \\
    Spider          & 1.09 \\ 
    Stingray        & 1.82 \\ 
    \bottomrule
    \end{tabular}
\end{table}

The use of novelty search in the selection of our test suite allows us to infer trends considering the reality gap as a function of morphological descriptors (symmetry, limb ratio, and block ratio) \cite{miras2018effects}. The reality gaps of all experiments are aggregated per morphology in \autoref{fig:res_RG_morph} (mean $\pm 95\%$ confidence interval). 

\begin{figure}[t!]\centering
\input{figures/RG_vs_morph}
\caption{\label{fig:res_RG_morph} Mean reality gap as a function of morphological traits. Error bars indicate $\pm 95\%$ confidence intervals. Dashed lines show different trends: Symmetry $RG= -1.102x +  2.208$; Limb ratio $RG= 9.211x^2-7.477x +  2.769$; Block ratio $RG= 21.619x^2+-21.269x + 6.786$.}
\end{figure}

For all three morphological descriptors some trends are visible (dashed lines in \autoref{fig:res_RG_morph}). Symmetry seems negatively correlated with the reality gap, meaning the more symmetric a morphology the smaller its reality gap during evolution. The reality gap as a function of limb ratio seems to follow a parabolic relationship. Here, a reality gap minimum can be found between 0.3 and 0.5 while an unbalanced limb ratio (very high or low) indicate a high reality gap. Furthermore, a lower ratio of limbs seems to imply a higher reality gap variability within a morphology. This is possibly a result of a less stable morphology due to a lower ratio of limbs. Lastly, the block ratio descriptor also indicates a weak parabolic relation to the reality gap (although the evidence is less convincing than the limb ratio). 


Testing 11 different controllers per morphology in the real world results in 66 distinct behaviors with corresponding reality gap values. Below we present the reality gap as a function of our 3 behavioral measures (vertical speed, velocity direction, and balance; see \autoref{fig:res_RG_controller}). Here, we consider individual trends per morphology (shown as different trend lines). For Blokky, Salamander and Stingray the reality gap seems rather indifferent to the behavioral measures, as expected since their behavior exploits the simulator from the start. The Snake's performance seems very inconsistent, although some trends are visible with vertical speed and balance. The best trends are apparent for Spider and Gecko, where higher vertical speed and velocity direction leads to a lower reality gap.

Visual comparison of the real- and simulated behavior clarifies the different results in \autoref{fig:res_RG_controller} (see short video\footnote{\url{https://www.youtube.com/watch?v=spetUQIfPdM}}). The Snake's gait is identifiable by its low balance and results in a highly variable reality gap by being very unstable. Blokky and Salamander exploit contact dynamics in the simulator causing them to slide horizontally (shown as low vertical speed and velocity direction, and high Balance). Stingray seems to slip less in the real world due to a difference in simulated friction. Finally, Gecko and Spider show to lower the reality gap when exhibiting a stepping behavior in contrast to sliding over the ground (i.e. `walking on all four'). 

\begin{figure}[t!]
\input{figures/RG_vs_controller}\centering
\caption{\label{fig:res_RG_controller}Reality gap as a function of behavioral measures. Trendlines of the reality gap as a function of behavioral measure are shown within each morphology. For the sake of clarity we do not report the trendline coefficients.}
\end{figure}

The reality gap landscape can help us identifying the afore-mentioned behaviors more clearly (see \autoref{fig:res_RG_contour}). For example, the `sliding behavior' of Blokky and Salamander and the high reality gap results of the Snake show themselves as individual peaks in the reality gap landscape. More interestingly, the combined trends for the behavioral measures `velocity speed' and `velocity direction' show a large reality gap valley in behavioral space.

\begin{figure}[ht!]\centering
\input{figures/RG_contour}
\caption{\label{fig:res_RG_contour}Contour plots of the reality gap as a function of behavioral measures. Dots represent individual reality gap values.}
\end{figure}

At last, we re-run the same full evolutionary experiment (evolving both body and brain) from which we obtained our test-set \cite{miras2018effects}. But, to showcase the viability of using a heuristic measure, we now penalize exploitative behaviors before parent selection using our findings presented above. The behavioral indicator `vertical speed' is used in the following way. If the vertical is higher than \unit[4]{cm/s} then the heuristic fitness $fitness_{heur} = 0$, while for a vertical speed lower than \unit[4]{cm/s} $fitness_{heur} = fitness(1-\frac{VS}{4})$, here $VS$ denotes vertical speed in \unit[]{cm/s}. The same fitness is applied as in \cite{miras2018effects} to obtain value $fitness$. Keep in mind that vertical speed is defined as an absolute number. The cutoff at \unit[4]{cm/s} is based on visual assessment of \autoref{fig:res_RG_controller}a. To see the effect of the heuristic measure, we compare the final populations of the original and heuristic experiment in morphological descriptor space. The results are presented in \autoref{fig:hist_compare}.

\begin{figure}[ht!]\centering
\input{figures/hist_compare}
\caption{\label{fig:hist_compare} Distribution in morphological space of the final populations in a full evolutionary experiment (corresponding y-axis on the left), where blue shows the original test-set run without the use of a heuristic measure, and orange the same experiment repeated with a `vertical speed' penalty in the fitness function. The black trendlines indicate predictions of the reality gap as a function of the respective descriptor (same as in \autoref{fig:res_RG_morph}), with corresponding values on the right y-axis.}
\end{figure}

The results show a clear effect of the measure in the population's distribution in the symmetry and block ratio descriptor space. Using the trends found in \autoref{fig:res_RG_morph}, we can see that the distribution of the population shifted more towards the regions with lower predicted reality gap (striped black lines), as intended. This shift shows a successful use of a controller measure to reduce the reality gap based on its prediction in morphological space. Thus, even though our heuristic measure is in behavioral space it indirectly influenced the morphological designs into a region that we deem more beneficial. This interaction may not be that surprising from an embodied intelligence perspective, but nonetheless, it shows the effectiveness of this pragmatic methodology.

A link to the full raw data-set with processing scripts and processed results for all experiments can be found here\footnote{\url{https://doi.org/10.34894/GGNAQ3}}.

\section{Discussion and Conclusion}

This paper aims to shed light on the reality gap in evolutionary robot systems where morphologies and controllers evolve simultaneously. Our goal is to gain new insights into the factors that influence the reality gap in such a system. Specifically, we address two research questions.  Firstly,  how does the reality gap depend on the robot morphologies? Secondly,  how does the reality gap change during an evolutionary run?

Discovering morphological properties that correlate with a big reality gap is especially interesting because such findings can be used to steer the evolutionary process away from likely wrong pathways. To this end, it is important to note that measuring morphological properties is much quicker than testing the behavior of a robot. This implies that monitoring morphologies for known indicators of a big reality gap is a computationally efficient way to prevent overfitting to simulation artefacts. For instance, morphologies that raise the red flag can be removed without wasting time on their fitness evaluation, the population can be (partially) restarted if it contains too many red-flagged morphologies, or the fitness function can be extended with a penalty term, such that the fitness of red-flagged individuals is reduced.

It should be noted that the impact of such preventive measures can be very different. Constraining the search by removing red-flagged individuals can heavily alter the evolutionary process and cut off certain pathways entirely. For example, by filtering out snake-like morphologies (\autoref{fig:models_s}d) we could impair the ability to evolve a gecko-like shape (\autoref{fig:models_s}b). A penalty-based approach is not this harsh as it does not eliminate entire regions of the search space, it makes them only less attractive to explore. The effectiveness of penalizing is shown by our last experiment where we re-ran a full body-brain experiment using an altered fitness that incorporated `vertical speed' as a risk indicating factor. The effect of this heuristic on the robot population was visible in the morphological space with a shifted distribution towards lower reality gap regions. This demonstrates a new option, using patterns of robot {\it behavior}, rather than {\it morphology} as indicators of a big reality gap. 
%in e viability of the idea So just by flagging exploitive behaviors, this behavioral constraint indirectly achieved similar outcomes as a morphological filter would when reducing the reality gap.

The differences in useful applications for the morphological and behavioral indicators are subtle but substantial. During evolution, the reality gap tends to increase by exploiting certain flaws in the simulator and the underlying physics engine. But, before the reality gap becomes a detrimental factor for reliable performance in the real world, robot designs are improved by utilizing transferable dynamics for the real world. Arriving efficiently at this sweet spot without being `tempted' to try exploitative designs can be accomplished by filtering out `inherently exploitative' morphological candidates (e.g. having low symmetry and an unbalanced limb ratio) before being tested. Arriving at the sweet spot, within a `non-exploitive' region in morphological space, a chance of over-fitting persist and unwanted behavior can still be beneficial. Here, monitoring the behavior after each evaluation helps the optimizer to mainly use general dynamics that are transferable to the real world. Thus, in short, when pushing for a low reality gap morphological descriptors improve the efficiency of the optimization (we don't test bad designs from the get-go) while behavioral indicators improve its robustness (i.e. we make sure no exploitative behavior is reproduced).

It should be noted that the descriptors studied in this paper may only be effective to study the reality gap for the design and task considered here, and may not generalize to the evolution of other tasks. However, we showed an overall process to study the dynamics of the reality gap which is applicable to other systems as well. In parallel, related research has been done to identify different descriptors for various tasks~\cite{de2020Tasks} that could be used in future work. As a final point, we believe that certain exploitable flaws are present in all simulators (e.g. contact dynamics, friction, and truncation errors) which makes the approach we outlined here relevant across all kinds of simulator applications.

For future work, testing and developing more filtering tools could improve the efficiency and robustness of an evolutionary setup where both the body and brain evolve. With proper filtering and dismissing of exploitative designs we will be able to reduce the reality gap pre-emptively during simulation (before real-world testing). This would make a robot evolution process that delivers high performing robots in the real world as end result more feasible. Unfortunately, conducting such an extensive experiment is currently not practicable, because a real experiment implementing controller and morphology evolution would produce about $60\times 100$ = $6000$ morphologies per run (where all the intermediate morphologies would require to be built and tested manually in the real world). With this work we hope to pave the way for evolution to become efficient enough for real experiments in the future by reducing the required effort to obtain viable solutions.

% \section{Acknowledgements} This work is supported by the Technology Innovation Institute, UAE.

==> 2/figures/CPG.tex <==
\centering

    \begin {tikzpicture}
	    [-latex,
		auto,
		node distance =1.375cm and 1.375cm,
		on grid,
		semithick,
		state/.style = {circle,draw,inner sep=0pt,minimum width = 0.7 cm}]
	\node[state] (X) {$x_i$};
	\node[state] (Y) [left = of X] {$y_i$};
	\node[state] (Output) [right = of X] {$out_i$};
	\path (X) edge [bend left = 30] node [] {$w_{x_iy_i}$} (Y);
	\path (Y) edge [bend left = 30] node [] {$w_{y_ix_i}$} (X);
	\path (X) edge  node [] {$w_{x_io_i}$} (Output);
	\node (ghost) [below of = X]       {};
	\end {tikzpicture}


==> 2/figures/CPG_net.tex <==
\centering
\resizebox{0.8\linewidth}{!}{%
\begin {tikzpicture}
	    [
		auto,
		node distance =0.33cm and 0.35cm,
		on grid,
		thick,
		state/.style = {circle,draw,inner sep=0pt, minimum width = 0.35 cm},
		box/.style={rectangle,draw,minimum width = 0.3 cm, minimum size=0.3 cm},
		core/.style={rectangle,draw=red!60,fill=red!5,very thick,minimum width = 0.6 cm, minimum size=0.6 cm}]
	\node[box] (B_l1) {};
	\node[state] (O4) [right = of B_l1] {$4$};
	\node[box] (B_l2) [right = of O4] {};
	\node[state] (O3) [right = of B_l2] {$3$};
	\node[core] (core) [right = 0.49cm of O3] {};
	\node[state] (O2) [above=0.48cm of core] {$2$};
	\node[box] (B_t2) [above=of O2] {};
	\node[state] (O1) [above=of B_t2] {$1$};
	\node[box] (B_t1) [above=of O1] {};
	\node[state] (O6) [right= 0.49cm of core] {$6$};
	\node[box] (B_r2) [right= of O6] {};
	\node[state] (O5) [right=of B_r2] {$5$};
	\node[box] (B_r1) [right=of O5] {};
	\node[state] (O8) [below=0.48cm of core] {$8$};
	\node[box] (B_b2) [below=of O8] {};
	\node[state] (O7) [below=of B_b2] {$7$};
	\node[box] (B_b1) [below=of O7] {};
	\path[draw=blue] (O4.10) to node [] {} (O3.170);
	\path[draw=blue] (O3.-170) to node [] {} (O4.-10);
	\path[draw=blue] (O6.10) to node [] {} (O5.170);
	\path[draw=blue] (O5.-170) to node [] {} (O6.-10);
	\path[draw=blue] (O2.100) to node [] {} (O1.-100);
	\path[draw=blue] (O1.-80) to node [] {} (O2.80);
	\path[draw=blue] (O7.100) to node [] {} (O8.-100);
	\path[draw=blue] (O8.-80) to node [] {} (O7.80);
	\path[draw=blue] (O3.50) to node [] {} (O2.-140);
	\path[draw=blue] (O2.-120) to node [] {} (O3.30);
	\path[draw=blue] (O3.10) to node [] {} (O6.170);
	\path[draw=blue] (O6.-170) to node [] {} (O3.-10);
	\path[draw=blue] (O3.10) to node [] {} (O6.170);
	\path[draw=blue] (O6.-170) to node [] {} (O3.-10);
	\path[draw=blue] (O6.150) to node [] {} (O2.-60);
	\path[draw=blue] (O2.-40) to node [] {} (O6.130);
	\path[draw=blue] (O2.-80) to node [] {} (O8.80);
	\path[draw=blue] (O8.100) to node [] {} (O2.-100);
	\path[draw=blue] (O6.-130) to node [] {} (O8.40);
	\path[draw=blue] (O8.60) to node [] {} (O6.-150);
	\path[draw=blue] (O6.-130) to node [] {} (O8.40);
	\path[draw=blue] (O8.60) to node [] {} (O6.-150);
	\path[draw=blue] (O3.-30) to node [] {} (O8.120);
	\path[draw=blue] (O8.140) to node [] {} (O3.-50);
	\end {tikzpicture}
}

==> 2/figures/Con_measures.tex <==
\begin{minipage}[c]{0.9\textwidth}
        \begin{minipage}[t]{0.45\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/results/controller1.pdf}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.45\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/results/controller3.1.pdf}
        \end{minipage}
        % \hfill
        % \begin{minipage}[t]{0.3\textwidth}
        %     \centering
        %     \includegraphics[width=\textwidth]{figures/results/controller3.png}
        % \end{minipage}
\end{minipage}

==> 2/figures/Perf_curve.tex <==
\begin{minipage}[c]{0.9\textwidth}
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Blokky]{\includegraphics[width=\textwidth]{figures/results/blokky.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Gecko]{\includegraphics[width=\textwidth]{figures/results/gecko.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Salamander]{\includegraphics[width=\textwidth]{figures/results/salamander.pdf}}
        \end{minipage}
    \end{minipage}

    \begin{minipage}[c]{0.9\textwidth}
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Snake]{\includegraphics[width=\textwidth]{figures/results/snake.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Spider]{\includegraphics[width=\textwidth]{figures/results/spider.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Stingray]{\includegraphics[width=\textwidth]{figures/results/stingray.pdf}}
        \end{minipage}
\end{minipage}

==> 2/figures/RG_class.tex <==
\small
\begin{tabular}{r| l | l}
    RG & \multicolumn{2}{l}{\makecell{Focus \\ \hspace{-2.2em}\textbf{Simulation process} \hspace{2.2em} \textbf{Design process}}}
            \\ \hline
            \multirow{10}[0]{*}{ \rotatebox{90}{\makecell{Improvement \\ \textbf{Robustness} \quad\quad \textbf{Reduce RG}}}
            }
            
        % \multirow{5}[0]{*}{
        %     \rotatebox{90}{Accuracy}
        % }
        & \multirow{4}{10em}{Miglino \textit{et al.} \cite{miglino1995evolving}
        \newline Jakobi \textit{et al.} \cite{jakobi1995noise}
        \newline Bongard \& Lipson \cite{bongard2004once}
        \newline Zagel \textit{et al.} \cite{zagal2004back}}  
            & \multirow{4}{10em}{Koos \textit{et al.} \cite{koos2012transferability}
            \newline\newline\newline}\\
           &    \\
           &        \\
           &        \\ \cline{2-3}
        % \multirow{5}[0]{*}{
        %         \rotatebox{90}{Robustness}
        % }
        & \multirow{7}{10em}{Jakobi \cite{jakobi1997evolutionary,jakobi1998minimal}
        \newline Boeing \& Brauml \cite{boeing2012leveraging}
        \newline Tobin \textit{et al.} \cite{tobin2017domain}
        \newline van Diggelen \textit{et al.} \cite{van2020effects}
        \newline\newline\newline} 
            & \multirow{7}{11em}{Floreano \& Mondada \cite{floreano1996evolution}
            \newline Urzelai \& Floreano \cite{urzelai2000evolutionary}
            \newline Floreano \& Urzelai \cite{floreano2001evolution}
            \newline Francesca \textit{et al.} \cite{francesca2014automode}
            \newline Ligot \textit{et al.} \cite{ligot2020simulation}
            \newline Moreno \& Faiña \cite{10.3389/frobt.2021.699814}
            \newline Chand \& Howard \cite{10.3389/frobt.2021.684304}
            }\\
        &   &        \\
        &   &        \\
        &   &        \\
        &   &        \\ 
        &   &        \\ 
\end{tabular}

==> 2/figures/RG_contour.tex <==
\begin{minipage}{0.9\textwidth}
        \begin{minipage}[t]{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/results/contour_0.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/results/contour_1.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/results/contour_2.pdf}
    \end{minipage}
    \begin{minipage}[t]{0.075\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/results/contour_grad.pdf}
    \end{minipage}
    \hfill
\end{minipage}

==> 2/figures/RG_vs_controller.tex <==
\begin{minipage}[c]{0.9\textwidth}
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Vertical speed]{\includegraphics[width=\textwidth]{figures/results/RG_Vel_Z-dir.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Velocity direction]{\includegraphics[width=\textwidth]{figures/results/RG_vel_dir.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Balance]{\includegraphics[width=\textwidth]{figures/results/RG_Balance.pdf}}
        \end{minipage}
\end{minipage}


==> 2/figures/RG_vs_gen.tex <==
\begin{minipage}[c]{0.9\textwidth}
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Blokky]{\includegraphics[width=\textwidth]{figures/results/blokky_RG.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Gecko]{\includegraphics[width=\textwidth]{figures/results/gecko_RG.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Salamander]{\includegraphics[width=\textwidth]{figures/results/salamander_RG.pdf}}
        \end{minipage}
    \end{minipage}

    \begin{minipage}[c]{0.9\textwidth}
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Snake]{\includegraphics[width=\textwidth]{figures/results/snake_RG.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Spider]{\includegraphics[width=\textwidth]{figures/results/spider_RG.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Stingray]{\includegraphics[width=\textwidth]{figures/results/stingray_RG.pdf}}
        \end{minipage}
\end{minipage}

==> 2/figures/RG_vs_morph.tex <==
\begin{minipage}[c]{0.9\textwidth}
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Symmetry]{\includegraphics[width=\textwidth]{figures/results/RG_symmetry.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Limb ratio]{\includegraphics[width=\textwidth]{figures/results/RG_limbs.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Block ratio]{\includegraphics[width=\textwidth]{figures/results/RG_block_ratio.pdf}}
        \end{minipage}
\end{minipage}

==> 2/figures/hist_compare.tex <==
\begin{minipage}[c]{0.9\textwidth}
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Symmetry]{\includegraphics[width=\textwidth]{figures/results/hist_compare_symmetry.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Limb ratio]{\includegraphics[width=\textwidth]{figures/results/hist_compare_limb_ratio.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Block ratio]{\includegraphics[width=\textwidth]{figures/results/hist_compare_block_ratio.pdf}}
        \end{minipage}
\end{minipage}

==> 2/figures/lab.tex <==
\begin{minipage}[c]{0.9\textwidth}
        \begin{minipage}[t]{0.591\textwidth}
            \centering
            \subfloat[Lab setup]{\includegraphics[width=\textwidth]{figures/lab/setup.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.388\textwidth}
            \centering
            \subfloat[Motion tracking]{\includegraphics[width=\textwidth]{figures/lab/motion_cap.pdf}}
        \end{minipage}
\end{minipage}

==> 2/figures/models/models.tex <==
\begin{minipage}[c]{0.9\textwidth}
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Blokky]{\includegraphics[width=\textwidth]{figures/models/blokky.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Gecko]{\includegraphics[width=\textwidth]{figures/models/gecko.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Salamander]{\includegraphics[width=\textwidth]{figures/models/salamander.jpg}}
        \end{minipage}
    \end{minipage}

    \begin{minipage}[c]{0.9\textwidth}
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Snake]{\includegraphics[width=\textwidth ]{figures/models/snake.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Spider]{\includegraphics[width=\textwidth ]{figures/models/spider.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Stingray]{\includegraphics[width=\textwidth]{figures/models/stingray.jpg}}
        \end{minipage}
\end{minipage}

==> 2/figures/models/models_r.tex <==
\begin{minipage}[c]{0.9\textwidth}
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Blokky]{\includegraphics[trim={0 4cm 0 1cm}, clip=true, width=\textwidth]{figures/models/blokky_r1.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Gecko]{\includegraphics[trim={0 2.5cm 0 2.5cm}, clip=true, width=\textwidth]{figures/models/gecko_r1.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Salamander]{\includegraphics[trim={0 5cm 0 0}, clip=true, width=\textwidth]{figures/models/salamander_r1.jpg}}
        \end{minipage}
\end{minipage}

\begin{minipage}[c]{0.9\textwidth}
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Snake]{\includegraphics[trim={0 5cm 0 0}, clip=true,
            width=\textwidth]{figures/models/snake_r1.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Spider]{\includegraphics[trim={0 0 0 5cm}, clip=true,
            width=\textwidth]{figures/models/spider_r1.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Stingray]{\includegraphics[trim={0 0 0 5cm}, clip=true,
            width=\textwidth]{figures/models/stingray_r1.jpg}}
        \end{minipage}
\end{minipage}

==> 3/AAC_main.tex <==


% \setlength{\abovedisplayskip}{9pt}
% \setlength{\belowdisplayskip}{9pt}
% \setlength{\belowcaptionskip}{-1pt}
% % Make Figure Great Again
%     \usepackage{float} % [H]
%     \usepackage{wrapfig} % text wrapping
%     % \usepackage{caption} % \caption
%     \usepackage{subcaption} % \subcaption
%     \usepackage{graphicx} % \includegraphics
%     \usepackage[font=small,labelfont=bf]{caption}

    % packages for Flow diagrams
    % \usepackage{tikz}
    \usetikzlibrary{shapes.geometric, arrows, positioning, automata}
    \tikzstyle{process} = [rectangle, minimum width=2cm, minimum height=1cm, text centered, draw=black, fill=white!30]
    \tikzstyle{sum} = \tikzstyle{sum} = [draw, circle, minimum size=.5cm]
    \tikzstyle{arrow} = [thick,->,>=stealth]
    \def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;}
\begin{document}
%
% paper title
% Titles are generally capitalized except for words such as a, an, and, as,
% at, but, by, for, in, nor, of, on, or, the, to and up, which are usually
% not capitalized unless they are the first or last word of the title.
% Linebreaks \\ can be used within to get better formatting as desired.
% Do not put math or special symbols in the title.
% \title{The Effects of Adaptive Control on Learning Directed Locomotion}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:introduction}
\input{BAA_Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work} \label{sec:related}
\input{BAB_related}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experimental Setup} \label{sec:method}
\input{CAA_Method}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Results} \label{sec:results}
\input{DAA_Results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussion} \label{sec:discussion}
\input{EAA_Discussion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
\label{sec:conclusion}
\input{FAA_Conclusion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Acknowledgements}
%   This work is supported by the Technology Innovation Institute, UAE.
\end{document}


==> 3/AAD_abstract.tex <==
This study is motivated by evolutionary robot systems where robot bodies and brains evolve simultaneously. In such systems robot `birth' must be followed by `infant learning' by a learning method that works for various morphologies evolution may produce. Here we address the task of directed locomotion in modular robots with controllers based on Central Pattern Generators. We present a bio-inspired adaptive feedback mechanism that uses a forward model and an inverse model that can be learned on-the-fly. We compare two versions (a simple and a sophisticated one) of this concept to a traditional (open-loop) controller using Bayesian Optimization as a learning algorithm. 
The experimental results show that the sophisticated version outperforms the simple one and the traditional controller. It leads to a better performance and more robust controllers that better cope with noise.  

% This study is motivated by evolutionary robot systems where robot bodies and brains evolve simultaneously. In such systems robot `birth' must be followed by `infant learning' by a learning method that works for various morphologies evolution may produce. Here we address the task of directed locomotion in modular robots with controllers based on Central Pattern Generators. We present a bio-inspired adaptive feedback mechanism that uses a forward model and an inverse model that can be learned on-the-fly. Our experiments showed that adding this system to existing controllers helps learn proper movement execution without hampering the learning of a locomotion task. The system also can reduce the learning effort and increase the robustness of the learned controllers.

%against and  bio-inspired Internal Model Control feedback controller (IMC) that can function as an extension to already existing designs. As a test, we extended a previous controller (based on Central Pattern Generators, CPG) with two different versions of our IMC. \textit{IMC vanilla}, with two Deep Neural Networks (DNN) as internal models that learn on all layers; and \textit{IMC reservoir}, with two DNN that only learn on the output layers. We compared the performance of these controllers on the task of learning directed locomotion in 6 different robots. 

==> 3/BAA_Introduction.tex <==
The behavior of a robot is determined by its morphology (`body') and its controller (`brain') and the field of Evolutionary Robotics (ER) successfully demonstrated that good controllers can be evolved for various tasks \cite{bongard2013evolutionary, doncieux2015evolutionary}. To maximize the potential of the evolutionary approach morphologies and controllers should be evolved together, but this implies particular challenges. Specifically, since the inherited brain of a newborn robot may not match its inherited body, evolution can end up with premature convergence of the robot population \cite{lipson2016difficulty}. It has therefore been argued that a fully evolving robot system must contain a learning stage, directly following the `birth' of offspring robots \cite{eiben2013triangle,eiben2020if}. In such a system, the design and optimization of good robots take place through two processes: 1) the evolutionary process, where both the body and the brain evolve to obtain a higher fitness, 2) a lifetime learning loop, where the brain is optimized to control a given body (produced by the evolutionary process) to obtain high task performance. This idea motivates the development of controllers that can be optimized quickly for a broad range of morphologies.

Currently, most controllers in ER are evolved on using an open-loop control architecture in simulation \cite{winfield2015evolvable}. For real-world applications, this is clearly limiting, since in practice feedback control is often preferred.
%, thus creating a reality gap \cite{jakobi1995noise}. 
%If we want to develop controllers for real robot application we should start thinking about the effects of feedback as well.
Unfortunately, feedback control can be hard to implement, especially when the environment and morphologies are not known beforehand. Many feedback mechanisms require a lot of engineering per robot, which is infeasible if robots are (re)produced automatically by an evolutionary process. Furthermore, PID controllers will likely fail in  accommodating complex morphologies, as they are hard to design optimally and not well-suited for nonlinear systems \cite{babuvska2012fuzzy}. In this paper, we address this problem by introducing an adaptive bio-inspired feedback controller called Internal Model Control (IMC), which can be used as an extension to already available designs. This allows for simple real robot implementation, while minimally affecting the way evolution improves the original controllers. %However, adaptability might influence the lifetime learning process. 
To this end, we add our IMC as an extension to an existing CPG controller (\cite{lan2018directed,lan2020learning}) used for learning directed locomotion (see \autoref{fig:FlowOL}).

\begin{figure}[ht]
% \vspace{-.125em}
     \input{Figures/FlowOL}
\captionsetup{width=.95\textwidth}\footnotesize
\caption{\label{fig:FlowOL} A schematic overview of open-loop CPG controller with and without our adaptive IMC. For the IMC the \textit{inverse model} calculates the required motor input ($\mathrm{model}_{inv}\rightarrow u_i$) to follow a reference ($\phi_{ref,i}$), while the \textit{feedforward model} predicts the robots state based on its input ($\mathrm{model}_{ff}\rightarrow\phi_{pred}$). Differences between the predictied and actual state ($\phi$) are sent back ($e$).}
\vspace{-1.5em}
\end{figure}
\normalsize
The idea behind the IMC design is grounded both in industry and in neuroscience \cite{hunt1991neural} as a way for (human) controllers to compensate for errors in (movement) control. As an extension to an open-loop controller (in Figure~\ref{fig:FlowOL}, the CPG) we add two models that work together for proper movement execution. The inverse model calculates the required control input $u$ to get the robot from the current state to the reference state, $\mathrm{model}_{inv}: \phi_{ref}\rightarrow u$. The feedforward model predicts the result of that command, $\mathrm{model}_{ff}: u\rightarrow \phi_{pred}$. A perfect model will allow the IMC to subtract any error in the movement. For applications in ER, we will need to learn these models since we do not know the morphologies beforehand. We propose the use of Deep Neural Network (DNN) to learn the models of the IMC scheme. To this end, we will evaluate two different DNN types for our IMC: \textit{IMC vanilla}, in which the two DNN internal models learn on all their layers; and \textit{IMC reservoir}, in which the DNNs only learn on the output layers, much like in reservoir computing \cite{lukovsevivcius2009reservoir}.

With the IMC controller we can accommodate two important user needs in ER, 1) applicability to a wide range of morphologies, 2) easy implementation as an extension of already existing controller designs. However, it is possible that the adaptability might influence the lifetime learning process.  Thus, the overarching research question behind this paper is:

\textit{What is the effect of adding the IMC on learning control for directed locomotion in a variety of different morphologies?}








==> 3/BAB_Related.tex <==
Most of the work in ER in simulation does not address feedback control. ER experiments in which evolution is solely done in real robots do implement feedback control, but not learning, see e.g. the publications by Brodbeck \textit{et al.} \cite{brodbeck2015morphological}, Vujovic \textit{et al.} \cite{vujovic2017evolutionary}, and Nygaard \textit{et al.} \cite{nygaard2020environmental}. In these papers, feedback control is implemented using P(I)D controllers on simple robots. As PID control is limited in its capability, we believe that it can greatly influence the resulting morphologies. %The idea behind our IMC controller is to be minimally invasive to current ER controllers by adapting the internal models for optimal control.
The idea behind our IMC controller is to be minimally invasive to the evolutionary process with the controllers that are currently used in ER.
    
The benefits of adaptive feedback control have been shown before by Bongard \textit{et al.} \cite{bongard2006resilient}. They showed that their four-legged robot was able to learn locomotion rapidly through efficient sampling and continuous self-modelling. Furthermore, the adaptive self-modelling made their machine able to reconfigure its self-representation and control policy after physical damage. Other forms of adaptive feedback have been studied in the form of coupling sensory information back to the controller (\cite{ryu2010locomotion,inoue2007cpg}). In the case of CPGs, this means modulation of frequency or amplitude of the signals to the motors.  For other types of neural networks like HyperNEAT and recurrent neural networks (\cite{huang2003neural,drchal2009hyperneat,nordmoen2019evolved}), feedback allowed switching on and off certain parts of the network based on sensory information. Such an adaptive feedback control changes the overall robot behavior based on the sensory feedback, which is different from our aim to follow a reference trajectory as closely as possible. In other words, our feedback control is much more focused on the correct execution of movements at the local joint level while the other studies change the combined motor behaviors.

Similarly to our feedback design, Kawato \textit{et al.} \cite{kawato1987hierarchical} implemented an inverse model controller that learned to follow a reference signal with a three-link manipulator using a neural network. In a study by Miyamoto \textit{et al.} \cite{Miyamoto1988}, two neural networks were used in a similar IMC structure with feedback error learning to control a simulated manipulator as well. Hunt and  Sbarbaro \cite{hunt1991neural} implemented IMC with two neural networks that learned their models by example (a pre-existing feedback controller), before testing it on a simulated plant. Li and Deng \cite{li2006approximate} implemented an IMC design in which a single neural network was used to compensates for model mismatches in both internal models. More recently, \cite{massi2019combining} compared two adaptive feedback controllers (a PID with and without a convolutional neural network) that used evolution to learn locomotion in a real quadruped robot. These studies show that the IMC structure can be used to obtain high-performance nonlinear control. To our knowledge, we are the first to test an adaptive IMC controller within ER.

Our work positions itself in a rare intersection of adaptive feedback control and ER. Many (adaptive) feedback control studies focus primarily on the dynamics of the errors when following a reference and not on the robot behavior itself. However, in the context of our paper, the robot's behavior is also influenced by the changing feedforward CPG. Conversely, much research in ER is solely focused on the behavior of the controllers, while overlooking the influence of feedback control. We suspect a strong coupling between both within ER, thus playing a vital role in transferring from simulation to the real world. From this perspective, we position ourselves uniquely in comparison to other (bio-inspired) controllers, in that we implement both learning directed locomotion as well as adaptive feedback control. On top of that, we require learning to occur quickly, on a broad range of different robot morphologies.

% Our work positions itself in a rare intersection of adaptive feedback control and ER. Many (adaptive) feedback control studies focus primarily on the dynamics of the errors and not on the actual movements itself. However, in the context of our paper, the robot's behaviour is also influenced by the feedforward CPG. Much ER research is solely focused on the learned performance of the robot behaviour, while forgetting the difficulties arising from implementing feedback control. We think that the interplay between both plays a vital role in transferring ER from simulation to the real world. Lastly, in comparison to other (bio-inspired) controllers, we position ourselves uniquely from an ER perspective which requires the IMC to be broadly applicable to morphologically different robots.



==> 3/CAA_Method.tex <==
\subsection{Test suite}
We will use 6 different robots ($N=6$) that are made of off-the-shelf components based on the modular RoboGen framework, see  \autoref{fig:subjects}. Spider, Gecko, and Snake (top row) are designed beforehand, while BabyA and BabyB are first generation children from the Gecko and Spider. Finally, the 6677 is a product of the evolution of multiple generations. 
\subsection{Test Procedure}
Each robot is tested in $10$ different experiments with three different controllers. The original open-loop controller \cite{lan2020learning}, and the two IMCs (vanilla and reservoir). Each experiment consists of $300$ learning trials in which the controller improves on the task of directed locomotion. This makes the total of $3\times6\times10\times300=5400$ learning trials. At the start of each learning trial, we place the robot in the center of a flat horizontal plane with a gravitational pull of $\unit[9.81]{m/s^2}$ downward. Each trial takes $60\mathrm{s}$ in simulation. In total we simulate $5400\times60=\unit[3.24\times10^6]{s}$, which equals $\unit[900]{h}$. Simulation is done in Gazebo using the ODE physics engine with Runge-Kutta 4 integration ($\mathrm{dt}=\unit[0.05]{s}$). The sampling period of the controller is $\unit[0.125]{s}$.

\begin{figure}[h]\centering
% \vspace{-1em}
\begin{minipage}[c]{0.75\textwidth}
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Spider]{\includegraphics[width=\textwidth]{Figures/Subjects/spider9-body.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Gecko]{\includegraphics[width=\textwidth]{Figures/Subjects/gecko7-body.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[Snake]{\includegraphics[width=\textwidth]{Figures/Subjects/snake.png}}
        \end{minipage}
    \end{minipage}

    \begin{minipage}[c]{0.75\textwidth}
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[BabyA]{\includegraphics[width=\textwidth]{Figures/Subjects/babyA-body.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[BabyB]{\includegraphics[width=\textwidth]{Figures/Subjects/babyB-body.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[6677]{\includegraphics[width=\textwidth]{Figures/Subjects/6677.png}}
        \end{minipage}
\end{minipage}
% \vspace{-.5em}
\captionsetup{width=.95\textwidth}\footnotesize
\caption{Test suite with custom (top) and evolved (bottom) designs.}
\label{fig:subjects}
\end{figure}
    
\section{Controller design}     
We start with explaining the open-loop CPG controller based on the work by Lan \textit{et al.} \cite{lan2020learning}. The added IMC controller will use the same CPG controller extended with the two DNN as internal models. The two flavors of IMC (IMC vanilla or IMC reservoir) will be explained in detail later on. Learning locomotion is done by updating the CPG weights in between learning trials while the weights of the DNN models in the IMC are updated during each trial. 

\subsection{Learning Locomotion with CPG}
The CPGs are based on the design by Ijspeert \textit{et al.} \cite{ijspeert2008central}. A single CPG is represented by a neuron pair ($x_i$,$y_i$) that reciprocally inhibit and excite each other to produce oscillatory behavior. Here, $i$ denotes the specific joint that is associated with this CPG. The dynamics of a single CPG is defined by the current state of its neuron pair. The change of every neuron state is calculated by multiplying the current state of the opposite neuron with a weight ($w$), as shown in \autoref{fig:CPG_model_IMC}a. The weights $w_{x_iy_i}$ and $w_{y_ix_i}$ represent a connection strength between each neuron pair within the CPG, while $w_{x_io_i}$ represents the coupling strength from the $x$-neuron to an output neuron that controls a joint (\textit{i.e.} servo). By changing the weights of the CPGs, we can learn locomotion. 

\begin{figure}[ht]
        \centering
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \subfloat[CPG]{	    
            \centering
    		\begin {tikzpicture}
    		    [-latex,
    			auto,
    			node distance =1.375cm and 1.375cm,
    			on grid,
    			semithick,
    			state/.style = {circle,draw,inner sep=0pt,minimum width = 0.7 cm}]
    		\node[state] (X) {$x_i$};
    		\node[state] (Y) [left = of X] {$y_i$};
    		\node[state] (Output) [right = of X] {$out_i$};
    		\path (X) edge [bend left = 30] node [] {$w_{x_iy_i}$} (Y);
    		\path (Y) edge [bend left = 30] node [] {$w_{y_ix_i}$} (X);
    		\path (X) edge  node [] {$w_{x_io_i}$} (Output);
    		\node (ghost) [below of = X]       {};
    		\end {tikzpicture}}
        \end{minipage}
        % \hfill
        \begin{minipage}[t]{0.4\textwidth}
            \centering
            \subfloat[CPG network]{\input{Figures/CPG_net}}
        \end{minipage}
            % \includegraphics[width=0.6\linewidth, ,keepaspectratio]{Figures/CPG_model.png}
           \vspace{-.5em} \captionsetup{width=.95\textwidth}\footnotesize
           \caption{\textbf{a}: A single CPG \textbf{b}: The CPG network for our Spider, containing 8 CPGs (numbers) with 10 connections (blue lines).}\label{fig:CPG_model_IMC}
\end{figure}
        
To enable complex output patterns, we allow CPG connection to exist between neighboring joints, see \autoref{fig:CPG_model_IMC}b. The set of neighboring joints ($\mathcal{N}_i$) at joint $i$, consists of all the joints $j$ positioned within a distance of 2 modules. The ordinary differential equations of the resulting CPG network are described in \autoref{eq:ODE_CPG_IMC}. Connections between neighboring joints $j$ are denoted as $w_{x_jx_i}$.
        
        \begin{align}\label{eq:ODE_CPG_IMC}
            % \begin{split}
                \Dot{x}_i =  w_{y_ix_i}y_i + \sum_{j \in \mathcal{N}_i} x_{j} w_{x_jx_i} &&\Dot{y}_i =  w_{x_iy_i}x_i
            % \end{split}
        \end{align}
        
        For the output neuron a tangent hyperbolic activation function is used (see \autoref{eq:output}). To simplify the search space we implement the following ralations between the weights: $w_{x_iy_i} =  -w_{y_ix_i}; w_{x_jx_i} = w_{x_ix_j}; w_{x_io_i} = 1$. At the start of each learning trial all neuron states will be set to a predefined value $(x,y)=\left(-\frac{1}{\sqrt{2}},\frac{1}{\sqrt{2}}\right)$. %Simple Newton-Heun integration is used to update the state of each neuron for the subsequent time step.
        
        \begin{equation}\label{eq:output}
            \begin{split}
                out_i(x_i) & = \frac{2}{1 + e^{-2 x_iw_{x_io_i}}} - 1
            \end{split}
        \end{equation}
    
To improve the weights of the CPG network, we define a performance measure ($\mathcal{F}$). During a learning trial the CPG network commands the robot to move through space, which can be described by a trajectory $p(t)$, see \autoref{fig:fitness_IMC}a. In the case of directed locomotion, we want this movement to 1) be as far as possible in the target direction ($\beta_T$), and 2) have as minimum possible deviations from this direction ($\delta$). To this end, we formulate $\mathcal{F}$ as follows:
    
    \quad 1) First obtain $\delta$:
        \begin{equation}
        % \delta = 
        \delta{(\beta_0, \beta_1)} = 
          \left\{
           \begin{aligned}
           &2 \pi - \lvert \beta_1 - \beta_0\rvert  &\hspace*{2em} (\lvert \beta_1 - \beta_0 \rvert > \pi) \\
           &\lvert \beta_1 - \beta_0 \rvert    &\hspace*{2em} ~(\lvert \beta_1 - \beta_0 \rvert \leq \pi) \\
           \end{aligned}
           \right.
        \end{equation}
\noindent Note that $\delta$ ranges from $\left[-\pi,\pi\right)$, with the range $\left(-\frac{1}{2}\pi,\frac{1}{2}\pi\right)$ being (partly) towards the target direction.

    \quad 2) Calculate the distance travelled in the target direction at the end of a trial, $\mathcal{D}_{dir}$:
    
    \begin{equation}
        \mathcal{D}_{dir} = \lvert P_{end}-P_0 \rvert\cos{\delta}
    \end{equation}
    
\noindent Here $\lvert P_{end}-P_0 \rvert$ denotes the Euclidean distance between $P_{end}$ and $P_0$.% $\mathcal{D}_{dir}$ is equal to the projection of the the end position on the target direction $P_{end,\perp}$.

    \quad 3) Calculate the total distance deviated from the target direction at the end of the trial, $\mathcal{D}_{dev}$:
    
    \begin{equation}
        \mathcal{D}_{dev} = \lvert P_{end}-P_0 \rvert\sin{\delta}
    \end{equation}

    \quad 4) Now we formulate $\mathcal{F}$ as follows:
    
    \begin{equation}
        \label{eq:fitness_IMC}
        \mathcal{F}(\mathcal{D}_{dir}, \mathcal{D}_{dev}) = \lvert\mathcal{D}_{dir}\rvert\mathcal{D}_{dir} - \mathcal{D}_{dev}^2
    \end{equation}


\noindent $\mathcal{D}_{dev}$ is squared to penalize strong deviation from the target direction, $\mathcal{D}_{dir}$ is multiplied by its absolute value to encourage movement towards the target direction. The units of our performance measure are $\unit[[\mathcal{F}]]{=m^2}$. A contour plot of $\mathcal{F}(\mathcal{D}_{dir},\mathcal{D}_{dev}$) is shown in \autoref{fig:fitness_IMC}b.

\begin{figure}[ht]
\centering
        \begin{minipage}[t]{0.3\textwidth}
            \subfloat[Performance variables]{\includegraphics[width=\textwidth,keepaspectratio]{Figures/direction.pdf}}
        \end{minipage}
        \hspace{1em}
        \begin{minipage}[t]{0.3\textwidth}
            \subfloat[Contour plot]{\includegraphics[width=\textwidth, ,keepaspectratio]{Figures/fitness_cont.pdf}}
        \end{minipage}
    \captionsetup{width=.95\textwidth}\footnotesize
    \caption{\textbf{(a)}: Visualization of the variables necessary for the performance measure. $\beta_T$ shows the target direction, while $\beta_{end}$ the actual direction, $P_0$ start, $P_{end}$ end positions. The difference in direction is denoted by angle $\delta$ and the projection of $P_{end}$ onto the target direction by $P_{end,\perp}$.
    \textbf{(b)}: contour plot of the performance measure. The black isolines show monotonically increasing performance values ranging [-6,8] with steps of 2, from the bottom to top in target direction (red arrow).}
    \label{fig:fitness_IMC}
\end{figure}

The optimization of the weight will be done using a Bayesian Optimization (BO) algorithm, which models the fitness function using Gaussian Processes ($\mathcal{GP}$) \cite{jasper2012practical}. With $\mathcal{GP}$ BO efficiently selects promising samples for subsequent trials. The hyperparameters of the BO are derived from \cite{lan2020learning}, which shown in \autoref{tab:parameters_bo}. We initialize the BO algorithm by pseudo-randomly evaluating 50 evenly distributed samples in search-space  using Latin Hypercube Sampling (LHS).

\begin{table}[ht!]
    % \setlength{\textfloatsep}{0.7\baselineskip plus 0.2\baselineskip minus 0.5\baselineskip}    
    \footnotesize
    \caption{Hyperparameters of the BO algorithm, from \cite{lan2020learning}.}
    \label{tab:parameters_bo}
    \centering
    \renewcommand{\arraystretch}{1}
    \begin{tabular}{l ll}
    \toprule
    Parameters          & Value & Description \\ \midrule
    Initial sampling    & LHS       & Sampling method\\
    Initial samples     & 50        & Number of samples\\ 
    Learning iterations & 250       & Number of evaluations\\ 
    Kernel type         & Mat\'ern 5/2 & Approximation kernel\\
    Kernel variance     & 1.0       \\ 
    Kernel length       & 0.2       \\ 
    UCB alpha           & 3.0       & Acquisition function weight\\  \bottomrule
    \end{tabular}
\end{table}
% \v
    
\subsection{Adaptive IMC Control}
for the implementation of optimal feedback control, we extend the open-loop CPG controller with our IMC controller. For the internal models we will use two different DNN. The design of the DNN for the inverse model consists of an input layer containing $4k$ neurons (input layer $\mathrm{model}_{inv} = [\phi_{1:k}$, $\Dot{\phi}_{1:k}$, $\phi_{ref,1:k}$, $\Dot{\phi}_{ref,1:k}]^T$), with $k$ being the total number of servomotors; two hidden layers of the same size ($4k$) with Rectified Linear activation units (ReLU); and an output layer of $k$ neurons (output layer $\mathrm{model}_{inv} = [u_{1:k}]^T$), which sends the control signals to the servomotors. For the output layer, we choose the same tangent hyperbolic neuron as in \autoref{eq:output}. 
        
%For the feedforward model the DNN consists of an input layer of $3k$ neurons ($\mathrm{input}_{ff} = [\phi_{1:k}$, $\Dot{\phi}_{1:k}$, $u_{1:k}]^T$), two hidden layers of the same size ($3k$) with ReLU activation units, and an output layer of $2k$ neurons ($\mathrm{output}_{inv} = [\phi_{pred,1:k},\Dot{\phi}_{pred,1:k}]^T$) that predicts the state at the next time step ($\phi_{pred,1:k}$ and $\Dot{\phi}_{pred,1:k}$). For the output layer we also use the tangent hyperbolic neuron similarly as in Equation \autoref{eq:output}.

The DNN for the feedforward model has an input layer of $3k$ neurons (input layer $\mathrm{model}_{ff} = [\phi_{1:k}$, $\Dot{\phi}_{1:k}$, $u_{1:k}]^T$); two hidden layers of the same size ($3k$) with ReLU; and an output layer of $2k$ neurons (output layer $\mathrm{model}_{ff} = [\phi_{pred,1:k},\Dot{\phi}_{pred,1:k}]^T$). For the output neurons we also use the tangent hyperbolic function.

The implementation of the DNN is done in C++ using libtorch v1.4.0. For optimization, we update both biases and weights. Only at the beginning of an experiment (\textit{i.e.} at the start of the first trial) we randomly initialize these parameters by sampling from a Gaussian distribution with zero mean and variance of one. To train the models in the IMC vanilla we continuously update all the weights and biasses for the hidden and output layers. For the IMC reservoir, we freeze the weights and biases of the hidden layers after initialization and only optimize the output layer. Updating of the weights and biases is done whenever a new reference signal is sent to the IMC. For the IMC vanilla controller the total number of parameters to be optimized in the $\mathrm{model}_{inv}$ is $4(4+4+1)2k = 72k$, and for the $\mathrm{model}_{ff}$ $3(3+3+2)2k = 48k$. While for the IMC reservoir the total number of parameters in the $\mathrm{model}_{inv}$ is defined as $4(0+1)2k = 8k$, and for the $\mathrm{model}_{ff}$ $3(0+2)2k = 12k$.
        
The goal of the IMC is to minimize the error between the reference state and the actual state. This is achieved by 1) the $\mathrm{model}_{inv}$ providing correct motor inputs to follow the desired state, and 2) the $\mathrm{model}_{ff}$ correctly predicting the next robot state. To improve our DNN, we will learn these tasks separately for each model by updating the weights and biases of the DNN with the well-known ADAM optimizer not re-initializing the parameters in each subsequent trial \cite{Goodfellow-et-al-2016}. The ADAM optimizer requires a loss function, which will be different for each model based on the error it makes. For $\mathrm{model}_{inv}$ the desired output is the reference state, with the error being the difference between the reference and the actual robot state ($E_{inv}=\phi-\phi_{ref}$). For $\mathrm{model}_{ff}$, the desired model output is the actual robot state, with the error being the difference between the actual and the predicted robot state ($E_{ff}=e=\phi_{pred}-\phi$). The loss function is defined as the summed squared error ($\mathcal{L}=E\frac{1}{2}E^T$). With $\mathcal{L}$ we calculate the gradients for ADAM. For regularization, we implement L2 weight decay \cite{Goodfellow-et-al-2016}. The hyperparameters for the ADAM optimizer are shown in \autoref{tab:parameters_NN}.
    
        % \input{Pseudo_code/IMC}
    
        \begin{table}[ht!]
            \small \setlength{\textfloatsep}{0.7\baselineskip plus 0.2\baselineskip minus 0.5\baselineskip}    
            \caption{Hyperparameters of the ADAM optimizer.}
            \label{tab:parameters_NN}
            \centering
            \renewcommand{\arraystretch}{1}
            \begin{tabular}{rp{0.9cm}l}
            \toprule
            Parameters & Value & Description \\ \midrule
            % \multicolumn{2}{l}{Hidden layer neuron}  & ReLU      &   \\
            % \multicolumn{2}{l}{Output layer neuron}  & $\tanh$   &   \\ 
                $\alpha$      & 0.005     & Learning rate \\ 
                $\beta_1$ & 0.9       & First moment decay	\\ 
                $\beta_2$ & 0.99      & Second moment decay	\\ 
                $\varepsilon$ & $\unit[1]{e^{-6}}$ & Division constant \\
                L2        & 0.001     & Weight decay \\ \bottomrule
            \end{tabular}
        \end{table}

Below we have summarized the most important differences between our controller conditions (see \autoref{tab:cont_comp}). For all conditions, we learn directed locomotion in a CPG network using BO to adjust the weights of the CPG network. The number of CPG weights is dependent on the number of servomotors ($k$) and neighbor pairs ($|\mathcal{N}|$) in a specific morphology. In addition, the IMC controllers also learn feedback control with their two DNN models using the ADAM optimizer. The IMC vanilla and IMC reservoir differ in the number of parameters that are adapted during feedback learning (based on the number of servomotors as well). The full code is publicly available on github \href{https://github.com/fudavd/revolve}{\underline{here}}.

To test the validity of the feedback control, we will select the final open-loop controller and the best performing IMC controller (either vanilla or reservoir) and re-test them in a noisy environment for all experiments (in total, 120 re-evaluations). The noise (a Gaussian with mean 0 and STD 0.05) will be applied on the servomotor input at every iteration. We will compare the mean difference ($\Delta$) between the open-loop and best IMC.

\begin{center}
\begin{table}[ht!]
\footnotesize
% \scriptsize
    % \setlength{\textfloatsep}{0.7\baselineskip plus 0.2\baselineskip minus 0.5\baselineskip}
    \captionsetup{width=.95\textwidth}\footnotesize
    \caption{Summary of the different controller conditions. The open-loop controller is also implemented in the two IMC controllers, which differ in the number of parameters to optimize.  \label{tab:cont_comp}}
    \centering
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{p{1.2cm} r lll}
    \toprule
       \multicolumn{2}{r}{Parameters}     & Open-loop & IMC vanilla & IMC reservoir\\ \midrule
    \scriptsize{Directed} & Controller  & CPG   & CPG  & CPG  \\
    \scriptsize{Locomotion} & Optimizer   & BO    & BO    & BO  \\
     & nr. param.   &  $k+|\mathcal{N}|$ & $k+|\mathcal{N}|$ & $k+|\mathcal{N}|$  \\\midrule
     \scriptsize{IMC} & Models  & -   & 2 DNN  & 2 DNN  \\
    \scriptsize{Conrol} & Optimizer   & -    & ADAM    & ADAM  \\
     & nr. param.   & - & $(72+48)k$ & $(8+12)k$   \\
    \bottomrule
    \end{tabular}
\end{table}
\vspace{-2em}
\end{center}
\subsection{Statistical analysis}
    For the data analysis, we compare the progression of the performance measure as a function of evaluations for all controllers (open-loop, IMC vanilla, IMC reservoir) per robot. Additionally, we compare differences between the performance end-values of each controller within a certain robot morphology, as well as a grouped comparison. Similarly, in the noisy condition, we compare the mean difference in performance ($\Delta$) between the open-loop and the best IMC per robot morphology, and aggregated in a group. Per robot morphology comparison is done using an independent samples \textit{t-test} ($N=10$), while for the grouped comparison we use a paired samples \textit{t-test} ($N$=6). Assumptions on normality and equal variance are checked by performing a Shapiro–Wilk test (normality for $p>0.95$) and an \textit{F}-test (normal ratio between variances $\frac{1}{2}$ and $2$). Additional report on the effects size are done using Cohens-\textit{d}.


==> 3/DAA_Results.tex <==
In total conducting all $180$ experiments took approximately $\unit[45]{h}$ in real-time, which is an average of $\unit[15]{min}$ per experiment. In comparison to the $\unit[900]{h}$ of simulated time this equates to a 20$\times$ speedup. In \autoref{fig:res_curve} we plotted the progression of the mean performance ($\pm\mathrm{SE}$ confidence interval) over the number of evaluations for all six robots. Four of these plots show an usual improvement over time, but the Snake and 6677 do not seem to learn much. The reason is the orientation of the robots at the start of the learning period. Unfortunately, both the snake and 6677 were placed orthogonal to the required direction to follow. This made the learning task extremely hard as they should have discovered the strategy of turning 90 degrees first and then walking into the right direction (video\footnote{\href{https://youtu.be/TgC0gHII7mg}{https://youtu.be/TgC0gHII7mg}}). Occasionally this occurred for the Snake, but not for 6677.
%Here we can see that learning occurs in all morphologies for all controllers, open-loop in blue, IMC vanilla in red, and IMC reservoir in green.  The highest mean performance at the end of the evaluations is obtained by the Gecko morphology with the IMC reservoir controller, while the lowest mean performance end-value is found in 6677 with open-loop control. 

The learning curves show that the IMC reservoir performed better or just as good as the other controllers for half of the morphologies. Furthermore the open-loop performed similarly to the IMC reservoir except for the Spider and BabyB in which it performed worse. Lastly, the IMC vanilla performed worse or just as good as the open-loop for all morphologies except for the Spider. The rate of learning is similar for all controllers at the start of the learning task (evaluations < 100), except for the Gecko in which the IMC vanilla learns slower than the others. After about 100 evaluations learning diverges for the Spider, BabyA, and BabyB.

\begin{figure}[h]\centering
\begin{minipage}[c]{0.75\textwidth}       
        \centering
        \includegraphics[width=\linewidth]{Figures/Results_curve/legend_tu_short.eps}
\end{minipage}

\begin{minipage}[c]{0.8\textwidth}
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Spider]{\includegraphics[width=\textwidth]{Figures/Results_curve/spider_tu.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Gecko]{\includegraphics[width=\textwidth]{Figures/Results_curve/gecko_tu.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Snake]{\includegraphics[width=\textwidth]{Figures/Results_curve/snake_tu.pdf}}
        \end{minipage}
\end{minipage}

\begin{minipage}[c]{0.8\textwidth}
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[BabyA]{\includegraphics[width=\textwidth]{Figures/Results_curve/babyA_tu.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[BabyB]{\includegraphics[width=\textwidth]{Figures/Results_curve/babyB_tu.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[6677]{\includegraphics[width=\textwidth]{Figures/Results_curve/6677_tu.pdf}}
        \end{minipage}
\end{minipage}
\captionsetup{width=.95\textwidth}\footnotesize
\caption{Mean learning curves ($\pm\mathrm{SE}$) of the task of directed locomotion for the Spider, Gecko, Snake, BabyA, BabyB, and 6677. The blue lines denote the open-loop controller, red lines the IMC vanilla controller, and the green lines the IMC reservoir.}
\label{fig:res_curve}
        % \vspace{-1em}
\end{figure}

Checks on the performance end-values met the requirements on normality (Shapiro-Wilk $p>0.95$), and homogeneity of variance ($\frac{1}{2}<$\textit{F}-test$<2$) between the different groups that were being compared. In \autoref{fig:res_end} we can see that there was no significant difference found between the end-values of the open-loop controller (blue bars) and the IMC reservoir (green bars) for all morphologies. Spider $p=0.24$, Gecko $p=0.36$, Snake $p=0.20$, BabyA $p=0.77$, and 6677 $p=0.90$. BabyB was closest to a statically significant difference $p=0.08$ with MEAN$\pm$STD for the OL: $0.81\pm0.55$ and IMC reservoir: $1.65\pm1.21$, effect size$=0.89$. 

When comparing the performance of the open-loop control and the IMC vanilla (red bars), no significant difference was found in the end-values for the Spider ($p=0.88$), Snake ($p=0.57$), BabyB ($p=0.63$) and 6677 ($p=0.32$) morphologies. Significant difference in learning locomotion performance was found between the open-loop control and the IMC vanilla for the 
Gecko ($p=0.02$, OL: $1.72\pm0.81$ and IMC vanilla: $0.90\pm0.48$, effect size$=1.15$), and 
BabyA ($p<0.007$, OL: $1.34\pm0.81$ and IMC vanilla: $0.50\pm0.18$, effect size$=1.43$). 

In the final comparison, no significant difference was found between the IMC vanilla and the IMC reservoir, for the Spider ($p=0.82$), Snake ($p=0.23$), and 6677 ($p=0.25$). Here, a statistically significant difference in performance end-values was found for the morphology
Gecko ($p=0.003$, IMC vanilla: $0.90\pm0.48$, and IMC reservoir: $2.11\pm0.93$, effect size$=1.63$),
BabyA ($p=0.003$, IMC vanilla: $0.50\pm0.18$, and IMC reservoir: $1.24\pm0.64$, effect size$=1.57$), and
BabyB ($p=0.05$, IMC vanilla: $0.76\pm0.32$, and IMC reservoir: $1.65\pm1.21$, effect size$=0.99$). 


\begin{figure}[ht]\centering
\begin{minipage}[c]{0.75\textwidth}       
        \centering
        \includegraphics[width=\linewidth]{Figures/Results_end/legend_tu_end_short.eps}
\end{minipage}

\begin{minipage}[c]{0.8\textwidth}
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Spider]{\includegraphics[width=\textwidth]{Figures/Results_end/spider_tu_end.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Gecko]{\includegraphics[width=\textwidth]{Figures/Results_end/gecko_tu_end.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[Snake]{\includegraphics[width=\textwidth]{Figures/Results_end/snake_tu_end.pdf}}
        \end{minipage}
\end{minipage}

\begin{minipage}[c]{0.8\textwidth}
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[BabyA]{\includegraphics[width=\textwidth]{Figures/Results_end/babyA_tu_end.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[BabyB]{\includegraphics[width=\textwidth]{Figures/Results_end/babyB_tu_end.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\textwidth}
            \centering
            \subfloat[6677]{\includegraphics[width=\textwidth]{Figures/Results_end/6677_tu_end.pdf}}
        \end{minipage}
\end{minipage}
\captionsetup{width=.95\textwidth}\footnotesize
\caption{Mean end-values ($\pm SE$) of the performance ($N=10$) per robot (Spider, Gecko, Snake, BabyA, BabyB, and 6677) for the open-loop controller (blue), IMC vanilla (red), and IMC reservoir (green). Here, * denotes $p<0.05$, and ** $p<0.01$.}
\label{fig:res_end}
        \vspace{-1em}
\end{figure}
% \vspace{-1em}
The grouped comparison ($N=6$) between the controllers did not show any statistical significant difference  between mean performance end-values over all morphologies (OL $=0.77\pm0.61$; IMC vanilla $=0.50\pm0.35$; IMC reservoir $=0.98\pm0.78$). OL vs. IMC vanilla controller $=p=0.19$; OL vs. IMC reservoir $=p=0.23$; and IMC reservoir vs. IMC vanilla $p=0.08$ (with \textit{d}$=0.79$). 

% \begin{center}
% \begin{table}[ht!]
% \footnotesize
%     % \setlength{\textfloatsep}{0.7\baselineskip plus 0.2\baselineskip minus 0.5\baselineskip}    
%     \caption{Grouped comparison of the mean end-values of the fitnesses ($\pm$STD) for each controller  (OL vs. IMC vanilla vs. IMC reservoir). For statistical analysis we performed a paired samples \textit{t-test} between each group. The corresponding  $p$-values ($\unit[]{d.f.}=10$) are shown underneath. We define significant difference at $p<0.05$ (denoted with *). Effect size was calculated using Cohens-\textit{d}}.
%     \label{tab:stats_group}
%     \centering
%     \renewcommand{\arraystretch}{1.1}
%     \begin{tabular}{l rl}
%     \toprule
%     \multirow{2}{*}{Controllers} & OL & IMC vanilla\\ 
%     & $0.77\pm0.61$ & $0.50\pm0.35$ \\ \midrule

%     $p$-value   & \multicolumn{2}{c}{0.22}
%                 \\ 
%     Cohens-\textit{d} & \multicolumn{2}{c}{0.52}
%                 \\ 
%     \bottomrule
%     \end{tabular}
%     \begin{tabular}{rl}
%     \toprule
%     OL & IMC reservoir\\ 
%     $0.77\pm0.61$ & $0.98\pm0.78$ \\ \midrule
%     \multicolumn{2}{c}{0.22}    \\ 
%     \multicolumn{2}{c}{0.31}    \\ 
%     \bottomrule
%     \end{tabular}
%     \begin{tabular}{rl}
%     \toprule
%      IMC reservoir & IMC vanilla\\ 
%     $0.98\pm0.78$ & $0.50\pm0.36$ \\ \midrule
%     \multicolumn{2}{c}{0.08}    \\ 
%     \multicolumn{2}{c}{0.79}    \\ 
%     \bottomrule
%     \end{tabular}
% \end{table}
% \end{center}

Based on the results from \autoref{fig:res_end}, we choose to compare the open-loop against the IMC reservoir controller in the noisy condition experiment. 
The results of the statistical analysis on the feedback validation experiment with added noise are shown in  \autoref{tab:stats_noise}. It should be noted that a negative difference means that the performance decreased after adding noise. Here we can see that for most morphologies the average performance decreased after adding noise (except for the $\Delta$open-loop in the 6677, and $\Delta$IMC reservoir in the BabyB morphology). Furthermore, we found that there was a statistically significant difference between the $\Delta$open-loop and the $\Delta$IMC reservoir controller for the 
Gecko ($p=0.008$, $\Delta$open-loop: -$0.66\pm0.42$, and $\Delta$IMC reservoir: -$0.18\pm0.25$, \textit{d}$=1.40$),
Snake ($p=0.03$, IMC vanilla: -$0.19\pm0.23$, and IMC reservoir: -$0.46\pm3.62\cdot e^{-2}$, \textit{d}$=1.10$), and
BabyB ($p=2.56\cdot e^{-6}$, IMC vanilla: -$0.51\pm0.20$, and IMC reservoir $=4.14\pm0.11\cdot e^{-4}$, \textit{d}$=3.10$). 

For the grouped comparison we did not find any statistical difference between the mean difference of the open-loop control and the IMC reservoir when adding noise ($p=0.08$).

\begin{center}
\begin{table}[ht!]
\scriptsize
    % \setlength{\textfloatsep}{0.7\baselineskip plus 0.2\baselineskip minus 0.5\baselineskip}    
    \caption{Mean difference ($\pm$STD) in performance after adding noise to the best controllers of each experiment ($N=10$). Negative differences indicate that the performance decreased.}
    \label{tab:stats_noise}
    \centering
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{l l l rc }
    \toprule
    Controller & $\Delta$ open-loop    & $\Delta$ IMC reservoir & $p$-value & \textit{d}\\ \midrule
    Spider  & -$0.24\pm0.29$    & -$0.03\pm0.12$    & 0.07      & 0.92 \\
    Gecko*  & -$0.66\pm0.42$    & -$0.18\pm0.25$    & <0.01     & 1.40\\
    Snake*  & -$0.19\pm0.23$    & -$0.46\pm3.62\cdot e^{-2}$ & 0.03 & 1.10\\
    BabyA   & -$0.18\pm0.38$    & -$0.27\pm0.39$    & 0.62      & 0.24\\
    BabyB*  & -$0.51\pm0.20$    & \hphantom{-}$4.14\pm0.11\cdot e^{-4}$  & <0.001 & 3.10\\
    6677    & \hphantom{-}$0.46\pm3.39\cdot e^{-3}$  & -$1.60\pm2.87\cdot e^{-3}$ & 0.18 & 0.65 \\ \midrule 
    Grouped & -$0.30\pm0.22$    & -$0.08\pm0.10$    & 0.08      & 1.24\\ 

    \bottomrule\
    \end{tabular}
\end{table}
    \vspace{-2em}
\end{center}

==> 3/EAA_Discussion.tex <==
The issue we address here is rooted in evolutionary robot systems, where robot bodies and brains evolve simultaneously. In such systems robot `birth' must be followed by `infant learning' with a robust learning method that works for all possible morphologies \cite{eiben2013triangle,eiben2020if}. Here, we consider a specific type of evolvable robots (modular morphologies) with specific controllers (based on CPGs) learning a specific task (directed locomotion). The key idea of the paper is to extend the usual open-loop controller used frequently in ER by an adaptive feedback mechanism that uses a forward model and an inverse model that can be learned on-the-fly. 

The straightforward way to test this concept would be to perform evolutionary runs with and without it. However, such runs would take enormous amounts of time. Therefore, we choose to use a test suite of six robots with various morphologies -- akin to a single generation in an ER experiment. %o  testing  machine  learning  algorithmson  a  few  data  sets  or  testing  optimization  methods  on  ahandful of objective functions.
Our experiments compare open-loop control with two versions of the extended controller on our test suite. The results show that using the IMC reservoir approach can have a positive effect on the achieved speed and the robustness of the controller compared to an open-loop controller.
%The robots in the test suite are chosen to be different to 

%for this purpose that we test on six different robot morphologies. The choice to use a test suite of $n$ robots instead of testing the learning algorithm inside an actual evolutionary process is purely practical. Running enough repetitions of complete evolutionary processes with infant learning would take far too long for such an initial study. 
%<Different Morphologies showcase the applicability of our controller within an evolutionary process, the goal was not to find out the influence on evolution but on learning??>



At the start of learning, we see similar learning curves for all controllers (\autoref{fig:res_curve}), which is to be expected since sampling was done pseudo-randomly for the first 50 samples with LHS. After this initial sampling, divergence starts around 100 evaluations in the Spider, Gecko, BabyA and BabyB, where the less performing controllers begin to plateau. The plateauing indicates to us that the end-values truly represents differences in task-performance between controllers, and were not caused by ending the experiments too soon. In support of our findings, it seems that the differences in end-values could have been more pronounced since performance in the IMC reservoir was still increasing in most morphologies. 

Overall, we did not find any significant differences between the grouped mean performance end-values. We suspect that this is mainly due to the low number of robots in our study (6 morphologies). Especially in the case of the IMC reservoir vs. IMC vanilla where there is a clear trend visible ($p=0.08$, $d=0.79$). In hindsight, this probably means that we could have increased the number of morphologies while still retaining a medium to large effect size. Additionally, the low performance of the Snake and the 6677 may have reduced the mean end-values considerately. In retrospect rotating the morphologies might have been sufficient to find a statistically significant difference between the controllers. 
A retesting in the `correct' direction did result in similar values to the Gecko and BabyB (not shown).  
%Additionally, the absence of a significant effect might also be caused by the choice of the performance function. Here, the choice of a quadratic performance measure might have been poor in hindsight since most behavior travelled less than $\unit[1]{m}$. For example, if we took a linear function (e.g. $\sqrt{\mathcal{F}}$, with unit $\unit[]{m}$) we would have seen increased differences in end-values for the Snakes and 6677.

% The low values in performance for the Snake and the 6677 greatly reduced the size of the mean difference between the controllers (\autoref{fig:res_end}). To us, this low performance was quite surprising since in previous work these morphologies performed (very) well \cite{lan2020learning}. Visual inspection of the simulated robots showed that learning did occur in these robots, but that the direction of locomotion was hard to optimize for in these models. We found in earlier work that one of the optimal movement strategies for the Snake was to roll sideways, while the 6677 performed well by hopping in a similar direction \cite{lan2020learning}. Quite remarkably the highest performance in the Snake showed a behavior in which the OL controller was able to make the snake turn 90 degrees before it started to roll sideways (resulting in an end-performance of $\unit[1.03]{m^2}$). In retrospect rotating the morphologies might have been sufficient to increase the performance tremendously (a rerun in the `correct' direction did show this).

The use of adaptive IMC has some interesting consequences for learning directed locomotion with the BO algorithm, due to the additional learning of the internal models. As the internal models change over time, we can see that the IMC controllers might behave inconsistently. This means that with retesting the same CPG weights a second time, after a period of DNN adaptations, we would likely see a slightly different behavior and thus a difference in performance. As a consequence, instead of a crisp representation of the performance, we should consider each data point more as a probability. Luckily, the BO algorithm is well equipped to do this as it evaluates samples with a certain uncertainty. Nevertheless, we did not put any extra effort into fine-tuning the BO algorithm for this, as we wanted to keep the locomotion learning equal between the controllers. 

Learning two internal models at the same time might be another cause for inconsistency. changing two interdependent systems can increase the risk of unstable adaptations that are unpredictable \cite{kawato1987hierarchical}. A way to show this is by imagining a special case in which one DNN internal model is perfect. Here it could happen that the other imperfect model causes an error that will change the weights of the perfect DNN. For future work, it might be better to learn each model differently, for example, switch which model learns for a period of time, store different sets of data in a buffer (odd vs. even samples), or imbalance the learning rates for fast vs. slow adaptation. 

Additionally, adaptations of the IMC in combination with the adaptation of the CPG weights for the locomotion task can lead to over-fitting of the DNNs. Namely, as the CPG network keeps improving its weights we will likely see that behavior converges to a (local) optimum. This may lead to the internal models recognizing which output is desired based on the robots state instead of the reference signal presented by the CPG. Resulting in bad behavior when the robot revisits the same state with a different reference signal. 
As a consequence, badly functioning feedback control causes bad performance during exploratory samples, which in return reinforces the convergence of the CPGs leading to early plateauing of the fitness.
% This reduces the fitness of exploratory samples, thereby reinforcing the early convergence of behavior and over-fitting of the DNNs. In the end, this will will lead to early plateauing in performance. 
We addressed over-fitting in the IMC with L2 regularization on the weights. Other possible solutions may be to change the BO accordingly, implementing dropout in the DNN \cite{Goodfellow-et-al-2016} or to reduce the size of the models. %The problems arising from over-fitting seem similar to those regarding continual learning. Here it has been found that models show a poor ability to adapt to new problems quicker and have difficulties in retaining acquired knowledge (also known as \textit{catastrophic forgetting}). As a solution, it has been proposed to memorize and learn on specific samples (evenly distributed in input space) rather than continuously learning on all samples which may cause convergence \cite{shin2017continual}.

Inconsistency of control can cause the resulting performance to be badly represented by the $\mathcal{GP}$ \cite{jasper2012practical}. The sample efficient nature of the BO algorithm becomes counterproductive if bad samples are regarded higher and/or good samples lower, as it will negatively affect the likelihood of samples being picked in the neighborhood of those points. 
The sensitivity to this bad sampling is different for each morphology, as a morphology with a narrow region of high performance in search space would be more sensitive than a morphology with a wider optimal region. Additionally, inconsistency in control leads to high variability in neighboring points, which can cause a very erratic and/or uncertain $\mathcal{GP}$ approximation of the fitness function. This is highly dependent on the amount of data and the type of kernel being used \cite{jasper2012practical}. Inconsistency in control will also occur in other types of feedback controller besides our IMC. For future work, we can take this into account when learning locomotion in real robots using BO. An interesting option might be to incorporate the total amount of loss by the DNNs per evaluation in the covariance matrix of the BO to directly indicate its uncertainty.


How the adaptive IMC influenced the learning locomotion task is difficult to tell. It is interesting to see that for the IMC vanilla the added feedback during learning seemed detrimental to its performance, while the IMC reservoir seemed to benefit. The differences in the number of parameters to be learned (\autoref{tab:cont_comp}) result in a reduced amount of learning capabilities and an increased rate of learning for the DNNs in the IMC reservoir \cite{lukovsevivcius2009reservoir}. The difference in performance indicates that there might be an optimal amount of learning for the IMC. For example, to prevent over-fitting one would like to have a DNN with a slow learning rate and low learning capacity, but, taking this into the extreme might lead to bad adaptations towards new behaviors and limitations in the complexity of the model. Additionally, slow adaptations increases the robustness of the feedback controller, while fast adaptation can cause it to adapt better to changes in control.

The fact that the IMC reservoir outperforms the open-loop controller also indicates that some inconsistencies in control can be beneficial. It can be argued that the aforementioned argument, \textit{bad samples are regarded higher and/or good samples lower} is conversely beneficial, but we disagree. Even though higher valued good samples might attract more samples in their neighborhood, bad samples would already be regarded as bad and ignored by the BO, thus not affecting the outcome at all. In the end, this would cause the net influence of inconsistencies to be more harmful than good. We, believe the source of improvement to lie in an increase in the amount of uncertainty of the $\mathcal{GP}$ for the IMC reservoir. This would encourage more exploration, which explains the extended periods of learning.

We tested the validity of our feedback controller in the added noise experiments. The results show that the IMC reservoir controller is able to reduce the effects of the perturbation more than the open-loop in the Gecko, Snake, and BabyB morphology. Differences between $\Delta$fitness was most apparent in the BabyB with a huge effect size ($d=3.1$). Overall, we found that the IMC reservoir tends to perform better ($p=0.08$, with very large effect size $d=1.24$). This difference was mainly caused by a deviation from the target direction (decrease in $\mathcal{D}_{dir}$ and increase in $\mathcal{D}_{dev}$, not shown). For the open-loop controller in BabyA the addition of noise does not seem to affect it that much. Visual inspection of these controllers with and without noise (same \href{https://youtu.be/TgC0gHII7mg}{video}) did not reveal anything noticeable. Noteworthy, the reduction in performance of the best movement behavior in the open-loop Snake (the one that rotated 90 degrees first) was due to a failure in rotation before rolling. This strengthens our belief that learning with open-loop leads to exploitation of behaviors that are very sensitive to the reality gap. 

Many controllers that were evolved in ER literature seem to have a problem with bridging the reality gap \cite{jakobi1995noise}. The results of our experiments revealed that small changes in controllers can lead to very different results in performance, which will eventually affect the whole ER process. In this paper, we addressed this issue in two ways simultaneously with our IMC implementation. First of all, we learned directed locomotion on a more realistic robot that uses feedback control instead of open-loop control. Secondly, the added feedback allows for more robust control in the sense that the effects of perturbations and noise on the robots are being actively reduced. Several other solutions to the reality gap have been proposed which we did not cover \cite{jakobi1995noise}. As a consequence, we may have overestimated the effect of the IMC reservoir on its ability to reduce the reality gap. We ignored these techniques as we were only interested to see the capabilities of the IMC controller and its effect on learning directed locomotion.

The necessity of a learning loop in ER is based on the difficulties that arise with simultaneous body and brain evolution \cite{lipson2016difficulty,eiben2013triangle}. Learning prevents potentially good morphologies with initially bad controllers to be discarded right away, which allows for `hard to control' morphologies to be more present. Another approach that has been proposed is protecting new morphologies that have recently been mutated during selection \cite{cheney2018scalable}. Here, controller adaptation to occur within the evolutionary process rather than an additional learning loop. For simple morphologies this method seems to work, but \cite{cheney2018scalable} noted that for larger creatures novelty protection is only beneficial with a minimum mutation threshold (which was obtained by a parameter sweep). The advantage of learning over novelty protection is the speed and scalability to more complex morphologies (as such tuning is not required beforehand). For further research we would like to test lifetime learning with IMC within an fully evolving robot system.



==> 3/FAA_Conclusion.tex <==
The advances of 3D-printing, rapid prototyping and automated assembly make Evolutionary Robotics with physical robots increasingly feasible. This implies that using realistic feedback control in the robots is becoming more important. To this end, we developed a bio-inspired IMC feedback system based on two internal models that can be learned on-the-fly. Our experiments showed that adding this system to existing controllers helps learn proper movement execution without hampering the learning of a locomotion task. The system also can reduce the learning effort and increase the robustness of the learned controllers. 

==> 3/Figures/CPG_net.tex <==
\centering
\resizebox{0.75\textwidth}{!}{%
\begin {tikzpicture}
	    [
		auto,
		node distance =0.33cm and 0.35cm,
		on grid,
		thick,
		state/.style = {circle,draw,inner sep=0pt, minimum width = 0.35 cm},
		box/.style={rectangle,draw,minimum width = 0.3 cm, minimum size=0.3 cm},
		core/.style={rectangle,draw=red!60,fill=red!5,very thick,minimum width = 0.6 cm, minimum size=0.6 cm}]
	\node[box] (B_l1) {};
	\node[state] (O4) [right = of B_l1] {$4$};
	\node[box] (B_l2) [right = of O4] {};
	\node[state] (O3) [right = of B_l2] {$3$};
	\node[core] (core) [right = 0.49cm of O3] {};
	\node[state] (O2) [above=0.48cm of core] {$2$};
	\node[box] (B_t2) [above=of O2] {};
	\node[state] (O1) [above=of B_t2] {$1$};
	\node[box] (B_t1) [above=of O1] {};
	\node[state] (O6) [right= 0.49cm of core] {$6$};
	\node[box] (B_r2) [right= of O6] {};
	\node[state] (O5) [right=of B_r2] {$5$};
	\node[box] (B_r1) [right=of O5] {};
	\node[state] (O8) [below=0.48cm of core] {$8$};
	\node[box] (B_b2) [below=of O8] {};
	\node[state] (O7) [below=of B_b2] {$7$};
	\node[box] (B_b1) [below=of O7] {};
	\path[draw=blue] (O4.10) to node [] {} (O3.170);
	\path[draw=blue] (O3.-170) to node [] {} (O4.-10);
	\path[draw=blue] (O6.10) to node [] {} (O5.170);
	\path[draw=blue] (O5.-170) to node [] {} (O6.-10);
	\path[draw=blue] (O2.100) to node [] {} (O1.-100);
	\path[draw=blue] (O1.-80) to node [] {} (O2.80);
	\path[draw=blue] (O7.100) to node [] {} (O8.-100);
	\path[draw=blue] (O8.-80) to node [] {} (O7.80);
	\path[draw=blue] (O3.50) to node [] {} (O2.-140);
	\path[draw=blue] (O2.-120) to node [] {} (O3.30);
	\path[draw=blue] (O3.10) to node [] {} (O6.170);
	\path[draw=blue] (O6.-170) to node [] {} (O3.-10);
	\path[draw=blue] (O3.10) to node [] {} (O6.170);
	\path[draw=blue] (O6.-170) to node [] {} (O3.-10);
	\path[draw=blue] (O6.150) to node [] {} (O2.-60);
	\path[draw=blue] (O2.-40) to node [] {} (O6.130);
	\path[draw=blue] (O2.-80) to node [] {} (O8.80);
	\path[draw=blue] (O8.100) to node [] {} (O2.-100);
	\path[draw=blue] (O6.-130) to node [] {} (O8.40);
	\path[draw=blue] (O8.60) to node [] {} (O6.-150);
	\path[draw=blue] (O6.-130) to node [] {} (O8.40);
	\path[draw=blue] (O8.60) to node [] {} (O6.-150);
	\path[draw=blue] (O3.-30) to node [] {} (O8.120);
	\path[draw=blue] (O8.140) to node [] {} (O3.-50);
	\end {tikzpicture}
}

==> 3/Figures/FlowIMC.tex <==
\begin{figure*}[h]
{
    \begin {tikzpicture}

%		\node(Text2)[text width=10cm, below of = pro1, yshift = -2cm]     {Gongjin's controller design:};		\node (pro3) [process,below of =Text2] {CPG?};		\node (pro4) [process, right of = pro3, xshift=3cm] {Robot};		\node [support, right of = pro4, xshift=2.5cm]    (last_S2)   {};		\draw [arrow] (pro3) -- node [anchor=south] {$u_i$}(pro4);		\draw [arrow] (pro4) -- node [anchor=south] {$y_i$}(last_S2);		\draw [arrow] (pro4) -| ([shift = {(1cm,-1cm)}]pro4.south east) -- ([shift={(-1cm,-1cm)}]pro3.south west) |-(pro3); %
		
		\node(Text2)[text width=10cm, below of = pro1, yshift = -1cm]     {Closed loop controller design:};
		\node (sum1)    [sum    , below of = Text2] {};
		\node (pro5)    [process, left of = sum1, xshift= -2cm] {CPG};
		\node (pro6)    [process, right of = sum1, xshift= 1.75cm] {inv. model};
		\node (pro7)    [process, right of = pro6, xshift=3cm] {Robot};
		\node (pro8)    [process, below of = pro7, yshift = -.5cm] {ff. model};
		\node (last_S3) [support, right of = pro7, xshift= 3 cm]       {};
		\node (sum2)    [sum, right of=pro8, xshift= 1.75cm] {};
		
		\draw [arrow] (pro5) -- node [anchor=south] {$\phi_{ref,i}$}  node[pos=0.95, anchor = north] {{\tiny $+$}}(sum1);
		\draw [arrow] (sum1) -- node [anchor=south] {}(pro6);
		\draw [arrow] (pro6) -- node [anchor=south] {$u_i$}(pro7);
		\draw [arrow] (pro6) -| ([shift = {(.5cm,-.25cm)}]pro6.south east) |-(pro8);
		\draw [arrow] (pro7) -- node [anchor=south] {$\phi_i$}(last_S3);
		\draw [arrow] (pro7) -| node [anchor=south] {} node[pos=0.95, anchor = east] {{\tiny $+$}}(sum2);
		\draw [arrow] (pro8) -- node [anchor=south] {$\phi_{pred,i}$} node[pos=0.95, anchor = north] {{\tiny $-$}}(sum2);
		\draw [arrow] (sum2) |- ([shift = {(0cm, -2cm)}]pro6.south) -| node [anchor=south west] {$error_i$} node[pos=0.98, anchor = west] {{\tiny $-$}}(sum1);
    \end{tikzpicture}
\caption{\label{fig:Flow} 
Schematic flow chart of the closed loop IMC design. Similarly, the CPG produces a movement pattern for locomotion, in this case a preferred state \textit{i.e.} reference state $\phi_{ref,i}$ for each servomotor $i$. The inverse model (inv. model) calculates the required servomotor input  $u_i$ to get to this state. Based on this input the feedforward model (ff. model) predicts the robot's state $\phi_{pred,i}$. The difference between the predicted state and the actual state $\phi_{i}$ gets send back to the inverse model.}}
\end{figure*}


==> 3/Figures/FlowOL.tex <==
% \begin{figure}[h]
% {
\centering
\resizebox{0.75\textwidth}{!}{%
    \begin {tikzpicture}[]
        \node(Text1)[text width=10cm] at (0,0) {\LARGE \textbf{Open loop controller design:}};
		\node (pro1) [process,below of = Text1] {\LARGE CPG};
		\node (pro2) [process, right of = pro1, xshift=3cm] {\LARGE Robot};
		\node (last_S1) [right of = pro2, xshift=2.5cm]       {};
		\draw [arrow] (pro1) -- node [anchor=south] {\LARGE $u$}(pro2);
		\draw [arrow] (pro2) -- node [anchor=south] {\LARGE $\phi$}(last_S1);
		
		
		\node(Text2)[text width=10cm, below of = pro1, yshift = -.25cm] 
    {\LARGE \textbf{Adaptive IMC design:}};
		\node (sum1)    [sum    , below of = Text2] {};
		\node (pro5)    [process, left of = sum1, xshift= -2cm] {\LARGE CPG};
		\node (pro6)    [process, right of = sum1, xshift= 1.75cm] {\LARGE $\mathrm{model}_{inv}$};
		\node (pro7)    [process, right of = pro6, xshift=3cm] {\LARGE Robot};
		\node (pro8)    [process, below of = pro7, yshift = -.5cm] {\LARGE  $\mathrm{model}_{ff}$};
		\node (last_S3) [right of = pro7, xshift= 3 cm]       {};
		\node (sum2)    [sum, right of=pro8, xshift= 1.85cm] {};
		
		\draw [arrow] (pro5) -- node [anchor=south] {\LARGE $\phi_{ref}$}  node[pos=0.95, anchor = north, below] {{\large $+$}}(sum1);
		\draw [arrow] (sum1) -- node [anchor=south] {}(pro6);
		\draw [arrow] (pro6) -- node [anchor=south] {\LARGE $u$}(pro7);
		\draw [arrow] (pro6) -| ([shift = {(.5cm,-.25cm)}]pro6.south east) |-(pro8);
		\draw [arrow] (pro7) -- node [anchor=south, xshift= 0.1cm] {\LARGE $\phi$}(last_S3);
		\draw [arrow] (pro7) -| node [anchor=south] {} node[pos=0.95, anchor = east, right] {{\large $+$}}(sum2);
		\draw [arrow] (pro8) -- node [anchor=south] {\LARGE $\phi_{pred}$} node[pos=0.95, anchor = north] {{\large $-$}}(sum2);
		\draw [arrow] (sum2) |- ([shift = {(0cm, -2cm)}]pro6.south) -| node [anchor=south west] {\LARGE $e$} node[pos=0.98, anchor = west] {{\large $-$}}(sum1);
		

    \end{tikzpicture}
}


==> 3/Figures/Timeline.tex <==
\begin{figure}[h!]
{
    \begin {tikzpicture}[node distance=1cm]
        \foreach \x in {-1,...,12}
        %  \draw[dotted, color=Gray] ({\x*2},-6) -- ({\x*2},3)
        %  \filldraw ({\x+0.5},-6) circle (2pt)
         \fill[fill=yellow!20!white] ({\x+-.25},-6) rectangle ({\x+0.25},3.5);
        
        
        % PO
        \filldraw[color=black] (0,3) -- (9.5,3)
        (-3.00,3) node[align=center,right] {PO}
        
        (0,3) circle (2pt) node[align=center,above]{[\citenum{lee1996hybrid}]}
        (2,3) circle (2pt) node[align=center,above]{[\citenum{lee2000evolving}]}
        (3.5,3) circle (2pt) node[align=center,above]{[\citenum{lee2003evolving}]}
        (7.5,3) circle (2pt) node[align=center,above]{[\citenum{larpin2011co}]}
        (8,3) circle (2pt) node[align=center,above]{[\citenum{auerbach2012relationship}]}
        (9.5,3) circle (2pt) node[align=right,above]{[\citenum{samuelsen2015real}]};
        
        % GOLEM and GenoBots
        \filldraw[color=black] (2,2) -- (5,2)
        (-3.00,2) node[align=center,right] {GOLEM/\\ \newline GenoBots}
        
        (2,2) circle (2pt) node[align=center,above]{[\citenum{pollack2000golem,lipson2000automatic}]}
        (2.5,2) circle (2pt) node[align=center,below]{[\citenum{hornby2001body}]}
        (3.5,2) node[align=center,above]{[\citenum{pollack2003computer}]}
        (3.5,2) circle (2pt) node[align=center,below]{[\citenum{pollack2003computer}]}
        (5,2) circle (2pt) node[align=center,below]{[\citenum{lipson2006evolving}]};
        
        % LEGO
        \filldraw[color=black] (1,0.5) -- (9.5,0.5)
        (-3.00,0.5) node[align=center,right] {LEGO}
        
        (1,0.5) circle (2pt) node[align=center,above]{[\citenum{lund1998evolutionary}]}
        (3,0.5) circle (2pt) node[align=center,above]{[\citenum{chirikjian2002self}]}
        (3.5,0.5) circle (2pt) node[align=center,above]{[\citenum{lund2003co}]}
        (4,0.5) circle (2pt) node[align=center,above]{[\citenum{macinnes2004crawling}]}
        (9.5,0.5) circle (2pt) node[align=center,above]{[\citenum{poikselka2015evolutionary}]};
        
        
        % Tensegrity
        \filldraw[color=black] (4.5,-.5) -- (9,-.5)
        (-3.00,-.5) node[align=center,right] {Tensegrity}
        
        (4.5,-.5) circle (2pt) node[align=center,above]{[\citenum{paul2005evolutionary}]}
        (5,-.5) circle (2pt) node[align=center,above]{[\citenum{paul2006design}]}
        (7,-.5) circle (2pt) node[align=center,above]{[\citenum{lobo2010evolutionary}]}
        (8.5,-.5) circle (2pt) node[align=center,above]{[\citenum{iscen2013controlling}]}
        (9,-.5) circle (2pt) node[align=center,above]{[\citenum{khazanov2014evolution}]}
        (9,-.5) circle (2pt) node[align=center,below]{[\citenum{bruce2014design}]};
        
        % HomoGen
        \filldraw[color=black] (5,-1.5) -- (11,-1.5)
        (-3.00,-1.5) node[align=center,right] {Homogen.}
        
        % molecubes
            (5.5,-1.5) circle (2pt) node[align=center,below]{\color{MidnightBlue}[\citenum{zykov2007evolved}]}
            (6,-1.5) circle (2pt) node[align=center,below]{\color{MidnightBlue}[\citenum{zykov2008molecubes}]}
            (7,-1.5) circle (2pt) node[align=center,below]{\color{MidnightBlue}[\citenum{zhong2010modular}]}
        % Yamor
            (5,-1.5) circle (2pt) node[align=center,above]{\color{BrickRed}[\citenum{mockel2006yamor}]}
            (6,-1.5) circle (2pt) node[align=center,above]{\color{BrickRed}[\citenum{sproewitz2008learning}]}
            (8.5,-1.5) circle (2pt) node[align=center,above]{\color{BrickRed}[\citenum{d2013online}]}
        %Y1
            (5,-1.5) circle (2pt) node[align=center,below]{\color{ForestGreen}[\citenum{gonzalez2006motion}]}
            (7.5,-1.5) circle (2pt) node[align=center,below]{\color{ForestGreen}[\citenum{ranganath2011distributed}]}
        % SMORES 
            (8,-1.5) circle (2pt) node[align=center,below]{\color{orange}[\citenum{davey2012emulating}]}
            (11,-1.5) circle (2pt) node[align=center,below]{\color{orange}[\citenum{tosun2018computer}]}
        % EMeRGe
            (10.5,-1.5) circle (2pt) node[align=center,above]{\color{VUblue}[\citenum{moreno2017emerge,veenstra2017evolution}]};
        
        % EDHMoR
        \filldraw[color=black] (7.5,-3) -- (9.5,-3)
        (-3.00,-3) node[align=center,right] {Heterogen.}
        
        (7.5,-3) circle (2pt) node[align=center,above]{[\citenum{faina2011first}]}
        (8.5,-3) circle (2pt) node[align=center,above]{[\citenum{faina2013edhmor}]}
        (9,-3) circle (2pt) node[align=center,above]{[\citenum{faina2014towards}]}
        (9.5,-3) circle (2pt) node[align=center,above]{[\citenum{faina2015evolution}]}; 
        
        % RoboGen
        \filldraw[color=black] (9,-4) -- (12,-4)
        (-3.00,-4) node[align=center,right] {RoboGen}
        
        (9,-4) circle (2pt) node[align=center,above]{[\citenum{auerbach2014robogen}]}
        (10,-4) circle (2pt) node[align=center,above]{[\citenum{jelisavcic2016improving}]}
        (10.5,-4) circle (2pt) node[align=center,above]{[\citenum{jelisavcic2017real}]}
        (11,-4) circle (2pt) node[align=center,above]{[\citenum{hupkes2018revolve}]}
        (11,-4) circle (2pt) node[align=center,below]{[\citenum{miras2018effects}]}
        (11.5,-4) node[align=center,below]{[\citenum{miras2019effects}]}
        (11.5,-4) circle (2pt) node[align=center,above]{[\citenum{jelisavcic2019lamarckian}]}
        (12,-4) circle (2pt) node[align=center,above]{[\citenum{lan2020learning}]}; 
        
        % Other
        \filldraw[color=black] 
        % (9.5,-5) -- (11.5,-5)
        (-3.00,-5) node[align=center,right] {Other}
        
        (-1,-5) circle (2pt) node[align=center, above]{[\citenum{sims1994evolving}]}

        (9,-5) circle (2pt) node[align=center,below]{[\citenum{cheney2014unshackling}]}

        (9.5,-5) circle (2pt) node[align=center,above]{[\citenum{brodbeck2015morphological}]}
        (10.5,-5) node[align=center,above]{[\citenum{vujovic2017evolutionary}]}
        
        (10.5,-5) circle (2pt) node[align=center,below]{[\citenum{cellucci20171d}]}
        (11.5,-5) circle (2pt) node[align=center,above]{[\citenum{hale2019robot}]}
        
        (12,-5) circle (2pt) node[align=center,below]{[\citenum{Kriegman1853}]};
        % Year
        \filldraw
            (-1.25,-6) node {}--
            (-1,-6) circle (2pt) node[align=center, below] {1994} --
            (0,-6) circle (2pt) node[align=center, below] {1996} --
            (1,-6) circle (2pt) node[align=center, below] {1998} --
            (2,-6) circle (2pt) node [align=center, below] {2000} --
            (3,-6) circle (2pt) node[align=center, below] {2002} --
            (4,-6) circle (2pt) node[align=center, below] {2004} --
            (5,-6) circle (2pt) node[align=center, below] {2006} --
            (6,-6) circle (2pt) node[align=center, below] {2008} --
            (7,-6) circle (2pt) node[align=center, below] {2010} --
            (8,-6) circle (2pt) node[align=center, below] {2012} --
            (9,-6) circle (2pt) node[align=center, below] {2014} --
            (10,-6) circle (2pt) node[align=center, below] {2016} --
            (11,-6) circle (2pt) node[align=center, below] {2018} --
            (12,-6) circle (2pt) node[align=center, below] {2020}--
            (12.25,-6);
        
        % \foreach \x in {0,.5,...,12} 
            % \draw[dotted] (\x,-4.025) -- (\x,3.025);

        \filldraw[color=\color{MidnightBlue}] 
            (12.5,-1.0) circle (2.5pt);
            \draw (12.5,-1.0) node[align=center, right] {\footnotesize\color{Black} \textbf{MoleCubes}}; 
            
        \filldraw[color=\color{ForestGreen}]  
            (12.5,-1.25) circle (2.5pt);
            \draw (12.5,-1.25) node[align=center, right] {\footnotesize\color{Black} \textbf{Y1}}; 
            
        \filldraw[color=\color{BrickRed}]  
            (12.5,-1.5) circle (2.5pt);
            \draw (12.5,-1.5) node[align=center, right] {\footnotesize\color{Black} \textbf{YaMoR}}; 
            
        \filldraw[color=\color{VUblue}]  
            (12.5,-1.75) circle (2.5pt);
            \draw (12.5,-1.75) node[align=center, right] {\footnotesize\color{Black} \textbf{EMeRGe}};
            
        \filldraw[color=\color{orange}]  
            (12.5,-2.0) circle (2.5pt);
            \draw (12.5,-2.0) node[align=center, right] {\footnotesize\color{Black} \textbf{SMORES}};
    \end{tikzpicture}
\caption{\label{fig:Timeline} 
Timeline of the progression of different types of morphological designs in the Evolutionary Robotics literature that use a modular framework. PO stands for Parameter Optimization. Note that the Homogeneous robot comprise of different modules}}
\end{figure}


==> 3/Figures/Timeline_old.tex <==
\begin{figure}[h!]
{
    \begin {tikzpicture}[node distance=1cm]
        \foreach \x in {-1,...,12}
        %  \draw[dotted, color=Gray] ({\x*2},-6) -- ({\x*2},3)
        %  \filldraw ({\x+0.5},-6) circle (2pt)
         \fill[fill=yellow!20!white] ({\x+-.25},-6) rectangle ({\x+0.25},3.5);
        
        
        % PO
        \filldraw[color=black] (0,3) -- (9.5,3)
        (-3.00,3) node[align=center,right] {PO}
        
        (0,3) circle (2pt) node[align=center,above]{\citenum{lee1996hybrid}}
        (2,3) circle (2pt) node[align=center,above]{\citenum{lee2000evolving}}
        (3.5,3) circle (2pt) node[align=center,above]{\citenum{lee2003evolving}}
        (7.5,3) circle (2pt) node[align=center,above]{\citenum{larpin2011co}}
        (8,3) circle (2pt) node[align=center,above]{\citenum{auerbach2012relationship}}
        (9.5,3) circle (2pt) node[align=right,above]{\citenum{samuelsen2015real}};
        
        % GOLEM and GenoBots
        \filldraw[color=black] (2,2) -- (5,2)
        (-3.00,2) node[align=center,right] {GOLEM/\\ \newline GenoBots}
        
        (2,2) circle (2pt) node[align=center,above]{\citenum{pollack2000golem,lipson2000automatic}}
        (2.5,2) circle (2pt) node[align=center,below]{\citenum{hornby2001body}}
        (3.5,2) node[align=center,above]{\citenum{pollack2003computer}}
        (3.5,2) circle (2pt) node[align=center,below]{\citenum{pollack2003computer}}
        (5,2) circle (2pt) node[align=center,below]{\citenum{lipson2006evolving}};
        
        % LEGO
        \filldraw[color=black] (1,0.5) -- (9.5,0.5)
        (-3.00,0.5) node[align=center,right] {LEGO}
        
        (1,0.5) circle (2pt) node[align=center,above]{\citenum{lund1998evolutionary}}
        (3,0.5) circle (2pt) node[align=center,above]{\citenum{chirikjian2002self}}
        (3.5,0.5) circle (2pt) node[align=center,above]{\citenum{lund2003co}}
        (4,0.5) circle (2pt) node[align=center,above]{\citenum{macinnes2004crawling}}
        (9.5,0.5) circle (2pt) node[align=center,above]{\citenum{poikselka2015evolutionary}};
        
        
        % Tensegrity
        \filldraw[color=black] (4.5,-.5) -- (9,-.5)
        (-3.00,-.5) node[align=center,right] {Tensegrity}
        
        (4.5,-.5) circle (2pt) node[align=center,above]{\citenum{paul2005evolutionary}}
        (5,-.5) circle (2pt) node[align=center,above]{\citenum{paul2006design}}
        (7,-.5) circle (2pt) node[align=center,above]{\citenum{lobo2010evolutionary}}
        (8.5,-.5) circle (2pt) node[align=center,above]{\citenum{iscen2013controlling}}
        (9,-.5) circle (2pt) node[align=center,above]{\citenum{khazanov2014evolution}}
        (9,-.5) circle (2pt) node[align=center,below]{\citenum{bruce2014design}};
        
        % HomoGen
        \filldraw[color=black] (5,-1.5) -- (11,-1.5)
        (-3.00,-1.5) node[align=center,right] {Homogen.}
        
        % molecubes
            (5.5,-1.5) circle (2pt) node[align=center,below]{\color{MidnightBlue}\citenum{zykov2007evolved}}
            (6,-1.5) circle (2pt) node[align=center,below]{\color{MidnightBlue}\citenum{zykov2008molecubes}}
            (7,-1.5) circle (2pt) node[align=center,below]{\color{MidnightBlue}\citenum{zhong2010modular}}
        % Yamor
            (5,-1.5) circle (2pt) node[align=center,above]{\color{BrickRed}\citenum{mockel2006yamor}}
            (6,-1.5) circle (2pt) node[align=center,above]{\color{BrickRed}\citenum{sproewitz2008learning}}
            (8.5,-1.5) circle (2pt) node[align=center,above]{\color{BrickRed}\citenum{d2013online}}
        %Y1
            (5,-1.5) circle (2pt) node[align=center,below]{\color{ForestGreen}\citenum{gonzalez2006motion}}
            (7.5,-1.5) circle (2pt) node[align=center,below]{\color{ForestGreen}\citenum{ranganath2011distributed}}
        % SMORES 
            (8,-1.5) circle (2pt) node[align=center,below]{\color{orange}\citenum{davey2012emulating}}
            (11,-1.5) circle (2pt) node[align=center,below]{\color{orange}\citenum{tosun2018computer}}
        % EMeRGe
            (10.5,-1.5) circle (2pt) node[align=center,above]{\color{VUblue}\citenum{moreno2017emerge,veenstra2017evolution}};
        
        % EDHMoR
        \filldraw[color=black] (7.5,-3) -- (9.5,-3)
        (-3.00,-3) node[align=center,right] {Heterogen.}
        
        (7.5,-3) circle (2pt) node[align=center,above]{\citenum{faina2011first}}
        (8.5,-3) circle (2pt) node[align=center,above]{\citenum{faina2013edhmor}}
        (9,-3) circle (2pt) node[align=center,above]{\citenum{faina2014towards}}
        (9.5,-3) circle (2pt) node[align=center,above]{\citenum{faina2015evolution}}; 
        
        % RoboGen
        \filldraw[color=black] (9,-4) -- (12,-4)
        (-3.00,-4) node[align=center,right] {RoboGen}
        
        (9,-4) circle (2pt) node[align=center,above]{\citenum{auerbach2014robogen}}
        (10,-4) circle (2pt) node[align=center,above]{\citenum{jelisavcic2016improving}}
        (10.5,-4) circle (2pt) node[align=center,above]{\citenum{jelisavcic2017real}}
        (11,-4) circle (2pt) node[align=center,above]{\citenum{hupkes2018revolve}}
        (11,-4) circle (2pt) node[align=center,below]{\citenum{miras2018effects}}
        (11.5,-4) node[align=center,below]{\citenum{miras2019effects}}
        (11.5,-4) circle (2pt) node[align=center,above]{\citenum{jelisavcic2019lamarckian}}
        (12,-4) circle (2pt) node[align=center,above]{\citenum{lan2020learning}}; 
        
        % Other
        \filldraw[color=black] 
        % (9.5,-5) -- (11.5,-5)
        (-3.00,-5) node[align=center,right] {Other}
        
        (-1,-5) circle (2pt) node[align=center, above]{\citenum{sims1994evolving}}

        (9,-5) circle (2pt) node[align=center,below]{\citenum{cheney2014unshackling}}

        (9.5,-5) circle (2pt) node[align=center,above]{\citenum{brodbeck2015morphological}}
        (10.5,-5) node[align=center,above]{\citenum{vujovic2017evolutionary}}
        
        (10.5,-5) circle (2pt) node[align=center,below]{\citenum{cellucci20171d}}
        (11.5,-5) circle (2pt) node[align=center,above]{\citenum{hale2019robot}}
        
        (12,-5) circle (2pt) node[align=center,below]{\citenum{Kriegman1853}};
        % Year
        \filldraw
            (-1.25,-6) node {}--
            (-1,-6) circle (2pt) node[align=center, below] {1994} --
            (0,-6) circle (2pt) node[align=center, below] {1996} --
            (1,-6) circle (2pt) node[align=center, below] {1998} --
            (2,-6) circle (2pt) node [align=center, below] {2000} --
            (3,-6) circle (2pt) node[align=center, below] {2002} --
            (4,-6) circle (2pt) node[align=center, below] {2004} --
            (5,-6) circle (2pt) node[align=center, below] {2006} --
            (6,-6) circle (2pt) node[align=center, below] {2008} --
            (7,-6) circle (2pt) node[align=center, below] {2010} --
            (8,-6) circle (2pt) node[align=center, below] {2012} --
            (9,-6) circle (2pt) node[align=center, below] {2014} --
            (10,-6) circle (2pt) node[align=center, below] {2016} --
            (11,-6) circle (2pt) node[align=center, below] {2018} --
            (12,-6) circle (2pt) node[align=center, below] {2020}--
            (12.25,-6);
        
        % \foreach \x in {0,.5,...,12} 
            % \draw[dotted] (\x,-4.025) -- (\x,3.025);

        \filldraw[color=\color{MidnightBlue}] 
            (12.5,-1.0) circle (2.5pt);
            \draw (12.5,-1.0) node[align=center, right] {\footnotesize\color{Black} \textbf{MoleCubes}}; 
            
        \filldraw[color=\color{ForestGreen}]  
            (12.5,-1.25) circle (2.5pt);
            \draw (12.5,-1.25) node[align=center, right] {\footnotesize\color{Black} \textbf{Y1}}; 
            
        \filldraw[color=\color{BrickRed}]  
            (12.5,-1.5) circle (2.5pt);
            \draw (12.5,-1.5) node[align=center, right] {\footnotesize\color{Black} \textbf{YaMoR}}; 
            
        \filldraw[color=\color{VUblue}]  
            (12.5,-1.75) circle (2.5pt);
            \draw (12.5,-1.75) node[align=center, right] {\footnotesize\color{Black} \textbf{EMeRGe}};
            
        \filldraw[color=\color{orange}]  
            (12.5,-2.0) circle (2.5pt);
            \draw (12.5,-2.0) node[align=center, right] {\footnotesize\color{Black} \textbf{SMORES}};
    \end{tikzpicture}
\caption{\label{fig:Timeline} 
Timeline of the progression of different types of morphological designs in the Evolutionary Robotics literature that use a modular framework. PO stands for Parameter Optimization. Note that the Homogeneous robot comprise of different modules}}
\end{figure}


==> 3/Pseudo_code/BO.tex <==
\begin{algorithm}[!ht]

  \caption{Bayesian optimization for learning the weights of CPG controllers.}
  \label{alg:bo}
  \begin{algorithmic}[1]
    \State Initiate $n$ initial samples: $\bm{X}=\left[ \bm{\vec{w}}_1, \bm{\vec{w}}_2, \dots, \bm{\vec{w}}_n \right] $ \Comment{with $n = 50$ pseudo-random samples by LHS}
    \State Obtain $n$ initial fitnesses: $\bm{Y}=\left[ \mathcal{F}_1, \mathcal{F}_2, \dots, \mathcal{F}_n \right]$ \Comment{using \autoref{eq:fitness}}
    \State Approximate the objective function: $f(\bm{\vec{w}}) \sim \mathcal{GP}\left(\mu(\bm{X}), \sigma^2(\bm{X})\right)$
    \For {$k = n+1,n+2, ...$}  \Comment{for  evaluation $k$}
    \State Select new sample $\bm{\vec{w}}_k$ based on approximation $f\left(\Vec{\bm{w}}|\bm{Y}\right)$:
     \[ \bm{\vec{w}}_k = \arg\max_{\bm{\vec{w}}_k}  a\left(f(\Vec{\bm{w}}_k),\bm{Y}\right)\]
    \State Obtain the new sample fitness $\mathcal{F}_k(\bm{\vec{w}}_k)$
    \State Append the data $\bm{X} = \left[\bm{X}, \bm{\vec{w}}_k\right], \quad \bm{Y} = \left[\bm{Y}, \mathcal{F}_k \right]$
    \State Update the approximation: $f(\bm{\vec{w}}) \sim \mathcal{GP}\left(\mu(\bm{X}), \sigma^2(\bm{X})\right)$
    \EndFor
    \State \textbf{return} data $\bm{X}, \bm{Y}, f(\bm{\vec{w}})$
  \end{algorithmic}
\end{algorithm}

==> 3/Pseudo_code/IMC.tex <==
\begin{algorithm}[!ht]
  \caption{IMC update rule for timestep $t=0,1,2,\dots,t_{end}$}
  \label{IMC_upd}
  \begin{algorithmic}[1]
    \For{$t=0,1,2,\dots,t_{end}$}
        \State Obtain the reference state vector:  $\vec{\bm{y}}_{ref,t} = $ CPG$(t)$ \Comment{with $\vec{\bm{y}} = [\phi_{1:k},\dot{\phi}_{1:k}]$}
        \State Obtain the current state vector: $\vec{\bm{y}}_{t}= proprioception(t)$
        \State Calculate the prediction error: $error_{ff,t}=\vec{\bm{y}}_t-\vec{\bm{y}}_{ref,t}$
        \State Calculate the movement error:
        $error_{inv,t}=\vec{\bm{y}}_{pred,t}-\vec{\bm{y}}_t$
        \State Update the models: 
        ADAM($\mathrm{model}_{inv},error_{inv,t}$); ADAM($\mathrm{model}_{ff},error_{ff,t}$)
    \newline \textbf{Calculate for next iteration step}
        \State Calculate the motor input: 
        $\vec{\bm{u}}_t=\mathrm{model}_{inv}(\vec{\bm{y}}_{ref,t},\vec{\bm{y}}_{t},error_{move,t}$)
        \State Predict the next state: $\vec{\bm{y}}_{pred,t+1}=\mathrm{model}_{ff}(\vec{\bm{y}}_t,\vec{\bm{u}}_t)$ 
        \State Obtain the next state $\vec{\bm{y}}_{t+1}=\mathrm{Robot}(\vec{\bm{y}}_t,\vec{\bm{u}})$
    \EndFor
  \end{algorithmic}
\end{algorithm}

==> 3/Tables/LM_table.tex <==
% \begin{landscape}
\null\vspace{-2.0cm}$^$

\renewcommand{\arraystretch}{1.1}% Tighter
\begin{table}[H]
    \centering
    \small 
    \setlength\tabcolsep{6pt} % default value: 6pt
        \begin{tabular*}{15.65cm}{ l c c c c c c c }
            \toprule
            
            & & \multicolumn{2}{c}{Morphology} & & Controller & 
          \\\cmidrule(lr){3-4}\cmidrule(lr){5-7} \multicolumn{2}{l}{Author(s)} & Framework & Evolution &  Design & Optimizer & Life. L.& Year
            \\\midrule
            Sims & [\citenum{sims1994evolving}]&
            Other & GA & ANN & GP & - & 1994
            \\
            Lee \textit{et al.} & [\citenum{lee1996hybrid}] & PO & GA & ANN & GP & - & 1996 
            \\
            Lund \textit{et al.} & [\citenum{lund1998evolutionary}] & LEGO & GA & ANN & GA & - & 2000
            \\
            Lee & [\citenum{lee2000evolving}] & PO. & GP & ANN & GP & - & 2000
            \\
            Pollack \& Lipson & [\citenum{pollack2000golem}] & GOLEM & EA & ANN & GP & - & 2000
            \\
            Lipson \& Pollack  & [\citenum{lipson2000automatic}] & GOLEM & EA & ANN & GP & - & 2000
            \\
            Hornby \& Pollack  & [\citenum{hornby2001body}] & GenoBots & GP & CPG & GP & - & 2001
            \\
            Chirikjian \textit{et al.} & [\citenum{chirikjian2002self}] & LEGO & GA  & \textit{n/a} & fixed & - & 2002
            \\
            Lee & [\citenum{lee2003evolving}] & PO & GA & ANN & GP & - & 2003
            \\
            Pollack \textit{et al.} & [\citenum{pollack2003computer}]  & \makecell{ GOLEM/ \\ GenoBots} & \makecell{ EA/ \\ GP} & ANN &  GP & - & 2003
            \\
            Lund & [\citenum{lund2003co}]
            & LEGO & EA & ANN & - & - & 2003
            \\
            Macinnes \& Di Paolo & [\citenum{macinnes2004crawling}] & LEGO & EA & RNN & GP & - & 2004
            \\
            Paul \textit{et al.} &  [\citenum{paul2005evolutionary}] & Tensegrity & EA & - & - & - & 2005
            \\
            Paul \textit{et al.} &  [\citenum{paul2006design}] & Tensegrity & GA & Sinus & GA & - & 2006
            \\
            Lipson \& Pollack & [\citenum{lipson2006evolving}] & GenoBots & GP & ANN & GP & - & 2006
            \\
            M{\"o}ckel \textit{et al.} & [\citenum{mockel2006yamor}] & YaMoR$^*$ & GA & Splines & GP & - & 2006
            \\
            Gonzales-Gomez \& Boemo & [\citenum{gonzalez2006motion}] & Y1$^*$ & - & Sinus & Grid search & Yes & 2006
            \\
            Zykov \textit{et al.} & [\citenum{zykov2007evolved}] & MoleCubes$^*$ & GA & AT & GA & - & 2007
            \\
            Sproewitz \textit{et al.} & [\citenum{sproewitz2008learning}] & YaMoR$^*$ & - & ANN & Powell's & Yes & 2008
            \\
            Zykov \textit{et al.} & [\citenum{zykov2008molecubes}] & MoleCubes$^*$ & GA & AT & GA & - & 2008
            \\
            Lobo \& Vico & [\citenum{lobo2010evolutionary}] & Tensegrity & EA & - & - & - & 2010
            \\
            Zhong \textit{et al.} & [\citenum{zhong2010modular}] & MoleCubes$^*$ & GA & AT & GA & - & 2010
            \\
            Larpin \textit{et al.} & [\citenum{larpin2011co}] & PO & EA & CPG & GP & -  & 2011
            \\
            Ranganath \textit{et al.} & [\citenum{ranganath2011distributed}] & Y1$^*$ & GA & ANN & GP & -  & 2011
            \\
            Fa{\'\i}{\~n}a \textit{et al.} & [\citenum{faina2011first}] & EDHMoR & EA & Sinus & SO & - & 2011
            \\
            Auerbach \& Bongard & [\citenum{auerbach2012relationship}] & PO & H-Neat & CPPN & H-Neat & - & 2012
            \\
            Davey \textit{et al.} & [\citenum{davey2012emulating}] & SMORES$^*$ & - & \textit{n/a} & GP  & - & 2012 
            \\
            Iscen \textit{et al.} & [\citenum{iscen2013controlling}] & Tensegrity & EA & Sinus & GA & - & 2013
            \\
            D'Angelo \textit{et al.} & [\citenum{d2013online}] & YaMoR$^*$ & EA & Spline & RL-PoWER & Yes & 2013
            \\
            Fa{\'\i}{\~n}a \textit{et al.} & [\citenum{faina2013edhmor}] & EDHMoR & EA & Sinus & SO & - & 2013
            \\
            Khazonov \textit{et al.} &  [\citenum{khazanov2014evolution}] & Tensegrity & - & Sinus & GA & Yes & 2014
            \\
            Bruce \textit{et al.} &  [\citenum{bruce2014design}] & Tensegrity & EA & Sinus & SO & - & 2014
            \\
            Fa{\'\i}{\~n}a \textit{et al.} & [\citenum{faina2014towards}] & EDHMoR & EA & Sinus & SO & - & 2014
            \\
            Auerbach \textit{et al.} & [\citenum{auerbach2014robogen}] & RoboGen & GA & RNN & H-Neat & - & 2014
            \\
            Cheney \textit{et al.} & [\citenum{cheney2014unshackling}] & Other & H-Neat & CPPN & H-Neat  & - & 2014 
            \\
            Samuelsen \& Glette & [\citenum{samuelsen2015real}] & PO & GA & CPG & GP & -  & 2015
            \\
            Poikselk{\"a} \textit{et al.} & [\citenum{poikselka2015evolutionary}] & LEGO & EA & ANN & GP & -  & 2015
            \\
            Fa{\'\i}{\~n}a \textit{et al.} & [\citenum{faina2015evolution}] & EDHMoR  & EA & Sinus & SO & - & 2015
            \\
            Brodbeck \textit{et al.} & [\citenum{brodbeck2015morphological}] & Other & GA & Sinus & GP & - & 2015
            \\
            Jelisavcic \textit{et al.} & [\citenum{jelisavcic2016improving}] & RoboGen & - & Splines & RL-PoWER & Yes & 2016
            \\
            Moreno \textit{et al.} & [\citenum{moreno2017emerge}] & EMeRGe$^*$ & GP & Sinus & SO & - & 2017
            \\
            Veenstra \textit{et al.} & [\citenum{veenstra2017evolution}] & EMeRGe$^*$ & GP & Sinus & SO & - & 2017
            \\
            Jelisavcic \textit{et al.} & [\citenum{jelisavcic2017real}] & RoboGen & GA & Splines & RL-PoWER & Yes & 2017
            \\
            Vujovic \textit{et al.} & [\citenum{vujovic2017evolutionary}] & Other & GP & Sinus & GP & - & 2017
            \\
            Cellucci \textit{et al.} & [\citenum{cellucci20171d}] & Other & H-Neat & CPPN & H-Neat & - & 2017
            \\
            Miras \textit{et al.} & [\citenum{miras2018effects}] & RoboGen & GP & ANN & GP & - & 2018
            \\
            Miras \textit{et al.} & [\citenum{miras2019effects}] & RoboGen & GP & CPG & GP & - & 2019
            \\
            Tosun \textit{et al.} & [\citenum{tosun2018computer}] & SMORES$^*$ & GP & AT & GA & - & 2018
            \\
            Hupkes \textit{et al.} & [\citenum{hupkes2018revolve}] & RoboGen & GA & ANN & GP & - & 2018
            \\
            Jelisavcic \textit{et al.} & [\citenum{jelisavcic2019lamarckian}] & RoboGen & EA & CPG & CPPN & Yes & 2019
            \\
            Hale \textit{et al.} & [\citenum{hale2019robot}] & Other & EA & \textit{n/a} & fixed & - & 2019
            \\
            Lan \textit{et al.} & [\citenum{lan2020learning}] & RoboGen & EA & CPG & \makecell{ H-Neat/ \\ BO}  & Yes & 2020 
            \\
            Kriegman \textit{et al.} & [\citenum{Kriegman1853}] & Other & H-Neat & CPPN & SO & - & 2020 
            \\\bottomrule
         \end{tabular*}
    \caption{Overview of all the included papers, $^*$ denotes a homogeneous framework}
    \label{tab:CD+LM}
\end{table}

% \end{landscape}


==> 3/Tables/LM_table_old.tex <==
% \begin{landscape}
\null\vspace{-2.0cm}

\renewcommand{\arraystretch}{1.1}% Tighter
\begin{table}[H]
    \centering
    \small 
    \setlength\tabcolsep{6pt} % default value: 6pt
        \begin{tabular*}{15.65cm}{ l l c c c c c c }
            \toprule
            
            & & \multicolumn{2}{c}{Morphology} & & Controller & 
          \\\cmidrule(lr){3-4}\cmidrule(lr){5-7} \multicolumn{2}{l}{Author(s)} & Framework & Evolution &  Design & Optimizer & Online L.& Year
            \\\midrule
            Sims & \citenum{sims1994evolving}&
            Other & GA & ANN & GP & - & 1994
            \\
            Lee \textit{et al.} & \citenum{lee1996hybrid} & PO & GA & ANN & GP & - & 1996 
            \\
            Lund \textit{et al.} & \citenum{lund1998evolutionary} & LEGO & GA & ANN & GA & - & 2000
            \\
            Lee & \citenum{lee2000evolving} & PO. & GP & ANN & GP & - & 2000
            \\
            Pollack \& Lipson & \citenum{pollack2000golem} & GOLEM & EA & ANN & GP & - & 2000
            \\
            Lipson \& Pollack  & \citenum{lipson2000automatic} & GOLEM & EA & ANN & GP & - & 2000
            \\
            Hornby \& Pollack  & \citenum{hornby2001body} & GenoBots & GP & CPG & GP & - & 2001
            \\
            Chirikjian \textit{et al.} & \citenum{chirikjian2002self} & LEGO & GA  & \textit{n/a} & fixed & - & 2002
            \\
            Lee & \citenum{lee2003evolving} & PO & GA & ANN & GP & - & 2003
            \\
            Pollack \textit{et al.} & \citenum{pollack2003computer}  & \makecell{ GOLEM/ \\ GenoBots} & \makecell{ EA/ \\ GP} & ANN &  GP & - & 2003
            \\
            Lund & \citenum{lund2003co}
            & LEGO & EA & ANN & - & - & 2003
            \\
            Macinnes \& Di Paolo & \citenum{macinnes2004crawling} & LEGO & EA & RNN & GP & - & 2004
            \\
            Paul \textit{et al.} &  \citenum{paul2005evolutionary} & Tensegrity & EA & - & - & - & 2005
            \\
            Paul \textit{et al.} &  \citenum{paul2006design} & Tensegrity & GA & Sinus & GA & - & 2006
            \\
            Lipson \& Pollack & \citenum{lipson2006evolving} & GenoBots & GP & ANN & GP & - & 2006
            \\
            M{\"o}ckel \textit{et al.} & \citenum{mockel2006yamor} & YaMoR$^1$ & GA & Splines & GP & - & 2006
            \\
            Gonzales-Gomez \& Boemo & \citenum{gonzalez2006motion} & Y1$^1$ & - & Sinus & Grid search & Yes & 2006
            \\
            Zykov \textit{et al.} & \citenum{zykov2007evolved} & MoleCubes$^1$ & GA & AT & GA & - & 2007
            \\
            Sproewitz \textit{et al.} & \citenum{sproewitz2008learning} & YaMoR$^1$ & - & ANN & Powell's & Yes & 2008
            \\
            Zykov \textit{et al.} & \citenum{zykov2008molecubes} & MoleCubes$^1$ & GA & AT & GA & - & 2008
            \\
            Lobo \& Vico & \citenum{lobo2010evolutionary} & Tensegrity & EA & - & - & - & 2010
            \\
            Zhong \textit{et al.} & \citenum{zhong2010modular} & MoleCubes$^1$ & GA & AT & GA & - & 2010
            \\
            Larpin \textit{et al.} & \citenum{larpin2011co} & PO & EA & CPG & GP & -  & 2011
            \\
            Ranganath \textit{et al.} & \citenum{ranganath2011distributed} & Y1$^1$ & GA & ANN & GP & -  & 2011
            \\
            Fa{\'\i}{\~n}a \textit{et al.} & \citenum{faina2011first} & EDHMoR & EA & Sinus & SO & - & 2011
            \\
            Auerbach \& Bongard & \citenum{auerbach2012relationship} & PO. & H-Neat & CPPN & H-Neat & - & 2012
            \\
            Davey \textit{et al.} & \citenum{davey2012emulating} & SMORES$^1$ & - & fixed & -  & - & 2012 
            \\
            Iscen \textit{et al.} & \citenum{iscen2013controlling} & Tensegrity & EA & Sinus & GA & - & 2013
            \\
            D'Angelo \textit{et al.} & \citenum{d2013online} & YaMoR$^1$ & EA & Spline & RL-PoWER & Yes & 2013
            \\
            Fa{\'\i}{\~n}a \textit{et al.} & \citenum{faina2013edhmor} & EDHMoR & EA & Sinus & SO & - & 2013
            \\
            Khazonov \textit{et al.} &  \citenum{khazanov2014evolution} & Tensegrity & - & Sinus & GA & Yes & 2014
            \\
            Bruce \textit{et al.} &  \citenum{bruce2014design} & Tensegrity & EA & Sinus & SO & - & 2014
            \\
            Fa{\'\i}{\~n}a \textit{et al.} & \citenum{faina2014towards} & EDHMoR & EA & Sinus & SO & - & 2014
            \\
            Auerbach \textit{et al.} & \citenum{auerbach2014robogen} & RoboGen & GA & RNN & H-Neat & - & 2014
            \\
            Cheney \textit{et al.} & \citenum{cheney2014unshackling} & Other & H-Neat & CPPN & H-Neat  & - & 2014 
            \\
            Samuelsen \& Glette & \citenum{samuelsen2015real} & P. & GA & CPG & GP & -  & 2015
            \\
            Poikselk{\"a} \textit{et al.} & \citenum{poikselka2015evolutionary} & LEGO & EA & ANN & GP & -  & 2015
            \\
            Fa{\'\i}{\~n}a \textit{et al.} & \citenum{faina2015evolution} & EDHMoR  & EA & Sinus & SO & - & 2015
            \\
            Brodbeck \textit{et al.} & \citenum{brodbeck2015morphological} & Other & GA & Sinus & GP & - & 2015
            \\
            Jelisavcic \textit{et al.} & \citenum{jelisavcic2016improving} & RoboGen & - & Splines & RL-PoWER & Yes & 2016
            \\
            Moreno \textit{et al.} & \citenum{moreno2017emerge} & EMeRGe$^1$ & GP & Sinus & SO & - & 2017
            \\
            Veenstra \textit{et al.} & \citenum{veenstra2017evolution} & EMeRGe$^1$ & GP & Sinus & SO & - & 2017
            \\
            Jelisavcic \textit{et al.} & \citenum{jelisavcic2017real} & RoboGen & GA & Splines & RL-PoWER & Yes & 2017
            \\
            Vujovic \textit{et al.} & \citenum{vujovic2017evolutionary} & Other & GP & Sinus & GP & - & 2017
            \\
            Cellucci \textit{et al.} & \citenum{cellucci20171d} & Other & H-Neat & CPPN & H-Neat & - & 2017
            \\
            Miras \textit{et al.} & \citenum{miras2018effects} & RoboGen$^1$ & GP & ANN & GP & - & 2018
            \\
            Miras \textit{et al.} & \citenum{miras2019effects} & RoboGen$^1$ & GP & CPG & GP & - & 2019
            \\
            Tosun \textit{et al.} & \citenum{tosun2018computer} & SMORES$^1$ & GP & AT & GA & - & 2018
            \\
            Hupkes \textit{et al.} & \citenum{hupkes2018revolve} & RoboGen & GA & ANN & GP & - & 2018
            \\
            Jelisavcic \textit{et al.} & \citenum{jelisavcic2019lamarckian} & RoboGen & EA & CPG & CPPN & Yes & 2019
            \\
            Hale \textit{et al.} & \citenum{hale2019robot} & Other & EA & \textit{n/a} & fixed & - & 2019
            \\
            Lan \textit{et al.} & \citenum{lan2020learning} & RoboGen & EA & CPG & \makecell{ H-Neat/ \\ BO}  & Yes & 2020 
            \\
            Kriegman \textit{et al.} & \citenum{Kriegman1853} & Other & H-Neat & CPPN & SO & - & 2020 
            \\\bottomrule
         \end{tabular*}
    \caption{Overview of all the included papers}
    \label{tab:CD+LM}
\end{table}

% \end{landscape}


==> 3/Tables/MD_table.tex <==
% \begin{landscape}

\begin{table}
\centering
 \begin{tabular*}{\textwidth}{ m{4.5em} 
 m{3.1cm}
 >{\centering}m{.7cm}   >{\centering}m{1.95cm}  >{\centering}m{1.95cm} m{5.5cm} }
    \toprule
    Name & Modules & $N_{mod}$  & Production & Architecture &  Papers 
    \\\midrule
       PO & \textit{spheres, rectangles, bars, wheels} & 4 & - & \textit{-} & [\citenum{lee1996hybrid,lee2000evolving,lee2003evolving,larpin2011co,auerbach2012relationship}]$^{1}$[\citenum{samuelsen2015real}]$^{1,2}$
    \\
       GOLEM/ Genobots & \textit{bars, joints} & 2 & 3D printing & \textit{tree} & [\citenum{pollack2000golem,lipson2000automatic,pollack2003computer}]$^{1,2}$/\newline [\citenum{hornby2001body}]$^1$[\citenum{pollack2003computer,lipson2006evolving}]$^{1,2}$
    \\
       LEGO & \textit{wheels, motors, bricks, sensors} & 4 & store bought & \textit{tree} &[\citenum{chirikjian2002self}]$^1$[\citenum{lund1998evolutionary,lund2003co,macinnes2004crawling,poikselka2015evolutionary}]$^{1,2}$
    \\
       Tensegrity & \textit{bars, tensile cables} & 2 & manufacture &\textit{tree} & [\citenum{paul2005evolutionary,lobo2010evolutionary,iscen2013controlling,bruce2014design}]$^1$[\citenum{paul2006design}]$^{1,2}$[\citenum{khazanov2014evolution}]$^2$
    \\
       Homogen. & \textit{robot} & 1 & manufacture & \textit{mobile} &[\citenum{d2013online}]$^1$[\citenum{mockel2006yamor,sproewitz2008learning,davey2012emulating,tosun2018computer,moreno2017emerge,veenstra2017evolution,gonzalez2006motion,ranganath2011distributed,zykov2007evolved,zykov2008molecubes,zhong2010modular}]$^{1,2}$
    \\
       Heterogen. & \textit{hinge, rotational, slider, telescope} & 4 & manufacture & \textit{lattice} &[\citenum{faina2011first,faina2013edhmor,faina2014towards,faina2015evolution}]$^{1,2}$
    \\
       RoboGen & \textit{core, brick, fixed joint, passive/active hinge, sensors} & 6 & 3D printing & \textit{tree/lattice} &[\citenum{jelisavcic2016improving,hupkes2018revolve,miras2018effects,miras2019effects,jelisavcic2019lamarckian}]$^1$[\citenum{auerbach2014robogen,jelisavcic2017real,lan2020learning}]$^{1,2}$
    \\
       Other & - & - & - & - & [\citenum{sims1994evolving}]$^1$[\citenum{brodbeck2015morphological,vujovic2017evolutionary}]$^2$[\citenum{cheney2014unshackling,cellucci20171d,hale2019robot,Kriegman1853}]$^{1,2}$
    \\
    \bottomrule
 \end{tabular*}
 \caption{Overview of the different types of morphological designs in the Evolutionary Robotics literature that use a modular framework, and their corresponding properties. PO refers to Parameter Optimization, and Homogen. refers to Homogeneous robots. Additionally, $^1$ denotes the robot being tested in simulation, while $^2$ denotes real robot testing the paper.}
 \label{tab:MD}
\end{table}
% \end{landscape}


==> 3/Tables/MD_table_old.tex <==
% \begin{landscape}

\begin{table}
\centering
 \begin{tabular*}{\textwidth}{ m{4.5em} 
 m{3.1cm}
 >{\centering}m{.7cm}   >{\centering}m{1.95cm}  >{\centering}m{1.95cm} m{5.5cm} }
    \toprule
    Name & Modules & $N_{mod}$  & Production & Architecture &  Papers 
    \\\midrule
       PO & \textit{spheres, rectangles, bars, wheels} & 4 & - & \textit{-} & \citenum{lee1996hybrid,lee2000evolving,lee2003evolving,larpin2011co,auerbach2012relationship}$^{1}$\citenum{samuelsen2015real}$^{1,2}$
    \\
       GOLEM/ Genobots & \textit{bars, joints} & 2 & 3D Printing & \textit{Tree} & \citenum{pollack2000golem,lipson2000automatic,pollack2003computer}$^{1,2}$/\newline \citenum{hornby2001body}$^1$\citenum{pollack2003computer,lipson2006evolving}$^{1,2}$
    \\
       LEGO & \textit{wheels, motors, bricks, sensors} & 4 & store bought & \textit{Tree} &\citenum{chirikjian2002self}$^1$\citenum{lund1998evolutionary,lund2003co,macinnes2004crawling,poikselka2015evolutionary}$^{1,2}$
    \\
       Tensegrity & \textit{bars, tensile cables} & 2 & manufacture &\textit{Tree} & \citenum{paul2005evolutionary,lobo2010evolutionary,iscen2013controlling,bruce2014design}$^1$\citenum{paul2006design}$^{1,2}$\citenum{khazanov2014evolution}$^2$
    \\
       Homogen. & \textit{robot} & 1 & manufacture & \textit{mobile} &\citenum{d2013online}$^1$\citenum{mockel2006yamor,sproewitz2008learning,davey2012emulating,tosun2018computer,moreno2017emerge,veenstra2017evolution,gonzalez2006motion,ranganath2011distributed,zykov2007evolved,zykov2008molecubes,zhong2010modular}$^{1,2}$
    \\
       Heterogen. & \textit{hinge, rotational, slider, telescope} & 4 & manufacture & \textit{lattice} &\citenum{faina2011first,faina2013edhmor,faina2014towards,faina2015evolution}$^{1,2}$
    \\
       RoboGen & \textit{core, brick, fixed joint, passive/active hinge, sensors} & 6 & 3D Printing & \textit{tree/lattice} &\citenum{jelisavcic2016improving,hupkes2018revolve,miras2018effects,miras2019effects,jelisavcic2019lamarckian}$^1$\citenum{auerbach2014robogen,jelisavcic2017real,lan2020learning}$^{1,2}$
    \\
       Other & - & - & - & - & \citenum{sims1994evolving}$^1$\citenum{brodbeck2015morphological,vujovic2017evolutionary}$^2$\citenum{cheney2014unshackling,cellucci20171d,hale2019robot,Kriegman1853}$^{1,2}$
    \\
    \bottomrule
 \end{tabular*}
 \caption{Overview of the different types of morphological designs in the Evolutionary Robotics literature that use a modular framework, and their corresponding properties. PO refers to Parameter Optimization, and Homogen. refers to Homogeneous robots. Additionally, $^1$ denotes the robot being tested in simulation, while $^2$ denotes real robot testing the paper.}
 \label{tab:MD}
\end{table}
% \end{landscape}


==> 3/Tables/Method_table.tex <==
\small
%         \begin{tabular}{r l| l l l | c}
%              \multicolumn{2}{c|}{Query} & AND $\rightarrow$ &   & & $N$
%              \\ \hline
%               \multirow{2}[0]{*}{
%                   \rotatebox{90}{$\leftarrow$ OR}
%               }
              
%             &   1. & "modular robot*" & design & evolution* & 92
%              \\
%             &   2. & "modular robot*" & framework & evolution* & 23
%              \\
%             &   3. & modular robot* & locomotion & evolution* & 45
%              \\
%             &   4. & modular robot* & gait & evolution* & 15
%              \\
%             &   5. & "evolution* robot*" & locomotion & modul*& 17
%              \\
%             &   6. & "evolution* robot*" & gait & modul* & 5

%          \end{tabular}
%         \captionof{table}{List of all the search queries that were used for this literature survey. A star (*) denotes a wildcard, \textit{e.g.} robot* $\rightarrow$ \{robot, robots, robotics, \textit{etc.}\}.}
% \label{tab:Methods}


        \begin{tabular}{r l| l l l }
             \multicolumn{2}{c|}{} & AND $\rightarrow$ &   & 
             \\ \hline
              \multirow{2}[0]{*}{
                  \rotatebox{90}{$\leftarrow$ OR}
              }
              
            &   1. & modular robot* & design & evolution* 
            \\
            &   2. & modular robot* & framework & evolution* 
            \\
            &   3. & modular robot* & locomotion & evolution* 
            \\
            &   4. & modular robot* & gait & evolution* 
            \\
            &   5. & evolution* robot* & locomotion & modul*
            \\
            &   6. & evolution* robot* & gait & modul* 

         \end{tabular}
        \captionof{table}{List of all the search queries that were used for this literature survey. Multi-word search terms were grouped using "quotation marks"  (left out for readability purposes). A star (*) denotes a wildcard, \textit{e.g.} robot* $\rightarrow$ \{robot, robots, robotics, \textit{etc.}\}.}
\label{tab:Methods}


==> 4/Math/T_two.tex <==
\begin{bmatrix}
\frac{- \lambda_{1}^{2} + w_{2}^{2}}{c w_{2}} & \frac{- \lambda_{1}^{2} + w_{2}^{2}}{c w_{2}} & \frac{- \lambda_{2}^{2} + w_{2}^{2}}{c w_{2}} & \frac{- \lambda_{2}^{2} + w_{2}^{2}}{c w_{2}}\\
\frac{w_{1} \left(\lambda_{1}^{2} - w_{2}^{2}\right)}{c \lambda_{1} w_{2}}i & -\frac{w_{1} \left(\lambda_{1}^{2} - w_{2}^{2}\right)}{c \lambda_{1} w_{2}}i & \frac{w_{1} \left(\lambda_{2}^{2} - w_{2}^{2}\right)}{c \lambda_{2} w_{2}}i & -\frac{w_{1} \left(\lambda_{2}^{2} - w_{2}^{2}\right)}{c \lambda_{2} w_{2}}i\\
\frac{\lambda_{1}}{w_{2}}i & - \frac{\lambda_{1}}{w_{2}}i & \frac{\lambda_{2}}{w_{2}}i & - \frac{\lambda_{2}}{w_{2}}i\\
1 & 1 & 1 & 1
\end{bmatrix}

==> 4/Math/T_two_inv.tex <==
\begin{bmatrix}- \frac{c w_{2}}{2\left( \lambda_{1}^{2} - \lambda_{2}^{2}\right)} & - \frac{c \lambda_{1} \lambda_{2}^{2}}{2 w_{1} w_{2} \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}i & \frac{\lambda_{1} \left(\lambda_{2}^{2} - w_{2}^{2}\right)}{2 w_{2} \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}i & -\frac{\lambda_{2}^{2} - w_{2}^{2}}{2 \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}\\
- \frac{c w_{2}}{2\left( \lambda_{1}^{2} -  \lambda_{2}^{2}\right)} & \frac{c \lambda_{1} \lambda_{2}^{2}}{2 w_{1} w_{2} \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}i & - \frac{\lambda_{1} \left(\lambda_{2}^{2} - w_{2}^{2}\right)}{2 w_{2} \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}i & -\frac{\lambda_{2}^{2} - w_{2}^{2}}{2 \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}\\
\frac{c w_{2}}{2 \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)} & \frac{c \lambda_{1}^{2} \lambda_{2}}{2 w_{1} w_{2} \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}i & -\frac{\lambda_{2} \left( \lambda_{1}^{2} - w_{2}^{2}\right)}{2 w_{2} \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}i & \frac{\lambda_{1}^{2} - w_{2}^{2}}{2 \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}\\
\frac{c w_{2}}{2 \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)} & - \frac{c \lambda_{1}^{2} \lambda_{2}}{2 w_{1} w_{2} \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}i & \frac{\lambda_{2} \left(\lambda_{1}^{2} - w_{2}^{2}\right)}{2 w_{2} \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}i & \frac{\lambda_{1}^{2} - w_{2}^{2}}{2 \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}\end{bmatrix}

==> 4/figures/CPG.tex <==
\centering
\resizebox{0.6\linewidth}{!}{\footnotesize
    \begin {tikzpicture}
	    [-latex,
		auto,
		node distance =1.375cm and 1.375cm,
		on grid,
		semithick,
		state/.style = {circle,draw,inner sep=0pt,minimum width = 0.7 cm}]
	\node[state] (X) {$x_i$};
	\node[state] (Y) [left = of X] {$y_i$};
	\node[state] (Output) [right = of X] {$o_i$};
	\path (X) edge [bend left = 30] node [] {$w_{x_iy_i}$} (Y);
	\path (Y) edge [bend left = 30] node [] {$w_{y_ix_i}$} (X);
	\path (X) edge  node [] {$w_{x_io_i}$} (Output);
	\node (ghost) [below of = X]       {};
	\end {tikzpicture}
}

==> 4/figures/CPG_net.tex <==
\centering
\resizebox{0.66\linewidth}{!}{%
\footnotesize
\begin {tikzpicture}
	    [
		auto,
		node distance =0.3375cm and 0.3375cm,
		on grid,
		thick,
		state/.style = {circle,draw,inner sep=0pt, minimum width = 0.35 cm},
		box/.style={rectangle,draw,minimum width = 0.3 cm, minimum size=0.3 cm},
		core/.style={rectangle,draw=red!60,fill=red!5,very thick,minimum width = 0.5 cm, minimum size=0.5 cm},
		state_l/.style = {circle,draw,inner sep=0pt, minimum width = 0.2 cm},
		box_l/.style={rectangle,draw,inner sep=0pt,minimum size=0.15 cm},
		core_l/.style={rectangle,draw=red!60,fill=red!5,very thick,inner sep=0pt, minimum size=0.15 cm}]

	\node[box] (B_l1) {};
	\node[state] (O4) [right = of B_l1] {$4$};
	\node[box] (B_l2) [right = of O4] {};
	\node[state] (O3) [right = of B_l2] {$3$};
	\node[core] (core) [right = 0.49cm of O3] {};
	\node[state] (O2) [above=0.48cm of core] {$2$};
	\node[box] (B_t2) [above=of O2] {};
	\node[state] (O1) [above=of B_t2] {$1$};
	\node[box] (B_t1) [above=of O1] {};
	\node[state] (O6) [right= 0.49cm of core] {$6$};
	\node[box] (B_r2) [right= of O6] {};
	\node[state] (O5) [right=of B_r2] {$5$};
	\node[box] (B_r1) [right=of O5] {};
	\node[state] (O8) [below=0.48cm of core] {$8$};
	\node[box] (B_b2) [below=of O8] {};
	\node[state] (O7) [below=of B_b2] {$7$};
	\node[box] (B_b1) [below=of O7] {};
	
% 	\node[rectangle,draw,minimum width=0.1cm, minimum size=0.1cm, minimum height=0.1cm] (legend_box) [above=1.4cm of B_l1] {};	
% 	\node[circle,draw,inner sep=0pt, minimum width = 0.3cm] (legend_state) [below= 0.4cm of legend_box] {};	
% 	\node[rectangle,draw=red!60,fill=red!5,very thick,minimum width = 0.1 cm, minimum size=0.1 cm] (legend_core) [below=0.4cm of legend_state] {};	
	\node[box_l] (legend_box) [above=1.4cm of B_l1] {};	
	\node[state_l] (legend_state) [below= 0.22cm of legend_box] {\tiny{$i$}};	
	\node[core_l] (legend_core) [below=0.22cm of legend_state] {};
	\node[rectangle,inner sep=0pt, minimum size=0.15 cm] (legend_arrow) [below=0.22cm of legend_core] {};
	\draw[-{Straight Barb[left, scale=0.5]}, blue] (legend_arrow.-180) to node [] {} (legend_arrow.0);
	\node[text width=1cm, align = left,right=0.7cm of legend_box]{\tiny Brick};
	\node[text width=1cm, align = left,right=0.7cm of legend_state]{\tiny Servo};
	\node[text width=1cm, align = left,right=0.7cm of legend_core]{\tiny Core};
	\node[text width=1cm, align = left,right=0.7cm of legend_arrow]{\parbox[b][0.4cm][b]{1cm}{\linespread{0.15}\tiny Inter-\newline connection}};
	
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0, draw=blue] (O4.10) to node [] {} (O3.170);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O3.-170) to node [] {} (O4.-10);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O6.10) to node [] {} (O5.170);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O5.-170) to node [] {} (O6.-10);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O2.100) to node [] {} (O1.-100);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O1.-80) to node [] {} (O2.80);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O7.100) to node [] {} (O8.-100);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O8.-80) to node [] {} (O7.80);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O3.50) to node [] {} (O2.-140);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O2.-120) to node [] {} (O3.30);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O3.10) to node [] {} (O6.170);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O6.-170) to node [] {} (O3.-10);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O3.10) to node [] {} (O6.170);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O6.-170) to node [] {} (O3.-10);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O6.150) to node [] {} (O2.-60);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O2.-40) to node [] {} (O6.130);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O2.-80) to node [] {} (O8.80);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O8.100) to node [] {} (O2.-100);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O6.-130) to node [] {} (O8.40);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O8.60) to node [] {} (O6.-150);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O6.-130) to node [] {} (O8.40);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O8.60) to node [] {} (O6.-150);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O3.-30) to node [] {} (O8.120);
	\path[-{Straight Barb[left, scale=0.5]}, bend left = 0,draw=blue] (O8.140) to node [] {} (O3.-50);
	\end {tikzpicture}
}

==> 4/figures/Solve_multi.tex <==


The eigenvalues for our coupled oscillators are defined as.

\begin{equation}
\begin{split}
    \mathrm{det}(\bm{A}-I\lambda)&=0\\
    \mathrm{det}\left(\begin{bmatrix}
-\lambda & w_{1}  & c & 0\\
-w_{1}  & -\lambda & 0 & 0\\
-c & 0 & -\lambda & w_{2}  \\
0  & 0& -w_{2} & -\lambda \\
\end{bmatrix}\right) & = 0\\
\lambda^4+\lambda^2c^2+\lambda^2w_1^2+\lambda^2w_2^2+ w_1^2w_2^2&=0\\
\lambda^4+\lambda^2(c^2+w_1^2+w_2^2) + w_1^2w_2^2&= 0 \\
p^2 + p(c^2+w_1^2+w_2^2) + w_1^2w_2^2&= 0 \quad\text{for $p=\lambda^2$}
\end{split}\label{eq:poly2}
\end{equation}

Using the quadratic-formula to solve for $p$:

\begin{alignat}{2}
p&= \frac{-b\pm \sqrt{b^2-4ac}}{2a} \nonumber \\
&= -\frac{1}{2}\left[c^2+w_1^2+w_2^2\pm \sqrt{(c^2+w_1^2+w_2^2)^2-4w_1^2w_2^2}\right] \nonumber \\
&= -\frac{1}{2}\left[c^2+w_1^2+w_2^2\pm \sqrt{c^4+2c^2(w_1^2+w_2^2)+w_1^4+w_2^4+2w_1^2w_2^2-4w_1^2w_2^2}\right] \nonumber \\
&= -\frac{1}{2}\left[c^2+w_1^2+w_2^2\pm \sqrt{c^4+2c^2(w_1^2+w_2^2)+w_1^4+w_2^4-2w_1^2w_2^2}\right] \nonumber \\
&= -\frac{1}{2}\left[c^2+w_1^2+w_2^2\pm \sqrt{c^4+2c^2(w_1^2+w_2^2)+(w_1^2-w_2^2)^2}\right] \nonumber \\
&= -\frac{1}{2}\left[\sqrt{(c^2+w_1^2+w_2^2)^2}\pm \sqrt{c^4+2c^2(w_1^2+w_2^2)+(w_1^2-w_2^2)^2}\right]\nonumber \\
&=-\frac{1}{2}\Big[\sqrt{c^4+2c^2(w_1^2+w_2^2)+w_1^4+w_2^4+2w_1^2w_2^2} \nonumber\\&  \hspace{4em} \pm \sqrt{c^4+2c^2(w_1^2+w_2^2)+(w_1^2-w_2^2)^2}\Big] \nonumber\\
&=-\frac{1}{2}\left[\sqrt{c^4+2c^2(w_1^2+w_2^2)+(w_1^2+w_2^2)^2} \pm \sqrt{c^4+2c^2(w_1^2+w_2^2)+(w_1^2-w_2^2)^2}\right] \label{eq:abc_pm}\\
&=-\frac{1}{2}\left[\sqrt{C+(W^+)^2} \pm \sqrt{C+(W^-)^2}\right] \label{eq:abc_p}\\%\hspace{4em}\text{where }\hspace{1em}\makecell[l]{ C=c^4+2c^2(w_1^2+w_2^2)\\ W^\pm=w_1^2\pm w_2^2 \hfill}
&\hspace{4em}\text{where }\hspace{1em} C=c^4+2c^2(w_1^2+w_2^2) \textrm{\hspace{1em} and, \hspace{1em}} W^\pm=w_1^2\pm w_2^2 \nonumber
\end{alignat}

Let's take a moment to assess what we have for a bit. We split our quadratic-formula into two distinct parts: $C$ (which is dependent on the interconnection $c$) and $W$ (which is solely dependent on the weights). \autoref{eq:abc_p} shows that for $p=\lambda^2$. Now, we can already get some intuition on the eigenvalues. 

$W^\pm$ provides two instances of $W$ for which the following is true $W^-\leq W^+$ for all combinations of $w_1, w_2$. In the most general case, where both oscillator weights are non-zero ($w_1\neq0 \land w_2\neq0$), we see that $W^-$ is strictly smaller than $W^+$ ($W^-< W^+$) which means that $p$ will always be strictly negative due to the discriminant being smaller than the non-discriminant:
\begin{equation}
\begin{split}
    p_{1,2}&<0 \hspace{5em} \forall C, W^-< W^+ \\
    \lambda_{1,2}^2&< 0 \\
    \lambda_{1,2}&=\pm\sqrt{|p_{1,2}|}i \hspace{2em}\in\mathbb{C}\setminus\mathbb{R}
\end{split}\label{eq:p_w_n0}
\end{equation}

This result shows that whatever values for $C$ and $W^-< W^+$ we use, our SO2-oscillator pair in its canonical form contains a set of purely imaginary eigenvalue pairs $\lambda$. Thus, our controller behaviour can always be described as a set of pure cosines.

Additionally, for the special case where `either one, but not both' oscillator weights are equal to zero ($w_1\neq0 \land w_2=0 $ or $w_1=0\land w_2\neq0$) it follows that $(W^-)^2=(W^+)^2$. From which we can derive the following values of $p$: 
% \begin{equation}
\begin{alignat}{2}
    p& \multicolumn{2}{l}{$=-\frac{1}{2}\left[\sqrt{c^4+2c^2w_{1 or 2}^2+w_{1 or 2}^4} \pm \sqrt{c^4+2c^2w_{1 or 2}^2+w_{1 or 2}^4}\right]$} \nonumber \\
    &=-\frac{1}{2}\left[(c^2+w_{1 or 2}^2) \pm (c^2+w_{1 or 2}^2)\right] & \nonumber \\
    p_1&= -(c^2+w_{1 or 2}^2) &p_2= 0 \nonumber \\
    \lambda_1&= \pm\sqrt{|p_1|}i \hspace{2em}\in\mathbb{C}\setminus\mathbb{R} &\lambda_2= 0 %
\end{alignat}\label{eq:p_w_0}
% \end{equation}

This shows that the resulting dynamics reduce to a single SO2-oscillator dependent on the amplitude of the interconnection and remaining weight $\sqrt{c^2+w_{1 or 2}^2}$. In fact, the LTI-description of our interconnected oscillators can be rewritten (by row-reduction) to a single oscillator with zeros at the remaining LTI-matrix indices, independent of which weight is set to zero. It is important to note that this reaffirms our previous finding that any type of SO2-oscillator can be defined as a set of cosines in its canonical form, where this special case reduces the number of cosines to a single oscillator.

For $C$ we can look at two other special cases $c$ approaches zero ($c\rightarrow 0$) or where c approaches infinity ($c\rightarrow\infty$): 
\begin{alignat}{2}
    p&= -\frac{1}{2}\left[\sqrt{(W^+)^2} \pm \sqrt{(W^-)^2}\right] &\hspace{3em}& \text{for } c\to 0 \implies C\to 0 \nonumber\\
     &= -\frac{1}{2}\left[W^+ \pm W^-\right] \nonumber\\
     &= -\frac{1}{2}\left[w_1^2+ w_2^2 \pm (w_1^2- w_2^2)\right] \nonumber\\
    p_1&= -\frac{1}{2}\left[2w_1^2\right] &\multicolumn{2}{l}{\hspace{0.05em}$p_2= -\frac{1}{2}\left[2w_2^2\right]$} \nonumber\\
    \lambda_1&= \pm w_1i \phantom{\frac{1}{2}\left[2\right]} &\multicolumn{2}{l}{$\lambda_2= \pm w_2i \hspace{2em}\in\mathbb{C}\setminus\mathbb{R}$}
\end{alignat}

Just like \autoref{eq:p_w_n0}, we again obtain two purely imaginary numbers as our eigenvalues when $c$ approaches zero. But now our oscillator weights dominate the behaviour cosines as if they were two separate oscillators. This is not surprising as $c\rightarrow 0$ implies that we almost remove the interconnection between the two base oscillators from \autoref{fig:CPG_intercon_v} and end up with two independent instances of the singular CPG defined before (\autoref{eq:CPG_single}) for which we already analytically solved the equations of motion (in Section \ref{secA3}). Now for $c\rightarrow\infty$:

\begin{alignat}{2}
    p&= -\frac{1}{2}\left[\sqrt{c^4} \pm \sqrt{c^4}\right] \hspace{2em}&\hspace{1em}& c\to \infty \implies C \approx c^4 \ggg W^\pm \nonumber\\
     &= -\frac{1}{2}\left[c^2 \pm c^2\right] \nonumber\\
    \lambda_1&= \pm ci \hspace{2em}\in\mathbb{C}\setminus\mathbb{R} &\multicolumn{2}{l}{$\lambda_2= 0\label{eq:p_c2inf}$}
\end{alignat}

This result shows a dependency of the two coupled oscillator frequencies on the relative size of $c$ with respect to $w_1$, $w_2$. If the interconnection weight dominates the oscillator weights, then the interconnected $x$-neurons start to behave as a single CPG together. This result resembles a singular CPG with frequency $c$ between the two $x-$neurons, because of the negligible effects of the two surrounding $y-$neuron weights. The results also show what happens when both oscillator weight are zero ($w_1=0\land w_2=0$) and only connection $c$ is non-zero.

The eigenvalue analysis reveals that for any type of interconnected SO2-oscillator the resulting behaviour can be described by its canonical form as a set of pure cosines. The weights in this aspect influence the frequency content non-linearly, where special cases with weights equal zero will abruptly change the dynamical system as a whole (i.e. reducing the number of cosines, or creating single oscillators). 

Now, for the more general case where the influence of both $c$ and $w$ are not negligible. Here we know that the eigenvalues are purely imaginary pairs (from \autoref{eq:p_w_n0}). For the sake of clarity, we refer to these eigenvalues as $\pm\lambda_{1}i$ and $\pm\lambda_{2}i$ while deriving our eigenvectors. The $i$ notation is there to remind us of the imaginary component. To obtain the eigenvectors we need to solve $(\bm{A}-I\lambda)V=0$ for all eigenvalues:

\begin{equation}
\begin{aligned}
    % &&(\bm{A}-I\lambda)V&=0 \\ &\\
&\text{for $\lambda=-\lambda_1i$} &
\begin{bmatrix}
\lambda_1i & w_{1}  & c & 0\\
-w_{1}  & \lambda_1i & 0 & 0\\
-c & 0 & \lambda_1i & w_{2}  \\
0  & 0& -w_{2} & \lambda_1i \\
\end{bmatrix}V_1 = 0 &\quad\rightarrow\quad V_1 = \begin{bmatrix}
\frac{-\lambda_1^2+w_2^2}{cw_2}\\
\frac{w_1i(\lambda_1^2-w_2^2)}{c\lambda_1w_2}\\
\frac{\lambda_1i}{w_2} \\
1 \\
\end{bmatrix}
\\ 
&\text{for $\lambda=\lambda_1i$} &
\begin{bmatrix}
-\lambda_1i & w_{1}  & c & 0\\
-w_{1}  & -\lambda_1i & 0 & 0\\
-c & 0 & -\lambda_1i & w_{2}  \\
0  & 0& -w_{2} & -\lambda_1i \\
\end{bmatrix}V_2 = 0 &\quad\rightarrow\quad V_2 = \begin{bmatrix}
\frac{-\lambda_1^2+w_2^2}{cw_2}\\
\frac{w_1i(-\lambda_1^2+w_2^2)}{c\lambda_1w_2}\\
-\frac{\lambda_1i}{w_2} \\
1 \\
\end{bmatrix}
\\ 
&\text{for $\lambda=-\lambda_2i$} &
\begin{bmatrix}
\lambda_2i & w_{1}  & c & 0\\
-w_{1}  & \lambda_2i & 0 & 0\\
-c & 0 & \lambda_2i & w_{2}  \\
0  & 0& -w_{2} & \lambda_2i \\
\end{bmatrix}V_3 = 0 &\quad\rightarrow\quad V_3 = \begin{bmatrix}
\frac{-\lambda_2^2+w_2^2}{cw_2}\\
\frac{w_1i(\lambda_2^2-w_2^2)}{c\lambda_2w_2}\\
\frac{\lambda_2i}{w_2} \\
1 \\
\end{bmatrix}
\\ 
&\text{for $\lambda=\lambda_2i$} &
\begin{bmatrix}
-\lambda_2i & w_{1}  & c & 0\\
-w_{1}  & -\lambda_2i & 0 & 0\\
-c & 0 & -\lambda_2i & w_{2}  \\
0  & 0& -w_{2} & -\lambda_2i \\
\end{bmatrix}V_4 = 0 &\quad\rightarrow\quad V_4 = \begin{bmatrix}
\frac{-\lambda_2^2+w_2^2}{cw_2}\\
\frac{w_1i(-\lambda_2^2+w_2^2)}{c\lambda_2w_2}\\
-\frac{\lambda_2i}{w_2} \\
1 \\
\end{bmatrix} 
\\ 
\end{aligned}
\end{equation}

With $\bm{T}=[V_1,V_2,V_3,V_4]$ we now get:

\begin{equation}
\begin{aligned}
    \bm{T} &= \input{Math/T_two}
\\
\\
\bm{\Lambda} &= \begin{bmatrix}
-\lambda_1i & 0 & 0 & 0 \\
 0  & \lambda_1i & 0 & 0 \\
 0 & 0 & -\lambda_2i &0\\
 0 & 0 & 0 & \lambda_2i\\
\end{bmatrix}
\\
\bm{T}^{-1} &= \input{Math/T_two_inv}
\end{aligned}\label{eq:eigendecom_members2}
\end{equation}


\begin{sidewaysfigure}
If we fill in \autoref{eq:matrix_exp_decom} we obtain $s(t)$ for a given initial state $s^0 = \left[x^0_1 , y^0_1 , x^0_2 , y^0_2 \right]^T$:

\begin{equation}    \tiny
\begin{aligned}\label{math:multi_solve}
    s(t) &= \bm{T}e^{\bm{\Lambda}t} \bm{T}^{-1}s^0
    \\
    s(t) &= \bm{T}
    \begin{bmatrix}
        \frac{1}{2}\left(-x^0_1\frac{c w_{2}}{\lambda_{1}^{2} - \lambda_{2}^{2}} -y^0_1 \frac{c \lambda_{1} \lambda_{2}^{2}}{ w_{1} w_{2} \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}i + x^0_2\frac{\lambda_{1} \left(\lambda_{2}^{2} - w_{2}^{2}\right)}{ w_{2} \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}i - y^0_2\frac{- \lambda_{2}^{2} + w_{2}^{2}}{\lambda_{1}^{2} - \lambda_{2}^{2}}\right)e^{-\lambda_1it}\\
        \frac{1}{2}\left(- x^0_1\frac{c w_{2}}{ \lambda_{1}^{2} - \lambda_{2}^{2}} +  y^0_1\frac{c \lambda_{1} \lambda_{2}^{2}}{ w_{1} w_{2} \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}i - x^0_2\frac{\lambda_{1} \left( \lambda_{2}^{2} - w_{2}^{2}\right)}{ w_{2} \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}i - y^0_2\frac{- \lambda_{2}^{2} + w_{2}^{2}}{\lambda_{1}^{2} - \lambda_{2}^{2}}\right)e^{\lambda_1it}\\
        \frac{1}{2}\left(x^0_1\frac{c w_{2}}{ \lambda_{1}^{2} - \lambda_{2}^{2}} + y^0_1\frac{c \lambda_{1}^{2} \lambda_{2}}{w_{1} w_{2} \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}i - x^0_2\frac{\lambda_{2} \left( \lambda_{1}^{2} + w_{2}^{2}\right)}{ w_{2} \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}i + y^0_2 \frac{\lambda_{1}^{2} - w_{2}^{2}}{ \lambda_{1}^{2} - \lambda_{2}^{2}}\right)e^{-\lambda_2it}\\
        \frac{1}{2}\left(x^0_1\frac{c w_{2}}{ \lambda_{1}^{2} - \lambda_{2}^{2}} - y^0_1\frac{c \lambda_{1}^{2} \lambda_{2}}{ w_{1} w_{2} \left(\lambda_{1}^{2} - \lambda_{2}^{2}\right)}i + x^0_2\frac{\lambda_{2} \left(\lambda_{1}^{2} + w_{2}^{2}\right)}{ w_{2} \left(\lambda_{1}^{2}  \lambda_{2}^{2}\right)}i + y^0_2\frac{\lambda_{1}^{2} - w_{2}^{2}}{ \lambda_{1}^{2} - \lambda_{2}^{2}}\right)e^{\lambda_2it}\\
    \end{bmatrix}\\
    &= 
    \begin{bmatrix}
    \frac{1}{2}x^{0^*}_1\left(-e^{-\lambda_1it}-e^{\lambda_1it} + e^{-\lambda_2it}+e^{\lambda_2it}\right) +
    \frac{1}{2}y^{0^*}_1\left(-ie^{-\lambda_1it}+ie^{\lambda_1it} + ie^{-\lambda_2it}-ie^{\lambda_2it}\right) +
    \frac{1}{2}x^{0^*}_2\left(-ie^{-\lambda_1it}+ie^{\lambda_1it} - ie^{-\lambda_2it}+ie^{\lambda_2it}\right) +
    \frac{1}{2}y^{0^*}_2\left(-e^{-\lambda_1it}-e^{\lambda_1it} + e^{-\lambda_2it}+e^{\lambda_2it}\right)
        \\
    \frac{1}{2}x^{0^*}_1\left(-ie^{-\lambda_1it}+ie^{\lambda_1it} + ie^{-\lambda_2it}+ie^{\lambda_2it}\right) +
    \frac{1}{2}y^{0^*}_1\left(-e^{-\lambda_1it}+e^{\lambda_1it} + -e^{-\lambda_2it}+e^{\lambda_2it}\right) +
    \frac{1}{2}x^{0^*}_2\left(e^{-\lambda_1it}-e^{\lambda_1it} + e^{-\lambda_2it}-e^{\lambda_2it}\right) +
    \frac{1}{2}y^{0^*}_2\left(-ie^{-\lambda_1it}+ie^{\lambda_1it} - ie^{-\lambda_2it}+ie^{\lambda_2it}\right)
        \\
    \frac{1}{2}x^{0^*}_1\left(-ie^{-\lambda_1it}+ie^{\lambda_1it} + ie^{-\lambda_2it}+ie^{\lambda_2it}\right) +
    \frac{1}{2}y^{0^*}_1\left(-e^{-\lambda_1it}+e^{\lambda_1it} + -e^{-\lambda_2it}+e^{\lambda_2it}\right) +
    \frac{1}{2}x^{0^*}_2\left(e^{-\lambda_1it}-e^{\lambda_1it} + e^{-\lambda_2it}-e^{\lambda_2it}\right) +
    \frac{1}{2}y^{0^*}_2\left(-ie^{-\lambda_1it}+ie^{\lambda_1it} - ie^{-\lambda_2it}+ie^{\lambda_2it}\right)
        \\
    \frac{1}{2}x^{0^*}_1\left(-e^{-\lambda_1it}-e^{\lambda_1it} + e^{-\lambda_2it}+e^{\lambda_2it}\right) +
    \frac{1}{2}y^{0^*}_1\left(-ie^{-\lambda_1it}+ie^{\lambda_1it} + ie^{-\lambda_2it}-ie^{\lambda_2it}\right) +
    \frac{1}{2}x^{0^*}_2\left(-ie^{-\lambda_1it}+ie^{\lambda_1it} - ie^{-\lambda_2it}+ie^{\lambda_2it}\right) +
    \frac{1}{2}y^{0^*}_2\left(-e^{-\lambda_1it}-e^{\lambda_1it} + e^{-\lambda_2it}+e^{\lambda_2it}\right)
    \end{bmatrix}\\ \\
  & {\footnotesize \textrm{with $x^{0^*}_1 = f(x^0_1, c, w_1, w_2, \lambda_1, \lambda_2)$, $y^{0^*}_1 = f(y^0_1, c, w_1, w_2, \lambda_1, \lambda_2)$, $x^{0^*}_2 = f(x^0_2, c, w_1, w_2, \lambda_1, \lambda_2)$, $y^{0^*}_2 = f(y^0_2, c, w_1, w_2, \lambda_1, \lambda_2) \in\mathbb{R}$}}\\ \\
    &=
    \begin{bmatrix}
    \frac{1}{2}\left(-x^{0^*}_1 - y^{0^*}_2\right)\left(e^{-\lambda_1it}+e^{\lambda_1it} \right)+ \frac{1}{2}\left(y^{0^*}_1 - x^{0^*}_2\right)i\left(-e^{-\lambda_1it}+e^{\lambda_1it} \right)+ 
    \frac{1}{2}\left(x^{0^*}_1 + y^{0^*}_2\right)\left(e^{-\lambda_2it}+e^{\lambda_2it} \right) - \frac{1}{2}\left(-y^{0^*}_1 + x^{0^*}_2\right)i\left(-e^{-\lambda_2it}-e^{\lambda_2it} \right) 
        \\
    \frac{1}{2}\left(x^{0^*}_1 + y^{0^*}_2\right)i\left(-e^{-\lambda_1it}+e^{\lambda_1it} \right) + \frac{1}{2}\left(y^{0^*}_1 - x^{0^*}_2\right)\left(e^{-\lambda_1it}+e^{\lambda_1it} \right) - 
    \frac{1}{2}\left(x^{0^*}_1 + y^{0^*}_2\right)i\left(-e^{-\lambda_2it}+e^{\lambda_2it} \right) + \frac{1}{2}\left(-y^{0^*}_1 + x^{0^*}_2\right)\left(e^{-\lambda_2it}+e^{\lambda_2it} \right)
        \\
    \frac{1}{2}\left(x^{0^*}_1 + y^{0^*}_2\right)i\left(-e^{-\lambda_1it}+e^{\lambda_1it} \right) + \frac{1}{2}\left(y^{0^*}_1 - x^{0^*}_2\right)\left(e^{-\lambda_1it}+e^{\lambda_1it} \right) - 
    \frac{1}{2}\left(x^{0^*}_1 + y^{0^*}_2\right)i\left(-e^{-\lambda_2it}+e^{\lambda_2it} \right) + \frac{1}{2}\left(-y^{0^*}_1 + x^{0^*}_2\right)\left(e^{-\lambda_2it}+e^{\lambda_2it} \right)
        \\
    \frac{1}{2}\left(-x^{0^*}_1 - y^{0^*}_2\right)\left(e^{-\lambda_1it}+e^{\lambda_1it} \right)+ \frac{1}{2}\left(y^{0^*}_1 - x^{0^*}_2\right)i\left(-e^{-\lambda_1it}+e^{\lambda_1it} \right)+ 
    \frac{1}{2}\left(x^{0^*}_1 + y^{0^*}_2\right)\left(e^{-\lambda_2it}+e^{\lambda_2it} \right) - \frac{1}{2}\left(-y^{0^*}_1 + x^{0^*}_2\right)i\left(-e^{-\lambda_2it}-e^{\lambda_2it} \right) 
    \end{bmatrix}\\
        &=
    \begin{bmatrix}
    \left(-x^{0^*}_1 - y^{0^*}_2\right)\cos{\lambda_1t} + \left(y^{0^*}_1 - x^{0^*}_2\right)\sin{\lambda_1t} + 
    \left(x^{0^*}_1 + y^{0^*}_2\right)\cos{\lambda_2t} - \left(-y^{0^*}_1 + x^{0^*}_2\right)\sin{\lambda_2t}
        \\
    \left(x^{0^*}_1 + y^{0^*}_2\right)\sin{\lambda_1t} + \left(y^{0^*}_1 - x^{0^*}_2\right)\cos{\lambda_1t} - 
    \left(x^{0^*}_1 + y^{0^*}_2\right)\sin{\lambda_2t} + \left(-y^{0^*}_1 + x^{0^*}_2\right)\cos{\lambda_2t}
        \\
    \left(x^{0^*}_1 + y^{0^*}_2\right)\sin{\lambda_1t} + \left(y^{0^*}_1 - x^{0^*}_2\right)\cos{\lambda_1t} - 
    \left(x^{0^*}_1 + y^{0^*}_2\right)\sin{\lambda_2t} + \left(-y^{0^*}_1 + x^{0^*}_2\right)\cos{\lambda_2t}
        \\
    \left(-x^{0^*}_1 - y^{0^*}_2\right)\cos{\lambda_1t} + \left(y^{0^*}_1 - x^{0^*}_2\right)\sin{\lambda_1t} + 
    \left(x^{0^*}_1 + y^{0^*}_2\right)\sin{\lambda_2t} - \left(-y^{0^*}_1 + x^{0^*}_2\right)\cos{\lambda_2t}
    \end{bmatrix}\\
        &=
    \begin{bmatrix}
    \sqrt{\left(-x^{0^*}_1 - y^{0^*}_2\right)^2 + \left(y^{0^*}_1 - x^{0^*}_2\right)^2}\cos{\left(\lambda_1t - \arctan\frac{y^{0^*}_1 - x^{0^*}_2}{-x^{0^*}_1 - y^{0^*}_2}\right)} - 
    \sqrt{\left(x^{0^*}_1 + y^{0^*}_2\right)^2 + \left(-y^{0^*}_1 + x^{0^*}_2\right)^2}\cos{\left(\lambda_2t + \arctan-\frac{-y^{0^*}_1 + x^{0^*}_2}{x^{0^*}_1 + y^{0^*}_2}\right)}
        \\
    \sqrt{\left(x^{0^*}_1 + y^{0^*}_2\right)^2 + \left(y^{0^*}_1 - x^{0^*}_2\right)^2}\cos{\left(\lambda_1t - \arctan\frac{x^{0^*}_1 + y^{0^*}_2}{y^{0^*}_1 - x^{0^*}_2}\right)} + 
    \sqrt{\left(x^{0^*}_1 + y^{0^*}_2\right)^2 + \left(-y^{0^*}_1 + x^{0^*}_2\right)^2}\cos{\left(\lambda_2t + \arctan\frac{x^{0^*}_1 + y^{0^*}_2}{-y^{0^*}_1 + x^{0^*}_2}\right)}
        \\
    \sqrt{\left(x^{0^*}_1 + y^{0^*}_2\right)^2 + \left(-y^{0^*}_1 + x^{0^*}_2\right)^2}\cos{\left(\lambda_1t - \arctan\frac{x^{0^*}_1 + y^{0^*}_2}{-y^{0^*}_1 + x^{0^*}_2}\right)} + 
    \sqrt{\left(x^{0^*}_1 + y^{0^*}_2\right)^2 + \left(y^{0^*}_1 - x^{0^*}_2\right)^2}\cos{\left(\lambda_2t + \arctan\frac{x^{0^*}_1 + y^{0^*}_2}{y^{0^*}_1 - x^{0^*}_2}\right)}
        \\
    \sqrt{\left(-x^{0^*}_1 - y^{0^*}_2\right)^2 + \left(-y^{0^*}_1 + x^{0^*}_2\right)^2}\cos{\left(\lambda_1t - \arctan\frac{-y^{0^*}_1 + x^{0^*}_2}{-x^{0^*}_1 - y^{0^*}_2}\right)} - 
    \sqrt{\left(x^{0^*}_1 + y^{0^*}_2\right)^2 + \left(y^{0^*}_1 - x^{0^*}_2\right)^2}\cos{\left(\lambda_2t + \arctan-\frac{y^{0^*}_1 - x^{0^*}_2}{x^{0^*}_1 + y^{0^*}_2}\right)}
    \end{bmatrix}
\end{aligned}
\end{equation}
\end{sidewaysfigure}
\clearpage

==> 4/figures/Solve_single.tex <==
From now on we will use Newton's dot notation to denote derivatives with respect to time. A single oscillator can be described by the following LTI-matrix.
\begin{equation} 
\begin{split}
\Dot{s} & = \begin{bmatrix}
0 & w \\
-w & 0 \\
\end{bmatrix} \begin{bmatrix}
x\\
y\\
\end{bmatrix} = \bm{A}s\\
\end{split}\label{eq:As}
\end{equation}

Rewriting gives us the following differential equation to solve:

\begin{equation}
    \Dot{s}-\bm{A}s = 0
\end{equation}

This is a first-order differential equation that can be written as follows using the Taylor series expansion:

\begin{equation}\label{eq:matrix_exp}
    s(t)=e^{\bm{A}t}s^0    \quad \mathrm{where} \quad    e^{\bm{A}t} := I+\bm{A}t+ \bm{A}^2\frac{t^2}{2!} + \bm{A}^3\frac{t^3}{3!} +.. = \sum _{ m=0}^{\infty }\frac{(\bm{A}t)^{m}}{m!}
\end{equation}

Here, $s^0$ indicates the initial state of the CPG (i.e. $x$,$y-$neuron). Properties of this power series are derived more in depth here \cite{Hall_2015}. We show that this expansion is true by taking the derivative of \autoref{eq:matrix_exp}:

\begin{align}
\Dot{s}(t) & = \frac{d}{dt}  s(t) \nonumber\\
& = \frac{d}{dt}  ( e^{\bm{A}t}s^0) \nonumber\\
& = \frac{d}{dt}(e^{\bm{A}t})s^0 & \text{\raggedright\footnotesize$s^0$ is time-independent} \nonumber\\
& = \frac{d}{dt}(I+\bm{A}t+ \bm{A}^2\frac{t^2}{2!} + \bm{A}^3\frac{t^3}{3!} +..)s^0 \nonumber\\
& = \phantom{\frac{d}{dt}}(0 + \bm{A}\phantom{t} + \bm{A}^2t \hspace{0.55em}+ \bm{A}^3\frac{t^2}{2!} +..)s^0\\
& = \hspace{0.1em}\bm{A}(I+\bm{A}t+ \bm{A}^2\frac{t^2}{2!} + \bm{A}^3\frac{t^3}{3!} +..)s^0 \nonumber\\
& = \hspace{0.1em}\bm{A} e^{\bm{A}t}s^0 \nonumber\\
& = \hspace{0.1em}\bm{A}  s(t) & \text{\footnotesize\autoref{eq:As} \nonumber} 
\end{align}



\autoref{eq:matrix_exp} is still confusing, as it is not clear what this infinite series entails for our CPG state over time. Fortunately, we can diagonalize $\bm{A}$ through its eigendecomposition $\bm{A} = \bm{T \Lambda T}^{-1}$ with $\bm{\Lambda}$ being a zero matrix with the eigenvalues on its diagonal and $\bm{T}$ being its corresponding eigenvectors. Rewriting \autoref{eq:matrix_exp} leads to \cite{Hall_2015}:
\begin{equation} \label{eq:matrix_exp_decom}
    \begin{aligned}
    s(t) &= e^{\bm{T\Lambda T^{-1}}t}s^0 \\
        &= \bm{T}e^{\bm{\Lambda}t}\bm{T}^{-1}s^0\\
    \end{aligned}
\end{equation}


If we solve the factorisation, we find the eigenvalues for our single oscillator:

\begin{equation}
\begin{aligned}
    \mathrm{det}(\bm{A}-I\lambda)&=0\\
    \mathrm{det}\left(\begin{bmatrix}
-\lambda & w \\
-w & -\lambda \\
\end{bmatrix}\right) & = 0\\
\lambda^2+w^2 &=0\\
\lambda_{1,2} &= \pm iw
\end{aligned}
\end{equation}

We obtain two purely imaginary numbers as our eigenvalues. To obtain the eigenvectors we need to solve $(\bm{A}-I\lambda)V=0$ for both eigenvalues:

\begin{equation}
\begin{aligned}
    (\bm{A}-I\lambda)V&=0 \\ \\
    \begin{bmatrix}
iw & w \\
-w & iw \\
\end{bmatrix}V_1 & = 0 &\quad\rightarrow\quad& V_1 = \begin{bmatrix}
i \\
1 \\
\end{bmatrix} &&\text{if $\lambda = -iw$}
\\ 
    \begin{bmatrix}
-iw & w \\
-w & -iw \\
\end{bmatrix}V_2 & = 0 &\quad\rightarrow\quad& V_2 = \begin{bmatrix}
-i \\
1 \\
\end{bmatrix} &&\text{if $\lambda = iw$}
\end{aligned}
\end{equation}

With $\bm{T}=[V_1,V_2]$ we now get:

\begin{equation}
    \bm{T} = \begin{bmatrix}
i & -i \\
1 & 1 \\
\end{bmatrix} \quad,\quad 
\bm{\Lambda} = \begin{bmatrix}
-iw & 0 \\
 0  & iw
\end{bmatrix} \quad and,\quad \bm{T}^{-1} = 
\begin{bmatrix}
-\frac{i}{2} & \frac{1}{2} \\
\frac{i}{2} & \frac{1}{2} \\
\end{bmatrix}\label{eq:eigendecom_members}
\end{equation}

Filling in $\bm{T\Lambda T}^{-1}$ in \autoref{eq:matrix_exp_decom} to obtain $s(t)$ for a given initial state $s^0 = [x^0,y^0]^T$:
% \begin{equation}
\begin{align*}
    s(t) &= \bm{T}e^{\bm{\Lambda}t} \bm{T}^{-1}s^0\\
    s(t) &= \begin{bmatrix}
i & -i \\
1 & 1 \\
\end{bmatrix} \mathrm{exp}\left(\begin{bmatrix}
-iw & 0 \\
 0  & iw
\end{bmatrix}t\right)
\begin{bmatrix}
-\frac{i}{2} & \frac{1}{2} \\
\frac{i}{2} & \frac{1}{2} \\
\end{bmatrix}
\begin{bmatrix}
x^0 \\
y^0 \\
\end{bmatrix} \\
% =========================================================================
&= \begin{bmatrix}
i & -i \\
1 & 1 \\
\end{bmatrix} \begin{bmatrix}
e^{-iwt} & 0 \\
 0  & e^{iwt}
\end{bmatrix}
\begin{bmatrix}
-\frac{i}{2}x^0 +  \frac{1}{2}y^0\\
\frac{i}{2}x^0 +  \frac{1}{2}y^0 \\
\end{bmatrix} \text{\hspace{2em} $e^{\bm{\Lambda}t}=\mathrm{diag}(e^{-iwt}, e^{iwt})$ see \autoref{eq:matrix_exp}}\\
% ==========================================================================
&= \begin{bmatrix}
i & -i \\
1 & 1 \\
\end{bmatrix}
\begin{bmatrix}
\frac{1}{2}(-ix^0e^{-iwt} +  y^0e^{-iwt})\\
\frac{1}{2}(ix^0e^{iwt} +  y^0e^{iwt}) \\
\end{bmatrix}\\
% ==========================================================================
&= 
\begin{bmatrix}
\frac{1}{2}(x^0e^{-iwt} +  iy^0e^{-iwt}) + \frac{1}{2}(x^0e^{iwt} -  iy^0e^{iwt})\\
\frac{1}{2}(-ix^0e^{-iwt} +  y^0e^{-iwt}) + \frac{1}{2}(ix^0e^{iwt} +  y^0e^{iwt}) \\
\end{bmatrix}\\
% ==========================================================================
&= 
\begin{bmatrix}
\frac{1}{2}x^0(e^{-iwt} + e^{iwt} ) + \frac{1}{2}iy^0(e^{-iwt} -  e^{iwt})\\
\frac{1}{2}ix^0(-e^{-iwt} + e^{iwt}) + \frac{1}{2}y^0(e^{-iwt} +  e^{iwt}) \\
\end{bmatrix}\\ \\
\multicolumn{2}{l}{\text{Euler's formula show: $e^{-iwt}+e^{iwt} = 2\cos{wt}$, $e^{-iwt}-e^{iwt} = 2i\sin{wt}$}}\\ \\
% ==========================================================================
&= 
\begin{bmatrix}
x^0\cos{wt}+ y^0\sin{wt} \\
-x^0\sin{wt} + y^0\cos{wt} \\
\end{bmatrix}\\
% ==========================================================================
&= 
\begin{bmatrix}
\sqrt{(x^0)^2+(y^0)^2}\cos{(wt - \arctan{\frac{y^0}{x^0}})}\\
\sqrt{(x^0)^2+(y^0)^2}\cos{(wt + \arctan{\frac{x^0}{y^0}})}\\
\end{bmatrix}\\
\end{align*}
% \end{equation}

Thus, for a single CPG the analytical solution of both neurons' state is:

\begin{align}\label{math:single_solve}
    x(t)&=\sqrt{(x^0)^2+(y^0)^2}\cos{(wt - \arctan{\frac{y^0}{x^0}})}\\
    y(t)&=\sqrt{(x^0)^2+(y^0)^2}\cos{(wt + \arctan{\frac{x^0}{y^0}})}
\end{align}

==> 4/figures/final_frames/figure.tex <==
\begin{figure}[h!]
\centering
\begin{minipage}[c]{0.99\linewidth}
\centering
\footnotesize
\end{minipage}
\begin{minipage}[c]{\linewidth}
        \begin{minipage}[t]{0.32\linewidth}
            \centering
            \subfloat[Ant]{
            \begin{minipage}[t]{\linewidth}
            \centering
            \begin{center}
                            \Gait \\
                            \tiny{\textbf{ISO} \hspace{8.5em} \textbf{WO}} 
                            \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/ant/gait.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/ant/gait.jpg}
                             \\ \RotL \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/ant/anti-clockwise.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/ant/anti-clockwise.jpg} \\ \RotR \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/ant/clockwise.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/ant/clockwise.jpg}
            \end{center}
            \end{minipage}
                             }
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\linewidth}
            \centering
            \subfloat[Gecko]{            
            \begin{minipage}[t]{\linewidth}
            \centering
            \begin{center}
                            \Gait \\
                            \tiny{\textbf{ISO} \hspace{8.5em} \textbf{WO}} 
                            \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/gecko/gait.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/gecko/gait.jpg}
                             \\ \RotL \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/gecko/anti-clockwise.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/gecko/anti-clockwise.jpg} \\ \RotR \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/gecko/clockwise.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/gecko/clockwise.jpg}
            \end{center}
            \end{minipage}
            }
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.32\linewidth}
            \centering
            \subfloat[Spider]{            
            \begin{minipage}[t]{\linewidth}
            \centering
            \begin{center}
                            \Gait \\
                            \tiny{\textbf{ISO} \hspace{8.5em} \textbf{WO}} 
                            \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/spider/gait.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/spider/gait.jpg}
                             \\ \RotL \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/spider/anti-clockwise.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/spider/anti-clockwise.jpg} \\ \RotR \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/spider/clockwise.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/spider/clockwise.jpg}
            \end{center}
            \end{minipage}
            }
        \end{minipage}
    \end{minipage}
\begin{minipage}[c]{\textwidth}
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \subfloat[Blokky]{            
            \begin{minipage}[t]{\linewidth}
            \centering
            \begin{center}
                            \Gait \\
                            \tiny{\textbf{ISO} \hspace{8.5em} \textbf{WO}} 
                            \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/blokky/gait.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/blokky/gait.jpg}
                             \\ \RotL \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/blokky/anti-clockwise.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/blokky/anti-clockwise.jpg} \\ \RotR \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/blokky/clockwise.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/blokky/clockwise.jpg}
            \end{center}
            \end{minipage}
            }
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \subfloat[Salamander]{            
            \begin{minipage}[t]{\linewidth}
            \centering
            \begin{center}
                            \Gait \\
                            \tiny{\textbf{ISO} \hspace{8.5em} \textbf{WO}} 
                            \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/salamander/gait.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/salamander/gait.jpg}
                             \\ \RotL \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/salamander/anti-clockwise.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/salamander/anti-clockwise.jpg} \\ \RotR \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/salamander/clockwise.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/salamander/clockwise.jpg}
            \end{center}
            \end{minipage}
            }
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \subfloat[Stingray]{            
            \begin{minipage}[t]{\linewidth}
            \centering
            \begin{center}
                            \Gait \\
                            \tiny{\textbf{ISO} \hspace{8.5em} \textbf{WO}} 
                            \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/stingray/gait.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/stingray/gait.jpg}
                             \\ \RotL \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/stingray/anti-clockwise.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/stingray/anti-clockwise.jpg} \\ \RotR \\
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/ISO/stingray/clockwise.jpg}
                             \includegraphics[width=0.4\linewidth]{figures/final_frames/WO/stingray/clockwise.jpg}
            \end{center}
            \end{minipage}
            }
    \end{minipage}
\end{minipage}
\caption{\label{fig:res_real} Initial State optimisation (ISO, blue) on real robots produces similar performanced to the sim-to-real transfer of the best out of the 30 runs from Weight Optimisation (WO*, orange). The bars show the performance of each physical robot concerning three different skills: gait (\Gait) and anti-/clockwise (\RotL, \RotR). The striped bars indicate the overall best ISO run (based on the total rank over all the skills).}
\end{figure}

==> 4/figures/legends_APP.tex <==
\begin{figure}\caption{Different representations of the same CPG.}
\end{figure}\begin{figure}\caption{Two inter-connected CPGs.}
\end{figure}\begin{figure}\caption{Density plot of the distribution of eigenvalues for a random CPG with 10 oscillators. Inter-connected density (d) indicates the percentage of inter-connections between x-neurons in the network. Weights and connections are randomly sampled from a uniform distribution between [-1,1].}
\end{figure}\begin{figure}\caption{WO finds a wide distribution of eigenvalues with varying weights across 30 different runs. \textbf{a}) Distribution of: Green, the true eigenvalues of the target CPG-network to be approximated; Blue, the initial eigenvalues of the random networks at the start of an evolutionary run; Orange, the best CPG-network's Eigenvalues after weight optimisation. \textbf{b}) True weights of the target network (in green), with the end-values of the best weights after optimisation (in orange) and the black lines indicating standard error.}
	\label{fig:results_freq}
\end{figure}\begin{figure}\caption{Initial State optimisation (ISO, blue) outperforms Weight optimisation (WO, orange) in time-series approximation experiment. The lines indicate the show the mean performance curves over 30 independent runs ($N_{rep}=30$) $\pm SE$.}
\end{figure}\begin{figure}\caption{\label{fig:APP_hyper_param} ISO hyper-parameter tests learning curves (mean $N_{rep}=30$, highlighting indicates $\pm SE$.). We compare efficacy to learn a time-series of length `window size' (denoted $\textsl{W}_*$). Rows: increasing trial time relative to window length (1:1 ratio means one sample per trial). Columns: number of trials. Note that the total experiment time increases with $\textsl{W}_*$, trial time, and \# trials.}
\end{figure}\begin{figure}\caption{ISO scalability tests learning curves (mean $N_{rep}=30$, Shaded area indicate $\pm SE$.). We compare efficacy to learn `n' time-series in parallel (denoted $\textsl{T}_n$).}
\end{figure}\begin{figure}\end{figure}\begin{figure}\caption{\label{fig:App_real_best} Initial State optimisation (ISO, left columns in each morphology) outperforms the best sim-to-real transfer of Weight Optimisation (WO*, right column) in eleven out of eighteen locomotion tasks (green border indicate the best robot behaviour). For each morphology we recorded the final optimised behaviour of three different skills: gait (\Gait) and anti-/clockwise (\RotL, \RotR). The white line indicates the position over time while the red (semi-)circle indicates the orientation over time (going from white to pink to red) with the red vector showing the current orientation.}

\end{figure}\begin{figure}\caption{\small Simulator and corresponding real world performance. Colors indicate an increase/decrease with respect to simulated performance (red/green respectively). Final column indicate the average performance drop per skill among all robots, with an underline indicating a statistically significant difference between ISO and WO* ($p<<0.05$ for all skills)}
\end{figure}

==> 4/figures/legends_MAIN.tex <==
\begin{figure}\caption{Initial State Optimisation on Central Pattern Generators (CPGs) quickly finds different locomotion skills (Gait: \Gait; Clockwise rotation: \RotR; Anti-clockwise rotation: \RotL). \textbf{A.} Our robot is initialised with a network of interconnected CPGs in which we freeze all weights. \textbf{B.} \textit{Top}, we sample a random initial state of the CPG-network and produce a time-series (based on its dynamics) that provides motor commands to our robot. \textbf{B.} \textit{Bottom-left}, we collect data of the intermediate CPG states ($\mathcal{S}$) and the corresponding robot behaviour ($\mathcal{D}$). \textbf{B.} \textit{Bottom-right}, we consider the intermediate CPG states as additional `initial state' samples (\textit{bootstrapping}) and assess the fitness values for multiple skills at the same time (\textit{parallelisation}). \textbf{C.} In the end, we re-test the best initial state sample for each skill \{$\bm{s^{*}_{\RotL}}, \bm{s^{*}_{\Gait}}, \bm{s^{*}_{\RotR}}$\} encoded in the same CPG-network. The real-world behaviour is shown in three pictures on the right with the robot position trajectory as a white line, and its orientation in red fading on a (semi-)circle.}
       	\end{figure}\begin{figure}\caption{Test suite of six robots as rendered in the simulator (left) and their physical twin (right).}
\end{figure}\begin{figure}\caption{\label{fig:res_tteq_curve} Initial State optimisation (ISO, blue curves) outperforms  both PPO (gray) and Weight optimisation (WO, orange). WO is outperformed in the first \SI{64}{\min} on average. Learning curves show Mean Best Fitness ($N_{rep}=30\pm\mathrm{SE}$) for gait (\Gait) and anti-/clockwise rotation (\RotL, \RotR) skills for the six different robots in simulation. The vertical dotted lines indicate the first cross-over point after which WO begins to outperform ISO, i.e., Time Till Equal Quality (TTEQ, higher is better). The specific TTEQ for each skill is presented in each sub-caption (ordered in: \Gait, \RotL, \RotR), while no cross-over point is denoted with a dash (-).}
\end{figure}\begin{figure}\caption{\label{fig:res_norm_perf} Initial State optimisation (ISO$_\Sigma$) obtains 50\% performance of Weight optimisation (WO$_{\Gait}$, WO$_{\RotL}$, WO$_{\RotR}$) in less than 5\% of the time. The bars indicate the time needed to obtain normalised performance quality with respect to WO ($N_{rep}=30$). In the sub-caption we specify the total time needed to attain 75\% relative performance in minutes (WO time vs. ISO time).}
\end{figure}\begin{figure}\caption{\label{fig:res_real} Initial State optimisation (ISO, blue) on real robots produces similar performance to the sim-to-real transfer of the best out of the 30 runs from Weight Optimisation (WO*, orange). The bars show the performance of each physical robot concerning three different skills: gait (\Gait) and anti-/clockwise (\RotL, \RotR). The striped bars indicate the overall best ISO run (based on the total rank over all the skills).}
       	\end{figure}\begin{figure}\caption{(\textbf{a}) A single CPG. (\textbf{b}) The CPG-network schematic of our Spider robot, containing eight CPGs (numbers) with ten pairs of neighbouring connections (blue arrows).}
	\end{figure}\begin{figure}\caption{Technical description of our six robots. }
	\end{figure}\begin{figure}\caption{\small Hyperparameters of the RevDE learning algorithm}
  \end{figure}\begin{figure}\caption{\small RevDE weight optimisation of CPG-networks}
  \end{figure}\begin{figure}\caption{\small Random search initial state optimisation of CPG-networks}
\end{figure}\begin{figure}\caption{\small Experimental setup}
 \end{figure}\begin{figure}\caption{\label{alg:unwrap}UNWRAP: Calculate relative $z$-angle between subsequent time-steps}
\end{figure}\begin{figure}\caption{\label{alg:mbf}Mean Best Fitness}
\end{figure}\begin{figure}\caption{\label{alg:tteq}Time Till Equal Quality}
\end{figure}\begin{figure}\caption{\label{alg:norm_perf}Normalised Performance}
\end{figure}


==> 4/figures/multi_skill.tex <==

\begin{minipage}[c]{0.99\textwidth} %## ROW 1
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Ant \footnotesize{($k=8$)}]{\includegraphics[width=\textwidth]{figures/multiskill/ant.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[BabyA \footnotesize{($k=8$)}]{\includegraphics[width=\textwidth]{figures/multiskill/babya.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[BabyB \footnotesize{($k=10$)}]{\includegraphics[width=\textwidth]{figures/multiskill/babyb.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Blokky \footnotesize{($k=5$)}]{\includegraphics[width=\textwidth]{figures/multiskill/blokky.pdf}}
        \end{minipage}
        \hfill
\end{minipage}

\begin{minipage}[c]{0.99\textwidth}  %## ROW 2
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Garrix \footnotesize{($k=10$)}]{\includegraphics[width=\textwidth]{figures/multiskill/garrix.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Gecko \footnotesize{($k=6$)}]{\includegraphics[width=\textwidth]{figures/multiskill/gecko.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Insect \footnotesize{($k=9$)}]{\includegraphics[width=\textwidth]{figures/multiskill/insect.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Linkin \footnotesize{($k=12$)}]{\includegraphics[width=\textwidth]{figures/multiskill/linkin.pdf}}
        \end{minipage}
        \hfill
\end{minipage}

\begin{minipage}[c]{0.99\textwidth}  %## ROW 3
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Longleg \footnotesize{($k=12$)}]{\includegraphics[width=\textwidth]{figures/multiskill/longleg.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Penguin \footnotesize{($k=12$)}]{\includegraphics[width=\textwidth]{figures/multiskill/penguin.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Pentapod \footnotesize{($k=10$)}]{\includegraphics[width=\textwidth]{figures/multiskill/pentapod.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Queen \footnotesize{($k=9$)}]{\includegraphics[width=\textwidth]{figures/multiskill/queen.pdf}}
        \end{minipage}
        \hfill
\end{minipage}

\begin{minipage}[c]{0.99\textwidth}  %## ROW 4
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Salamander \footnotesize{($k=14$)}]{\includegraphics[width=\textwidth]{figures/multiskill/salamander.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Spider \footnotesize{($k=8$)}]{\includegraphics[width=\textwidth]{figures/multiskill/spider.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Squarish \footnotesize{($k=6$)}]{\includegraphics[width=\textwidth]{figures/multiskill/squarish.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Stingray \footnotesize{($k=9$)}]{\includegraphics[width=\textwidth]{figures/multiskill/stingray.pdf}}
        \end{minipage}
\end{minipage}

\begin{minipage}[c]{0.99\textwidth}  %## ROW 5
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Tinlicker \footnotesize{($k=8$)}]{\includegraphics[width=\textwidth]{figures/multiskill/tinlicker.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Turtle \footnotesize{($k=13$)}]{\includegraphics[width=\textwidth]{figures/multiskill/turtle.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[WW \footnotesize{($k=10$)}]{\includegraphics[width=\textwidth]{figures/multiskill/ww.pdf}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{.24\textwidth}
            \centering
            \subfloat[Zappa \footnotesize{($k=11$)}]{\includegraphics[width=\textwidth]{figures/multiskill/zappa.pdf}}
        \end{minipage}
\end{minipage} 
% height=2.75cm

==> general/samenvatting.tex <==
Het wetenschappelijk gebied van Evolutionary Robotics (ER) ``heeft het toepassen van computationele- en evolutionaire technieken op het ontwerp en/of de controller van zowel echte als gesimuleerde robots tot doel" en bestaat sinds het begin van de jaren 90.
ER haalt inspiratie uit de natuur en werkt onder een simpele aanname: als natuurlijke evolutie natuurlijke intelligentie kan voort brengen, dan kan kunstmatige evolutie dat ook voor kunstmatige intelligentie. Hoewel ER systemen op het moment weinig autonoom zijn, vallen (autonome) zichzelf ontwerpende robot-systemem wel binnen de lange-termijn verwachting. Hoewel het bekend is dat de omgeving van grote invloed is voor natuurlijke levensvormen, is de invloed van de omgeving op ER systemen, en in het bijzonder de regulatie van genen door de omgeving, nauwelijks onderzocht.

De belangrijkste doelstellingen van dit onderzoek waren de invloeden van de omgeving op kunstmatig levende systemen duidelijk te maken. Voor het realiseren van dit onderzoek hebben wij een framework ontworpen dat het mogelijk maakt om populaties van robots te evolueren en de invloed van verschillende factoren op de geëvoloueerde robots te kwantificeren.
Onderdelen van dit framework zijn het ontwerp van \textit{a)} een robot coderingsmethode voor morphologie en controller, \textit{b)} morphologische descriptors, \textit{c)} controller descriptors, \textit{d)} gedragsgerelateerde descriptors, \textit{e)} een reeks met omgevingen met verschillende omgevingsfactoren, \textit{f)} een Evolutionary Algorithm, \textit{g)} een leer-mechanisme.
Wij hebben dit framework gebruikt om populaties van robots te ontwerpen die als taak hadden om zich voort te bewegen, hun fitness was sterk gerelateerd aan hun snelheid van voortbewegen. 
Hier presenteren wij de resultaten van meerdere uitgebreide experimenten aangaande de evolutie van morphologie en controllers van modulaire robots. In het bijzonder ligt de focus op de effecten van verschillende omgevingen op phenotypische en gedragsgerelateerde eigenschappen.

Ten eerste hebben wij op verschillende manieren de zoekruimte verkend en gedemonstreerd dat onze robot codering in staat is om hoge mates van diversiteit te coderen. 
Dit betekent dat een groot aantal morphologische vormen gevonden werden door evolutie.
Een aantal van van deze vormen had meerdere ledematen, een symmetrische structuur, proportionele morphologie, enz. 
Onder deze robots waren er exemplaren die dierlijke morphologische structuren en manieren van voortbeweging vertoonden.
Er waren bijvoorbeeld robots die qua structuur en manier van voortbeweging leken op onder andere salamanders, schildpadden, penguins en insecten.
Ten tweede hebben wij aangetoond dat gegeven een vlakke omgeving de selectiedruk heel sterk is voor robots met de morphologie van slangen (gekarakteriseerd door het bestaan uit één grote ledemaat), met rollen als manier van voortbeweging. 
Opmerkelijk was, dat deze eenvoudige slang-achtige vorm van robot zich in vrijwel alle gevallen sneller ging voortbewegen dan andere, eerder beschreven variaties.
Ten derde laten wij zien, dat het hellen van de vloer een nieuwe selectiedruk oplevert. 
In dit geval hadden de robots meer ledematen, waren proportioneler en kleiner, ook veranderde hun manier van voortbewegen van rollen naar roeien en slepen.
Daarnaast hebben wij in verdere experimenten veranderingen in de omgeving op twee verschillende manieren getest: over generaties of gedurende de levensduur van de robot. 
In het tweede geval was er, vanzelfsprekend, omdat de robots over dezelfde morphologie en controller beschikken, sprake van een trade-off.
De robots slaagden erin om zich voort te bewegen in beide omgevings-condities (seizoenen), maar hun prestatie was slechter dan in het geval waarin ze in elke statische omgeving apart getraind waren.
Tenslotte hebben wij een oplossing bedacht om de door het boven beschrevene trade-off veroorzaakte verslechtering in prestatie te verhelpen.
Deze oplossing is een nieuwe methode voor robot-codering genoemd \textit{Plasticoding}.
Deze codering geeft de genotype van robots het vermogen van \textit{phenotypische plasticiteit}, wat betekent dat een individu verschillende morphologien, controllers en gedragspatronen gedurende zijn levensduur kan ontwikkelen als een reactie op omgevings-gerelateerde stimuli.
Door \textit{Plasticoding} konden wij de verslechtering in prestatie reduceren. Het resultaat van \textit{Plasticoding} is een verbetering van 58\% op een baseline zonder plasticiteit. 

Omdat de omgeving van grote invloed is voor natuurlijke levensvormen, geloven wij dat dit onderwerp veel kansen biedt in het verbeteren van ER systemen. Desondanks is onderzoek naar dit onderwerp zeer schaars. Ons werk is daarom een fundamentele stap in de richting van een lange-termijn visie: het realiseren van kunstmatig leven in robots met de complexiteit en adaptiviteit van natuurlijk leven.

